Optimal Weighted Load Balancing in TCAMs

Traffic splitting is a required functionality in networks, for example for load balancing over multiple paths or among different servers. The capacities of the servers determine the partition by which traffic should be split. A recent approach implements traffic splitting within the ternary content addressable memory (TCAM), which is often available in switches. It is important to reduce the amount of memory allocated for this task since TCAMs are power consuming and are often also required for other tasks such as classification and routing. Previous work showed how to compute the smallest prefix-matching TCAM necessary to implement a given partition exactly. In this paper we solve the more practical case, where at most $n$ prefix-matching TCAM rules are available, restricting the ability to implement exactly the desired partition. We give simple and efficient algorithms to find $n$ rules that generate a partition closest in $L_\infty$ to the desired one. We do the same for a one-sided version of $L_\infty$ which equals to the maximum overload on a server and for a relative version of it. We use our algorithms to evaluate how the expected error changes as a function of the number of rules, the number of servers, and the width of the TCAM.

==> supplementary_materials_file.tex <==
\section*{Optimal Weighted Load Balancing in TCAMs - SUPPLEMENTARY MATERIALS}

%%%###%%%###%%%###%%% \input{section_bm_niagara_algorithms_review.tex}

\section{Reviewing Bit Matcher and Niagara}
\label{section_review_bitmatcher_and_niagara}

In this Section we provide pseudo-code (see Algorithm~\ref{algorithms_bitmatcher_and_niagara}) and a short description of the  algorithms Bit Matcher~\cite{BitMatcher} and Niagara~\cite{Niagara}. This description is based on~\cite{BitMatcher}.

Both algorithms are given a list of weights $x_1,\ldots,x_k$ that sum to $2^W$ as input, and compute a sequence of transactions that can be mapped to a TCAM. Bit Matcher can be implemented in $O(Wk)$  time, and Niagara can be implemented in $O(Wk\log k)$  time.

The core idea of Bit Matcher is that any odd weight of the partition must participate in a transaction of size $1$. After performing these transactions all weights whose second least significant bit is $1$ must participate in a transaction of size $2$  and so on. The order $<_{lex}$ (Definition~\ref{definition_lexicorder}) helps to identify which transactions to make at lower levels such that there will be fewer $1$-bits at higher levels. Loosely speaking,
we choose transactions that
 cancel as many $1$-bits as possible in the binary representation of the weights, using the carry caused by each one of these transaction.
 
A high level overview of Niagara is as follows. 
Consider the target partition $P^0 = (x_1,\ldots,x_k)$. The algorithm maintains an implicit partition $P^1$, such that the vector $P$ in the algorithm satisfies $P = P^0 - P^1$. Initially, when the TCAM's default rule is allocated to target $i$, $P^1 = (0, \ldots, 0, 2^W, 0, \ldots, 0)$ (non-zero in index $i$). Since $P = P^0-P^1$ we have $\sum(P)=0$. Thus while $P \ne (0,\ldots,0)$ it must contain a positive and a negative difference. Let $i$ be a coordinate with maximum (positive) value in $P$ and let $j$ be a coordinate with minimum (negative) value in $P$, then Niagara refines $P$ by computing a value  $\lambda = 2^h$  such that when moving $\lambda$ from $p_i$ to $p_j$, the $L_1$ norm of $P$ following this transaction is minimized.


\begin{algorithm}[ht]
    \SetAlgoLined
    \DontPrintSemicolon
    \KwIn{
          A partition $P = [p_1, \ldots, p_k]$, each $p_i$ is a non-negative integer and $\sum_{i=1}^k p_i =2^W$.
    }
    \KwOut{
        Shortest sequence $s$ of transactions (of
        sizes which are powers of $2$), that zeroes $P$.
    }
    
    \SetKwFunction{funcBitMatcher}{BitMatcher}
    \SetKwFunction{funcNiagara}{Niagara}
    \SetKwProg{Fn}{Function}{:}{} \SetKwProg{Fn}{}{:}{} %\SetKwProg{Fn}{Function}{:}{}
    
    Initialize $s$ to be an empty sequence. Then call either \funcBitMatcher{$P$} or \funcNiagara{$P$}, and \Return $s$.
    \;\;
    
    \Fn{\funcBitMatcher{$P$}}{
        \For{level $\ell = 0 \ldots W-1$} {
            \smallskip
     
            Let $A$ be the set of weights whose $\ell^{\text{th}}$ bit is $1$ (i.e. $x_i\in A$ iff bitwise $x_i\&2^\ell \ne 0$).
    
            \looseness=-1
            Let $A_h$ consists of the $|A|/2$ largest weights in $A$ in bit lexicographic order, and let $A_l$ consists of the $|A|/2$ smallest weights in $A$ in bit lexicographic order.
    
            Pair the elements of $A_h$ and $A_l$ arbitrarily and for each pair append to $s$ and apply to $P$ a transaction of value $2^\ell$ from the smallest weight to the largest weight in the pair.
        }
        Let $i$ be such that $p_i = 2^W$. Add to $s$ the transaction $[i \to_W \bot]$.
    }
    \;
    \Fn{\funcNiagara{$P$}}{
        Let $i = argmax(P)$. Subtract $2^W$ from $p_i$, and add to $s$ the transaction $[i \to_W \bot]$.
    
        \While{$P \ne (0, \ldots, 0)$} {
    	    Let $i = argmax(\Delta)$, $j = argmin(\Delta)$, and let $h$ be the largest integer minimizing $\Big(|p_i-2^h| + |p_j+2^h|\Big)$.
        
            Apply a transaction $[i\rightarrow_h j]$ to $P$ and append it to $s$.
        }
    }
    \caption{Bit Matcher and Niagara Algorithms}
    \label{algorithms_bitmatcher_and_niagara}
\end{algorithm}




%%%###%%%###%%%###%%% \input{section_code_sharing.tex}


\section{Supplementary Code Implementation}
\label{section_code_info}
We provide an implementation of our algorithms as supplementary material for two main purposes:
\begin{enumerate}
    \item Clarify low level details that the reader may find unclear or is curious about. For this purpose, the code includes both comments and test-cases which can be used as additional examples.
    
    \item Allowing any interested party to implement any of the algorithms described easily, in their chosen environment and language, and provide tests for verification.
\end{enumerate}

\noindent
The implementation covers the following in the paper:

\begin{enumerate}
    \item Utilities: bit-lexicographic comparison (Definition~\ref{definition_lexicorder}), partition complexity (Definition~\ref{definition_length_of_partition}), computation of the $\errLinf$, $\errLinfPos$ and $\errLinfPosRel$ distances, and sampling ordered-partitions as described in Section~\ref{section_experiments}.

    \item Lifting solvers: Algorithm~\ref{alg_lift_max_capacity_1}, Algorithm~\ref{alg_lift_capacity_1_2_3} and Algorithm~\ref{alg_lift_one_sided_dualversion}.
    
    \item Partition approximators: reductions from rule-based to error-based approximation (according to the reduction of Theorem~\ref{theorem_equivalent_rule_bound_error_bound1}), and from error-based approximation to a lifting problem (according to Lemma~\ref{theorem_special_case_lifting_reduction} and Lemma~\ref{lemma_reduction_to_one_sided_lifting}).
\end{enumerate}

\noindent
We provide python code for clarity. It allows us to deliver the logic clearly and reduce language-specific implementation details.







%%%###%%%###%%%###%%% \input{section_experiments_supplementary.tex}

\section{Supplementary Experiments}
\label{section_supplementary_experiments}

\subsection{Error as a function of \texorpdfstring{$k$}{k} Targets}
\label{section_experiments_var_k}
In this section we examine the expected $\errLinf$ approximation error as a function of the number of targets $k$. There are two opposite effects to consider. First, the number of rules is fixed so the larger $k$ is, the harder it is to approximate the partition. On the other hand, the average weight in the partition is $\frac{2^W}{k}$ so the larger $k$ is, the weights get smaller and therefore the error should get smaller as well. However, since the error is defined by the maximal error of the targets rather than the average, this latter effect should be weak.
Fig.~\ref{figure_var_k} shows the results for  $W=32$ and $n=25,50,100$. For $k \le 100$, we see
that the error grows with $k$. So the increase in error due to the larger number of targets is more dominant than the decrease in error due to the decrease in the average target size.
Interestingly, the growth is approximately linear, except for small values of $k$
for which we have many zero-error partitions. For $n=25$ the growth is linear when $k \ge 20$, for $n=50$ when $k\ge 40$ and for $n=100$ when $k \ge 80$. The case $n=25$ begins to show growth slowdown, since the error approaches its maximum possible value ($W=32$, and the error already passed $2^{27}$).


\begin{figure}[t]
	%\centering
    \subfigure[$n=25$ Rules.] {
        \hspace*{-1.0em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of targets $k$,
        		ymin=0, ymax = 160,
                ytick={32,64,96,128,160},
                ylabel=$(\text{approx.\ err.}) / 2^{20}$,
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.01,0.99)}, anchor=north west,font=\footnotesize,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black] coordinates{
            (4, 0.000) (5, 0.000) (6, 0.001) (7, 0.006) (8, 0.025) (9, 0.075) (10, 0.184) (11, 0.376) (12, 0.694) (13, 1.165) (14, 1.744) (15, 2.568) (16, 3.546) (17, 4.660) (18, 5.872) (19, 7.711) (20, 9.292) (21, 10.917) (22, 12.987) (23, 15.124) (24, 17.194) (25, 19.514) (26, 21.270) (27, 23.370) (28, 25.707) (29, 27.906) (30, 30.483) (31, 33.143) (32, 35.725) (33, 38.471) (34, 40.324) (35, 42.541) (36, 44.682) (37, 47.117) (38, 49.099) (39, 51.049) (40, 52.418) (41, 54.987) (42, 56.188) (43, 59.531) (44, 60.893) (45, 63.211) (46, 65.749) (47, 67.510) (48, 68.895) (49, 71.632) (50, 73.455) (51, 75.359) (52, 77.116) (53, 79.149) (54, 81.623) (55, 83.416) (56, 86.457) (57, 88.171) (58, 88.829) (59, 90.995) (60, 93.638) (61, 95.821) (62, 96.697) (63, 98.801) (64, 101.033) (65, 102.585) (66, 104.044) (67, 105.569) (68, 106.887) (69, 108.518) (70, 110.642) (71, 111.676) (72, 112.102) (73, 114.511) (74, 116.100) (75, 116.739) (76, 118.520) (77, 119.024) (78, 121.080) (79, 121.400) (80, 123.217) (81, 123.723) (82, 124.604) (83, 126.482) (84, 127.274) (85, 128.371) (86, 130.427) (87, 130.289) (88, 131.685) (89, 132.892) (90, 133.769) (91, 134.775) (92, 135.716) (93, 136.642) (94, 136.771) (95, 138.313) (96, 139.145) (97, 139.888) (98, 141.111) (99, 141.090) (100, 142.006)
            }; %\addlegendentry{$n=25$ rules} 
            
        \end{axis}
    \end{tikzpicture} 
    \label{figure_var_k_sub1}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$n=50$ Rules.] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of targets $k$,
        		ymin=0, ymax = 40,
                ytick={8,16,24,32,40},
                % ylabel=$(\text{approx.\ err.}) / 2^{20}$, % rely on the other figure
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black] coordinates{
            (4, 0.000) (5, 0.000) (6, 0.000) (7, 0.000) (8, 0.000) (9, 0.000) (10, 0.000) (11, 0.000) (12, 0.000) (13, 0.001) (14, 0.002) (15, 0.004) (16, 0.008) (17, 0.015) (18, 0.026) (19, 0.042) (20, 0.068) (21, 0.100) (22, 0.148) (23, 0.207) (24, 0.274) (25, 0.354) (26, 0.463) (27, 0.602) (28, 0.757) (29, 0.899) (30, 1.092) (31, 1.314) (32, 1.543) (33, 1.821) (34, 2.086) (35, 2.398) (36, 2.703) (37, 3.053) (38, 3.416) (39, 3.842) (40, 4.184) (41, 4.669) (42, 5.025) (43, 5.621) (44, 6.153) (45, 6.535) (46, 7.120) (47, 7.664) (48, 8.174) (49, 8.748) (50, 9.107) (51, 9.780) (52, 10.364) (53, 10.862) (54, 11.383) (55, 12.044) (56, 12.532) (57, 13.113) (58, 13.578) (59, 14.261) (60, 14.972) (61, 15.560) (62, 16.163) (63, 16.827) (64, 17.266) (65, 17.778) (66, 18.488) (67, 19.328) (68, 19.590) (69, 20.067) (70, 20.668) (71, 21.086) (72, 21.849) (73, 22.314) (74, 22.756) (75, 23.387) (76, 23.828) (77, 24.175) (78, 24.821) (79, 25.354) (80, 25.750) (81, 26.260) (82, 26.818) (83, 26.990) (84, 27.863) (85, 28.348) (86, 28.919) (87, 29.619) (88, 29.814) (89, 30.329) (90, 31.311) (91, 31.317) (92, 32.248) (93, 32.597) (94, 33.454) (95, 33.851) (96, 34.428) (97, 35.158) (98, 35.679) (99, 36.231) (100, 36.777)
            }; %\addlegendentry{$n=50$ rules} 
            
        \end{axis}
    \end{tikzpicture}
    \label{figure_var_k_sub2}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$n=100$ Rules.] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of targets $k$,
        		ymin=0, ymax = 5,
                ytick={1,2,3,4,5},
                % ylabel=$(\text{approx.\ err.}) / 2^{20}$, % rely on the other figure
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.01,0.99)}, anchor=north west,font=\footnotesize,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black] coordinates{
            (4, 0.000) (5, 0.000) (6, 0.000) (7, 0.000) (8, 0.000) (9, 0.000) (10, 0.000) (11, 0.000) (12, 0.000) (13, 0.000) (14, 0.000) (15, 0.000) (16, 0.000) (17, 0.000) (18, 0.000) (19, 0.000) (20, 0.000) (21, 0.000) (22, 0.000) (23, 0.000) (24, 0.000) (25, 0.000) (26, 0.000) (27, 0.000) (28, 0.001) (29, 0.001) (30, 0.001) (31, 0.002) (32, 0.003) (33, 0.004) (34, 0.006) (35, 0.008) (36, 0.010) (37, 0.013) (38, 0.017) (39, 0.022) (40, 0.028) (41, 0.034) (42, 0.043) (43, 0.051) (44, 0.060) (45, 0.075) (46, 0.086) (47, 0.103) (48, 0.120) (49, 0.135) (50, 0.160) (51, 0.182) (52, 0.209) (53, 0.234) (54, 0.264) (55, 0.293) (56, 0.336) (57, 0.374) (58, 0.412) (59, 0.455) (60, 0.502) (61, 0.549) (62, 0.600) (63, 0.657) (64, 0.718) (65, 0.762) (66, 0.844) (67, 0.908) (68, 0.961) (69, 1.053) (70, 1.118) (71, 1.189) (72, 1.248) (73, 1.351) (74, 1.425) (75, 1.517) (76, 1.609) (77, 1.667) (78, 1.801) (79, 1.877) (80, 1.972) (81, 2.072) (82, 2.185) (83, 2.307) (84, 2.421) (85, 2.528) (86, 2.703) (87, 2.818) (88, 2.916) (89, 3.084) (90, 3.151) (91, 3.324) (92, 3.449) (93, 3.542) (94, 3.691) (95, 3.832) (96, 3.956) (97, 4.086) (98, 4.201) (99, 4.388) (100, 4.505)
            }; % \addlegendentry{$n=100$ rules}
            
        \end{axis}
    \end{tikzpicture}
    \label{figure_var_k_sub3}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \caption{Expected $\errLinf$ approximation error as a function of the number of targets $k \in [4,100]$, for  $W=32$ and $n=25,50,100$ rules.
    \label{figure_var_k}}
\end{figure}


\subsection{Error as a function of Width \texorpdfstring{$W$}{W}}
\label{section_experiments_var_W}
In this section we examine the expected $\errLinf$ approximation error as a function of the address-width $W$. We expect the error to grow exponentially in proportion to $2^W$, because increasing $W$ by $1$ doubles the average weight, and therefore is likely to double the expected error because everything scales-up by a factor of $2$.
Fig.~\ref{figure_var_W} shows the results in logarithmic scale, for fixed values $k=10$ and $n=25,50$. As expected, the slopes are almost $1$: $1.0014$ (for $k=10,n=25$) and $1.0076$ (for $k=10,n=50$). The graphs are almost parallel and $n=50$ is lower, because more rules yield lower error. The slopes are not exactly $1$ since they  also depend  weakly on $n$ and $k$.

\begin{figure}[t]%[!ht]
	\centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.45\textwidth,
    		height=0.17\textwidth,
    		xmin=10,
    		xmax=50,
    		xtick={10,20,30,40,50},
    		xlabel=Addresses width $W$,
    		ymin=0,
            ymax = 40,
            ytick={-10,0,10,20,30,40},
            ylabel=$\lg(\text{approx. err.})$,
    		legend style={at={(0.01,0.99)}, anchor=north west,font=\footnotesize,},
    		label style={font=\footnotesize},
    		grid=both
        ]
        
        \addplot [black,mark=o] coordinates{ (50, 35.573) }; \addlegendentry{$n=25$ rules}
        \addplot [black,mark=*] coordinates{ (50, 21.892) }; \addlegendentry{$n=50$ rules}
        
         \addplot [black,mark=.] coordinates{
            (12, -6.644) (13, -2.708) (14, -0.651) (15, 0.485) (16, 1.517) (17, 2.478) (18, 3.588) (19, 4.528) (20, 5.569) (21, 6.561) (22, 7.524) (23, 8.518) (24, 9.547) (25, 10.586) (26, 11.511) (27, 12.536) (28, 13.614) (29, 14.597) (30, 15.550) (31, 16.549) (32, 17.532) (33, 18.561) (34, 19.535) (35, 20.551) (36, 21.527) (37, 22.491) (38, 23.589) (39, 24.543) (40, 25.551) (41, 26.516) (42, 27.525) (43, 28.537) (44, 29.581) (45, 30.592) (46, 31.564) (47, 32.480) (48, 33.577) (49, 34.546) (50, 35.573)
         }; % naked \addlegendentry{$n=25$ rules} 
     		
        \addplot [black,mark=.] coordinates{
            (25, -6.506) (26, -3.626) (27, -1.680) (28, -0.304) (29, 0.874) (30, 1.980) (31, 2.884) (32, 3.947) (33, 4.872) (34, 5.938) (35, 6.936) (36, 7.994) (37, 8.829) (38, 9.929) (39, 10.863) (40, 11.921) (41, 12.951) (42, 13.921) (43, 14.980) (44, 15.843) (45, 16.925) (46, 17.884) (47, 18.939) (48, 19.925) (49, 20.900) (50, 21.892)
         }; % naked \addlegendentry{$n=50$ rules}
     		
        \end{axis}
    \end{tikzpicture}
     \caption{Expected $\errLinf$ approximation error (log-scale) as a function of the address size $W \in [10,50]$, for fixed $k=10$ targets and $n=25,50$ rules. \label{figure_var_W}}
\end{figure}

\subsection{Error vs.\ fixed Rules per Target Ratio}
\label{subsection_experiments_ratio_nk}
In this section we examine the expected $\errLinf$ approximation error as a function of the number of targets $k$, 
where the number of rules is proportional to the number of targets, that is $n=ck$ for some constant $c$.
This setting represents the scenario in which we are willing to allocate a TCAM table of size that is proportional to the number of targets.
We expect the error to decrease as $k$ (and $n$) increases. The reason is that we have freedom to use the additional rules to decrease large weights and reduce error.

Most of the simulations in this paper consider moderate values of $n$ and $k$. In this section we not only consider moderate values (Fig.~\ref{figure_var_ratio_nk}) but also consider the ratio for a very large number of targets (Fig.~\ref{figure_var_ratio_nk_large}), in the order of $1K {-} 10K$, to show that the behaviour of the error is mostly affected by the average number of rules per target rather than some absolute quantity.

Fig.~\ref{figure_var_ratio_nk} shows the data for various ratios $n/k=0.5,\ldots,5.5$ and $W=32$. When $n/k=5$ the error is typically zero, so there was no point to proceed to higher ratios ($n/k=5.5$ emphasizes that). We also plot the error with one rule ($n=1$) to provide a baseline. Although the average weight decreases proportionally to $\frac{2^W}{k}$, a single rule only deals with the maximum weight, and it is not sufficient to provide any significant reduction in the error.

The relation which we see is an inverse-power law, meaning that the error is proportional to $k^{-\alpha}$ for some power $\alpha > 0$. The graph is in log-log scale to emphasize the linearity of the relation $\lg err \approx -\alpha \cdot \lg k + const$.
Although it may look like parallel slopes, it actually steepens slightly as $n/k$ grows, so $\alpha$ depends on $n/k$. Moreover, $const$ also depends on $n/k$. Factoring this into account, the numeric relation we get from this data is close to $\lg err = -(0.16(n/k) + 0.91) \lg k + (34.24-4.92(n/k))$. The constant $34.24$ is most likely in part due to $W$ (which is $32$ in this experiment), since we know the error is exponential in $W$ (Section~\ref{section_experiments_var_W}).
Replacing $34.24$ by $W+ 2.24$ we get:
\begin{equation}
\label{equation_empiric}
	    \mathbb{E}[\errLinf \text{\ error}] = 2^{W - 4.92 \cdot (n/k) + 2.24} \cdot k^{-(0.16 (n/k) + 0.91)}
\end{equation}
The ``magic'' constants in Equation~(\ref{equation_empiric}) probably result from a more intricate dependence of the error on $n$, $k$, and $W$.

The way to interpret Equation~(\ref{equation_empiric}) is as follows: The error grows 
exponentially (base $2$) with the width $W$. For a fixed $k$, it drops exponentially with $n$. The dependence on $k$ is more complex: When $k \le n$ the ratio $n/k$ is rapidly dropping as $k$ grows, causing a quick growth in the error. When $k \ge n$, although the base grows with $k$ and the power is negative, the exponent still drops slowly as $k$ grows ($n/k \in (0,1)$). This produces a moderate error-growth that seems linear in Fig.~\ref{figure_var_k}, until the change in $n/k$ becomes so small that the growth of the base $k$ takes effect and slows the error-growth.

Using Equation~(\ref{equation_empiric}) we can derive the exponential dependence of the error as a function of $n$, per Section~\ref{section_experiments_var_n}: $\lg err = An+B$ where $A(k) = -\frac{4.92 + 0.16 \lg k}{k}$ and $B(k,W) = W+2.24- 0.91 \lg k$. The data in Section~\ref{section_experiments_var_n} for $k=5,10,11,20$ highly agrees with these expressions; $A(k)$ deviates by at most $2.2\%$, and $B(k,32)$ deviates by at most $0.5\%$.

Equation~(\ref{equation_empiric}) can also be used to revisit the graphs in Section~\ref{section_experiments_var_k}. It produces pretty accurate curves for $n=50,100$ (Fig.~\ref{figure_var_k_sub2}-\ref{figure_var_k_sub3}), less than $8\%$ deviation from the computed data. However, for $n=25$ (Fig.~\ref{figure_var_k_sub1}) the 
error predicted by Equation~(\ref{equation_empiric})
deviates from the computed data for $k\ge 2n$ (deviation goes up to $30\%$), though still qualitatively exhibiting the slowdown, when the base $k$ becomes more important than the exponent $n/k$. A visual plot of Equation~(\ref{equation_empiric}) against the graphs from Section~\ref{section_experiments_var_k} is provided in Fig.~\ref{figure_var_k_and_equation_plot}.

Fig.~\ref{figure_var_ratio_nk_large} augments the analysis for large values of $k$, in multiples of $1000$ up to $20000$, for the ratios $n/k=1,2,3,4$. Due to the large values of $k$,  we obtained each data-point by averaging the error for 100 sampled partitions (rather than 1000 as in our other experiments). It is clear that for a very large number of targets, about $4$ rules on average per target are enough for almost no error. We note that the slopes of the trend lines that were discussed in the previous paragraphs for $k \in [4,100]$ are not accurate for larger $k$. For large $k$ the slope is smaller. For instance, for $n/k=2$ the trend-line for large $k$ is $\lg(error) = -1.0635 \lg(k) + 23.434$, compared to $\lg(error) = -1.2259 \lg(k) + 24.285$ when $k \le 100$ is considered. It could be that indeed the slope is not constant and decreases with $k$ or, possibly, the fact that the parameters ($k$, $W$, $n$) of the problem are discrete makes it less suitable to represent this (discrete) function by a (continuous) line.


\begin{figure}[!t]%[!ht]
	\centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.4\textwidth,
    		height=0.3\textwidth,
    		xmin=1,
    		xmax=7,
    		xtick={2,3,4,5,6},
    		xlabel=$\lg(k)$ (log of number of targets),
    		ymin=0,
            ymax=33,
            ytick={0,4,8,12,16,20,24,28,32},
            ylabel=$\lg(\text{approx. err.})$,
    		legend style={at={(0.99,0.99)}, anchor=north west,font=\footnotesize,},
    		label style={font=\footnotesize},
    		grid=both
        ]
    		
    	\addplot [black,mark=*] coordinates{ (2.000, 30.948) }; \addlegendentry{$n=1$}
    	\addplot [black,mark=.] coordinates{ (2.000, 29.486) }; \addlegendentry{$n=0.5k$}
    	\addplot [black,mark=+] coordinates{ (2.000, 27.037) }; \addlegendentry{$n=1.0k$}
    	\addplot [black,mark=.] coordinates{ (2.000, 24.506) }; \addlegendentry{$n=1.5k$}
    	\addplot [black,mark=o] coordinates{ (2.000, 22.019) }; \addlegendentry{$n=2.0k$}
    	\addplot [black,mark=.] coordinates{ (2.000, 19.416) }; \addlegendentry{$n=2.5k$}
    	\addplot [black,mark=square] coordinates{ (2.000, 16.904) }; \addlegendentry{$n=3.0k$}
    	\addplot [black,mark=.] coordinates{ (2.000,14.391) }; \addlegendentry{$n=3.5k$}
        \addplot [black,mark=diamond] coordinates{ (2.000,11.857) }; \addlegendentry{$n=4.0k$}
        \addplot [black,mark=.] coordinates{ (2.000,9.183) }; \addlegendentry{$n=4.5k$}
        \addplot [black,mark=triangle] coordinates{ (2.000,6.818) }; \addlegendentry{$n=5.0k$}
        \addplot [black,mark=.] coordinates{ (2.000,4.198) }; \addlegendentry{$n=5.5k$}
            
    	\addplot [black,mark=.] coordinates{
            (2.000, 30.948) (2.322, 31.115) (2.585, 31.241) (2.807, 31.334) (3.000, 31.399) (3.170, 31.455) (3.322, 31.507) (3.459, 31.529) (3.585, 31.568) (3.700, 31.591) (3.807, 31.621) (3.907, 31.636) (4.000, 31.661) (4.087, 31.671) (4.170, 31.690) (4.248, 31.703) (4.322, 31.716) (4.392, 31.723) (4.459, 31.736) (4.524, 31.741) (4.585, 31.754) (4.644, 31.760) (4.700, 31.770) (4.755, 31.774) (4.807, 31.779) (4.858, 31.789) (4.907, 31.788) (4.954, 31.803) (5.000, 31.806) (5.044, 31.812) (5.087, 31.815) (5.129, 31.817) (5.170, 31.825) (5.209, 31.825) (5.248, 31.830) (5.285, 31.834) (5.322, 31.840) (5.358, 31.841) (5.392, 31.842) (5.426, 31.845) (5.459, 31.849) (5.492, 31.851) (5.524, 31.854) (5.555, 31.857) (5.585, 31.859) (5.615, 31.863) (5.644, 31.863) (5.672, 31.867) (5.700, 31.868) (5.728, 31.871) (5.755, 31.874) (5.781, 31.873) (5.807, 31.876) (5.833, 31.879) (5.858, 31.881) (5.883, 31.882) (5.907, 31.881) (5.931, 31.883) (5.954, 31.885) (5.977, 31.888) (6.000, 31.887) (6.022, 31.891) (6.044, 31.892) (6.066, 31.892) (6.087, 31.895) (6.109, 31.896) (6.129, 31.896) (6.150, 31.898) (6.170, 31.899) (6.190, 31.900) (6.209, 31.902) (6.229, 31.903) (6.248, 31.905) (6.267, 31.904) (6.285, 31.905) (6.304, 31.906) (6.322, 31.908) (6.340, 31.907) (6.358, 31.910) (6.375, 31.911) (6.392, 31.911) (6.409, 31.911) (6.426, 31.914) (6.443, 31.913) (6.459, 31.915) (6.476, 31.915) (6.492, 31.916) (6.508, 31.917) (6.524, 31.919) (6.539, 31.919) (6.555, 31.919) (6.570, 31.920) (6.585, 31.922) (6.600, 31.922) (6.615, 31.921) (6.629, 31.923) (6.644, 31.924)
        }; \label{plot_c0_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 29.486) (2.322, 29.711) (2.585, 29.170) (2.807, 29.358) (3.000, 28.615) (3.170, 28.768) (3.322, 28.456) (3.459, 28.581) (3.585, 28.243) (3.700, 28.352) (3.807, 27.945) (3.907, 28.060) (4.000, 27.697) (4.087, 27.758) (4.170, 27.595) (4.248, 27.672) (4.322, 27.505) (4.392, 27.575) (4.459, 27.411) (4.524, 27.464) (4.585, 27.248) (4.644, 27.332) (4.700, 27.099) (4.755, 27.185) (4.807, 26.926) (4.858, 26.989) (4.907, 26.801) (4.954, 26.835) (5.000, 26.721) (5.044, 26.763) (5.087, 26.682) (5.129, 26.724) (5.170, 26.647) (5.209, 26.681) (5.248, 26.584) (5.285, 26.636) (5.322, 26.549) (5.358, 26.587) (5.392, 26.501) (5.426, 26.529) (5.459, 26.441) (5.492, 26.477) (5.524, 26.359) (5.555, 26.414) (5.585, 26.289) (5.615, 26.306) (5.644, 26.203) (5.672, 26.240) (5.700, 26.099) (5.728, 26.155) (5.755, 25.998) (5.781, 26.023) (5.807, 25.914) (5.833, 25.951) (5.858, 25.849) (5.883, 25.870) (5.907, 25.792) (5.931, 25.810) (5.954, 25.763) (5.977, 25.780) (6.000, 25.728) (6.022, 25.761) (6.044, 25.717) (6.066, 25.739) (6.087, 25.710) (6.109, 25.724) (6.129, 25.691) (6.150, 25.707) (6.170, 25.673) (6.190, 25.689) (6.209, 25.651) (6.229, 25.664) (6.248, 25.630) (6.267, 25.647) (6.285, 25.607) (6.304, 25.625) (6.322, 25.585) (6.340, 25.601) (6.358, 25.554) (6.375, 25.585) (6.392, 25.529) (6.409, 25.556) (6.426, 25.500) (6.443, 25.530) (6.459, 25.462) (6.476, 25.486) (6.492, 25.436) (6.508, 25.460) (6.524, 25.406) (6.539, 25.416) (6.555, 25.343) (6.570, 25.387) (6.585, 25.300) (6.600, 25.333) (6.615, 25.261) (6.629, 25.270) (6.644, 25.201)
        }; \label{plot_c0_5_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 27.037) (2.322, 26.695) (2.585, 26.487) (2.807, 26.218) (3.000, 25.985) (3.170, 25.889) (3.322, 25.699) (3.459, 25.535) (3.585, 25.426) (3.700, 25.286) (3.807, 25.170) (3.907, 25.048) (4.000, 24.924) (4.087, 24.892) (4.170, 24.773) (4.248, 24.664) (4.322, 24.622) (4.392, 24.531) (4.459, 24.439) (4.524, 24.388) (4.585, 24.330) (4.644, 24.272) (4.700, 24.211) (4.755, 24.137) (4.807, 24.101) (4.858, 24.044) (4.907, 23.988) (4.954, 23.953) (5.000, 23.871) (5.044, 23.831) (5.087, 23.785) (5.129, 23.719) (5.170, 23.679) (5.209, 23.651) (5.248, 23.585) (5.285, 23.549) (5.322, 23.507) (5.358, 23.481) (5.392, 23.439) (5.426, 23.405) (5.459, 23.386) (5.492, 23.339) (5.524, 23.323) (5.555, 23.298) (5.585, 23.256) (5.615, 23.238) (5.644, 23.216) (5.672, 23.172) (5.700, 23.141) (5.728, 23.109) (5.755, 23.098) (5.781, 23.062) (5.807, 23.025) (5.833, 23.000) (5.858, 22.973) (5.883, 22.953) (5.907, 22.938) (5.931, 22.889) (5.954, 22.889) (5.977, 22.846) (6.000, 22.803) (6.022, 22.780) (6.044, 22.765) (6.066, 22.741) (6.087, 22.719) (6.109, 22.677) (6.129, 22.661) (6.150, 22.662) (6.170, 22.632) (6.190, 22.602) (6.209, 22.579) (6.229, 22.551) (6.248, 22.548) (6.267, 22.523) (6.285, 22.497) (6.304, 22.491) (6.322, 22.473) (6.340, 22.457) (6.358, 22.426) (6.375, 22.420) (6.392, 22.409) (6.409, 22.384) (6.426, 22.379) (6.443, 22.347) (6.459, 22.350) (6.476, 22.312) (6.492, 22.317) (6.508, 22.295) (6.524, 22.283) (6.539, 22.262) (6.555, 22.245) (6.570, 22.229) (6.585, 22.224) (6.600, 22.207) (6.615, 22.189) (6.629, 22.191) (6.644, 22.167)
        }; \label{plot_c1_0_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 24.506) (2.322, 24.716) (2.585, 23.858) (2.807, 24.025) (3.000, 23.378) (3.170, 23.470) (3.322, 22.960) (3.459, 23.079) (3.585, 22.674) (3.700, 22.740) (3.807, 22.370) (3.907, 22.490) (4.000, 22.186) (4.087, 22.252) (4.170, 21.972) (4.248, 22.019) (4.322, 21.767) (4.392, 21.832) (4.459, 21.646) (4.524, 21.667) (4.585, 21.443) (4.644, 21.515) (4.700, 21.333) (4.755, 21.420) (4.807, 21.196) (4.858, 21.256) (4.907, 21.116) (4.954, 21.157) (5.000, 21.003) (5.044, 21.054) (5.087, 20.913) (5.129, 20.929) (5.170, 20.813) (5.209, 20.821) (5.248, 20.717) (5.285, 20.776) (5.322, 20.651) (5.358, 20.658) (5.392, 20.558) (5.426, 20.583) (5.459, 20.482) (5.492, 20.501) (5.524, 20.409) (5.555, 20.424) (5.585, 20.331) (5.615, 20.371) (5.644, 20.272) (5.672, 20.306) (5.700, 20.221) (5.728, 20.242) (5.755, 20.118) (5.781, 20.181) (5.807, 20.084) (5.833, 20.103) (5.858, 20.036) (5.883, 20.066) (5.907, 19.991) (5.931, 19.989) (5.954, 19.932) (5.977, 19.927) (6.000, 19.883) (6.022, 19.919) (6.044, 19.833) (6.066, 19.869) (6.087, 19.779) (6.109, 19.813) (6.129, 19.755) (6.150, 19.756) (6.170, 19.698) (6.190, 19.704) (6.209, 19.638) (6.229, 19.663) (6.248, 19.616) (6.267, 19.629) (6.285, 19.569) (6.304, 19.619) (6.322, 19.532) (6.340, 19.547) (6.358, 19.494) (6.375, 19.510) (6.392, 19.460) (6.409, 19.471) (6.426, 19.435) (6.443, 19.428) (6.459, 19.384) (6.476, 19.407) (6.492, 19.343) (6.508, 19.380) (6.524, 19.318) (6.539, 19.311) (6.555, 19.271) (6.570, 19.295) (6.585, 19.258) (6.600, 19.254) (6.615, 19.213) (6.629, 19.232) (6.644, 19.175)
        }; \label{plot_c1_5_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 22.019) (2.322, 21.631) (2.585, 21.267) (2.807, 20.928) (3.000, 20.656) (3.170, 20.471) (3.322, 20.215) (3.459, 20.127) (3.585, 19.899) (3.700, 19.730) (3.807, 19.622) (3.907, 19.477) (4.000, 19.338) (4.087, 19.216) (4.170, 19.163) (4.248, 19.054) (4.322, 18.923) (4.392, 18.852) (4.459, 18.790) (4.524, 18.678) (4.585, 18.609) (4.644, 18.538) (4.700, 18.457) (4.755, 18.449) (4.807, 18.357) (4.858, 18.274) (4.907, 18.205) (4.954, 18.161) (5.000, 18.090) (5.044, 18.042) (5.087, 17.995) (5.129, 17.960) (5.170, 17.908) (5.209, 17.879) (5.248, 17.814) (5.285, 17.752) (5.322, 17.722) (5.358, 17.666) (5.392, 17.647) (5.426, 17.627) (5.459, 17.546) (5.492, 17.521) (5.524, 17.482) (5.555, 17.466) (5.585, 17.420) (5.615, 17.392) (5.644, 17.328) (5.672, 17.308) (5.700, 17.287) (5.728, 17.249) (5.755, 17.216) (5.781, 17.183) (5.807, 17.157) (5.833, 17.127) (5.858, 17.114) (5.883, 17.072) (5.907, 17.059) (5.931, 17.000) (5.954, 16.967) (5.977, 16.956) (6.000, 16.936) (6.022, 16.917) (6.044, 16.870) (6.066, 16.863) (6.087, 16.826) (6.109, 16.834) (6.129, 16.805) (6.150, 16.778) (6.170, 16.707) (6.190, 16.706) (6.209, 16.687) (6.229, 16.678) (6.248, 16.667) (6.267, 16.632) (6.285, 16.634) (6.304, 16.613) (6.322, 16.564) (6.340, 16.547) (6.358, 16.543) (6.375, 16.535) (6.392, 16.484) (6.409, 16.464) (6.426, 16.468) (6.443, 16.458) (6.459, 16.438) (6.476, 16.421) (6.492, 16.390) (6.508, 16.375) (6.524, 16.356) (6.539, 16.340) (6.555, 16.329) (6.570, 16.298) (6.585, 16.316) (6.600, 16.279) (6.615, 16.266) (6.629, 16.240) (6.644, 16.226)
        }; \label{plot_c2_0_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 19.416) (2.322, 19.476) (2.585, 18.624) (2.807, 18.695) (3.000, 17.985) (3.170, 18.038) (3.322, 17.509) (3.459, 17.605) (3.585, 17.160) (3.700, 17.227) (3.807, 16.845) (3.907, 16.876) (4.000, 16.610) (4.087, 16.601) (4.170, 16.329) (4.248, 16.348) (4.322, 16.102) (4.392, 16.144) (4.459, 15.932) (4.524, 15.965) (4.585, 15.723) (4.644, 15.783) (4.700, 15.601) (4.755, 15.693) (4.807, 15.474) (4.858, 15.471) (4.907, 15.334) (4.954, 15.350) (5.000, 15.210) (5.044, 15.233) (5.087, 15.070) (5.129, 15.125) (5.170, 14.981) (5.209, 15.027) (5.248, 14.928) (5.285, 14.975) (5.322, 14.842) (5.358, 14.845) (5.392, 14.726) (5.426, 14.772) (5.459, 14.616) (5.492, 14.694) (5.524, 14.581) (5.555, 14.631) (5.585, 14.500) (5.615, 14.530) (5.644, 14.401) (5.672, 14.426) (5.700, 14.350) (5.728, 14.407) (5.755, 14.308) (5.781, 14.294) (5.807, 14.236) (5.833, 14.258) (5.858, 14.162) (5.883, 14.182) (5.907, 14.099) (5.931, 14.115) (5.954, 14.044) (5.977, 14.056) (6.000, 13.978) (6.022, 14.004) (6.044, 13.957) (6.066, 13.944) (6.087, 13.900) (6.109, 13.886) (6.129, 13.830) (6.150, 13.851) (6.170, 13.802) (6.190, 13.815) (6.209, 13.758) (6.229, 13.778) (6.248, 13.714) (6.267, 13.728) (6.285, 13.654) (6.304, 13.674) (6.322, 13.628) (6.340, 13.615) (6.358, 13.585) (6.375, 13.586) (6.392, 13.556) (6.409, 13.573) (6.426, 13.514) (6.443, 13.525) (6.459, 13.471) (6.476, 13.505) (6.492, 13.432) (6.508, 13.452) (6.524, 13.411) (6.539, 13.407) (6.555, 13.375) (6.570, 13.369) (6.585, 13.356) (6.600, 13.350) (6.615, 13.305) (6.629, 13.307) (6.644, 13.275)
        }; \label{plot_c2_5_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 16.904) (2.322, 16.443) (2.585, 16.022) (2.807, 15.632) (3.000, 15.346) (3.170, 15.101) (3.322, 14.830) (3.459, 14.601) (3.585, 14.445) (3.700, 14.213) (3.807, 14.068) (3.907, 13.930) (4.000, 13.773) (4.087, 13.605) (4.170, 13.460) (4.248, 13.429) (4.322, 13.259) (4.392, 13.191) (4.459, 13.087) (4.524, 13.034) (4.585, 12.919) (4.644, 12.834) (4.700, 12.729) (4.755, 12.650) (4.807, 12.594) (4.858, 12.544) (4.907, 12.457) (4.954, 12.391) (5.000, 12.336) (5.044, 12.242) (5.087, 12.202) (5.129, 12.189) (5.170, 12.105) (5.209, 12.058) (5.248, 12.011) (5.285, 11.994) (5.322, 11.909) (5.358, 11.858) (5.392, 11.800) (5.426, 11.747) (5.459, 11.722) (5.492, 11.693) (5.524, 11.614) (5.555, 11.620) (5.585, 11.595) (5.615, 11.527) (5.644, 11.499) (5.672, 11.481) (5.700, 11.452) (5.728, 11.396) (5.755, 11.361) (5.781, 11.330) (5.807, 11.271) (5.833, 11.271) (5.858, 11.238) (5.883, 11.196) (5.907, 11.169) (5.931, 11.123) (5.954, 11.110) (5.977, 11.072) (6.000, 11.037) (6.022, 11.032) (6.044, 10.995) (6.066, 10.986) (6.087, 10.975) (6.109, 10.928) (6.129, 10.855) (6.150, 10.855) (6.170, 10.815) (6.190, 10.803) (6.209, 10.791) (6.229, 10.760) (6.248, 10.753) (6.267, 10.740) (6.285, 10.723) (6.304, 10.675) (6.322, 10.638) (6.340, 10.643) (6.358, 10.650) (6.375, 10.584) (6.392, 10.603) (6.409, 10.590) (6.426, 10.516) (6.443, 10.526) (6.459, 10.523) (6.476, 10.493) (6.492, 10.470) (6.508, 10.477) (6.524, 10.431) (6.539, 10.435) (6.555, 10.418) (6.570, 10.380) (6.585, 10.355) (6.600, 10.322) (6.615, 10.368) (6.629, 10.301) (6.644, 10.301)
        }; \label{plot_c3_0_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 14.391) (2.322, 14.259) (2.585, 13.353) (2.807, 13.412) (3.000, 12.713) (3.170, 12.679) (3.322, 12.116) (3.459, 12.119) (3.585, 11.684) (3.700, 11.699) (3.807, 11.263) (3.907, 11.307) (4.000, 10.993) (4.087, 10.999) (4.170, 10.669) (4.248, 10.699) (4.322, 10.465) (4.392, 10.503) (4.459, 10.250) (4.524, 10.248) (4.585, 10.042) (4.644, 10.044) (4.700, 9.892) (4.755, 9.879) (4.807, 9.720) (4.858, 9.754) (4.907, 9.578) (4.954, 9.590) (5.000, 9.472) (5.044, 9.507) (5.087, 9.277) (5.129, 9.376) (5.170, 9.169) (5.209, 9.231) (5.248, 9.094) (5.285, 9.104) (5.322, 9.012) (5.358, 9.002) (5.392, 8.870) (5.426, 8.925) (5.459, 8.803) (5.492, 8.823) (5.524, 8.734) (5.555, 8.751) (5.585, 8.670) (5.615, 8.686) (5.644, 8.591) (5.672, 8.570) (5.700, 8.487) (5.728, 8.507) (5.755, 8.440) (5.781, 8.460) (5.807, 8.338) (5.833, 8.391) (5.858, 8.280) (5.883, 8.302) (5.907, 8.211) (5.931, 8.280) (5.954, 8.157) (5.977, 8.156) (6.000, 8.100) (6.022, 8.141) (6.044, 8.048) (6.066, 8.059) (6.087, 8.011) (6.109, 8.013) (6.129, 7.976) (6.150, 7.960) (6.170, 7.902) (6.190, 7.887) (6.209, 7.844) (6.229, 7.855) (6.248, 7.802) (6.267, 7.845) (6.285, 7.779) (6.304, 7.783) (6.322, 7.741) (6.340, 7.740) (6.358, 7.694) (6.375, 7.681) (6.392, 7.650) (6.409, 7.646) (6.426, 7.605) (6.443, 7.599) (6.459, 7.546) (6.476, 7.562) (6.492, 7.528) (6.508, 7.521) (6.524, 7.469) (6.539, 7.513) (6.555, 7.449) (6.570, 7.454) (6.585, 7.409) (6.600, 7.412) (6.615, 7.402) (6.629, 7.416) (6.644, 7.340)
        }; \label{plot_c3_5_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 11.857) (2.322, 11.389) (2.585, 10.740) (2.807, 10.311) (3.000, 10.031) (3.170, 9.697) (3.322, 9.390) (3.459, 9.084) (3.585, 8.867) (3.700, 8.641) (3.807, 8.531) (3.907, 8.358) (4.000, 8.135) (4.087, 8.009) (4.170, 7.810) (4.248, 7.764) (4.322, 7.614) (4.392, 7.493) (4.459, 7.410) (4.524, 7.271) (4.585, 7.185) (4.644, 7.116) (4.700, 7.025) (4.755, 6.888) (4.807, 6.823) (4.858, 6.771) (4.907, 6.717) (4.954, 6.625) (5.000, 6.561) (5.044, 6.489) (5.087, 6.434) (5.129, 6.355) (5.170, 6.280) (5.209, 6.219) (5.248, 6.163) (5.285, 6.130) (5.322, 6.073) (5.358, 5.983) (5.392, 6.009) (5.426, 5.928) (5.459, 5.918) (5.492, 5.824) (5.524, 5.796) (5.555, 5.754) (5.585, 5.739) (5.615, 5.684) (5.644, 5.685) (5.672, 5.587) (5.700, 5.574) (5.728, 5.505) (5.755, 5.491) (5.781, 5.467) (5.807, 5.427) (5.833, 5.390) (5.858, 5.349) (5.883, 5.329) (5.907, 5.293) (5.931, 5.242) (5.954, 5.226) (5.977, 5.215) (6.000, 5.181) (6.022, 5.143) (6.044, 5.124) (6.066, 5.071) (6.087, 5.063) (6.109, 5.029) (6.129, 5.014) (6.150, 4.997) (6.170, 4.937) (6.190, 4.946) (6.209, 4.926) (6.229, 4.896) (6.248, 4.867) (6.267, 4.824) (6.285, 4.779) (6.304, 4.813) (6.322, 4.750) (6.340, 4.762) (6.358, 4.709) (6.375, 4.679) (6.392, 4.675) (6.409, 4.646) (6.426, 4.632) (6.443, 4.626) (6.459, 4.629) (6.476, 4.591) (6.492, 4.576) (6.508, 4.525) (6.524, 4.511) (6.539, 4.492) (6.555, 4.503) (6.570, 4.478) (6.585, 4.439) (6.600, 4.417) (6.615, 4.424) (6.629, 4.393) (6.644, 4.395)
        }; \label{plot_c4_0_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 9.183) (2.322, 9.247) (2.585, 8.138) (2.807, 8.229) (3.000, 7.337) (3.170, 7.283) (3.322, 6.586) (3.459, 6.612) (3.585, 6.132) (3.700, 6.145) (3.807, 5.749) (3.907, 5.700) (4.000, 5.328) (4.087, 5.321) (4.170, 5.052) (4.248, 5.108) (4.322, 4.839) (4.392, 4.818) (4.459, 4.540) (4.524, 4.609) (4.585, 4.282) (4.644, 4.281) (4.700, 4.075) (4.755, 4.178) (4.807, 4.020) (4.858, 4.014) (4.907, 3.840) (4.954, 3.792) (5.000, 3.642) (5.044, 3.661) (5.087, 3.541) (5.129, 3.566) (5.170, 3.384) (5.209, 3.393) (5.248, 3.312) (5.285, 3.311) (5.322, 3.172) (5.358, 3.169) (5.392, 3.031) (5.426, 3.113) (5.459, 2.943) (5.492, 2.988) (5.524, 2.847) (5.555, 2.920) (5.585, 2.792) (5.615, 2.803) (5.644, 2.706) (5.672, 2.741) (5.700, 2.632) (5.728, 2.687) (5.755, 2.560) (5.781, 2.559) (5.807, 2.505) (5.833, 2.490) (5.858, 2.408) (5.883, 2.462) (5.907, 2.339) (5.931, 2.373) (5.954, 2.318) (5.977, 2.292) (6.000, 2.205) (6.022, 2.238) (6.044, 2.151) (6.066, 2.167) (6.087, 2.080) (6.109, 2.088) (6.129, 2.069) (6.150, 2.056) (6.170, 1.992) (6.190, 2.030) (6.209, 1.930) (6.229, 1.942) (6.248, 1.908) (6.267, 1.926) (6.285, 1.862) (6.304, 1.850) (6.322, 1.800) (6.340, 1.813) (6.358, 1.764) (6.375, 1.802) (6.392, 1.745) (6.409, 1.725) (6.426, 1.713) (6.443, 1.687) (6.459, 1.664) (6.476, 1.675) (6.492, 1.592) (6.508, 1.590) (6.524, 1.565) (6.539, 1.569) (6.555, 1.566) (6.570, 1.549) (6.585, 1.501) (6.600, 1.513) (6.615, 1.468) (6.629, 1.463) (6.644, 1.403)
        }; \label{plot_c4_5_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 6.818) (2.322, 6.026) (2.585, 5.523) (2.807, 5.003) (3.000, 4.677) (3.170, 4.339) (3.322, 3.890) (3.459, 3.638) (3.585, 3.338) (3.700, 3.121) (3.807, 2.936) (3.907, 2.634) (4.000, 2.543) (4.087, 2.414) (4.170, 2.250) (4.248, 2.004) (4.322, 1.932) (4.392, 1.757) (4.459, 1.634) (4.524, 1.586) (4.585, 1.460) (4.644, 1.313) (4.700, 1.252) (4.755, 1.192) (4.807, 1.068) (4.858, 1.004) (4.907, 0.921) (4.954, 0.822) (5.000, 0.746) (5.044, 0.700) (5.087, 0.643) (5.129, 0.574) (5.170, 0.458) (5.209, 0.478) (5.248, 0.407) (5.285, 0.308) (5.322, 0.275) (5.358, 0.228) (5.392, 0.212) (5.426, 0.138) (5.459, 0.047) (5.492, 0.003) (5.524, 0.052) (5.555, -0.097) (5.585, -0.117) (5.615, -0.149) (5.644, -0.226) (5.672, -0.178) (5.700, -0.297) (5.728, -0.278) (5.755, -0.366) (5.781, -0.355) (5.807, -0.470) (5.833, -0.460) (5.858, -0.462) (5.883, -0.621) (5.907, -0.597) (5.931, -0.697) (5.954, -0.783) (5.977, -0.776) (6.000, -0.900) (6.022, -0.935) (6.044, -0.930) (6.066, -0.952) (6.087, -1.080) (6.109, -1.127) (6.129, -1.258) (6.150, -1.204) (6.170, -1.482) (6.190, -1.326) (6.209, -1.396) (6.229, -1.381) (6.248, -1.690) (6.267, -1.718) (6.285, -1.806) (6.304, -1.761) (6.322, -1.971) (6.340, -1.966) (6.358, -2.146) (6.375, -2.152) (6.392, -2.258) (6.409, -2.272) (6.426, -2.344) (6.443, -2.388) (6.459, -2.747) (6.476, -2.680) (6.492, -2.708) (6.508, -2.900) (6.524, -2.955) (6.539, -3.095) (6.555, -3.158) (6.570, -3.442) (6.585, -3.366) (6.600, -3.644) (6.615, -3.816) (6.629, -3.900) (6.644, -4.059)
        }; \label{plot_c5_0_naked}
        
        \addplot [black,mark=.] coordinates{
            (2.000, 4.198) (2.322, 4.082) (2.585, 2.992) (2.807, 2.753) (3.000, 1.981) (3.170, 1.964) (3.322, 1.268) (3.459, 1.140) (3.585, 0.544) (3.700, 0.520) (3.807, 0.024) (3.907, 0.037) (4.000, -0.458) (4.087, -0.462) (4.170, -0.781) (4.248, -0.911) (4.322, -1.258) (4.392, -1.262) (4.459, -1.826) (4.524, -1.884) (4.585, -2.336) (4.644, -2.523) (4.700, -2.966) (4.755, -2.868) (4.807, -3.644) (4.858, -3.158) (4.907, -4.265) (4.954, -4.083) (5.000, -4.540) (5.044, -4.644) (5.087, -5.573) (5.129, -5.158) (5.170, -6.265) (5.209, -6.158) (5.248, -6.966) (5.285, -6.966) (5.322, -8.966) (5.358, -7.644) (5.392, -8.381) (5.426, -7.966) (5.459, -9.966) (5.492, -9.966) (5.524, -9.966)
        }; \label{plot_c5_5_naked}
         
        \end{axis}
    \end{tikzpicture}
    \caption{Expected $\errLinf$ approximation error as a function of the number of targets $k \in [4,100]$, in log-log-scale, for  $W=32$  and $n/k = const$ rules. Half-ratio are more jagged because a new rule is added only on every other increment of $k$.}
    \label{figure_var_ratio_nk}
\end{figure}




\begin{figure}[!t]%[!ht]
	\centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.4\textwidth,
    		height=0.3\textwidth,
    		xmin=0,
    		xmax=15,
    		xtick={3,6,9,12,15},
    		xlabel=$\lg(k)$ (log of number of targets),
    		ymin=0,
            ymax=30,
            ytick={0,5,10,15,20,25,30},
            ylabel=$\lg(\text{approx. err.})$,
    		legend style={at={(0.99,0.99)}, anchor=north west,font=\footnotesize,},
    		label style={font=\footnotesize},
    		grid=both
        ]

        \addplot [black,mark=+] coordinates{
            (9.965784285, 18.74334721) (10.96578428, 17.7334931) (11.55074679, 17.16453301) (11.96578428, 16.72514615) (12.28771238, 16.43805092) (12.55074679, 16.16641771) (12.77313921, 15.93130932) (12.96578428, 15.73103365) (13.13570929, 15.58360934) (13.28771238, 15.43936796) (13.4252159, 15.29802425) (13.55074679, 15.16341775) (13.666224, 15.05148426) (13.77313921, 14.93815253) (13.87267488, 14.81621369) (13.96578428, 14.72865289) (14.05324713, 14.65280857) (14.13570929, 14.58121647) (14.2137118, 14.51142776) (14.28771238, 14.44037543)
            
        }; \addlegendentry{$n=1k$}
        
        \addplot [black,mark=o] coordinates{
            (9.965784285, 12.77353898) (10.96578428, 11.77362552) (11.55074679, 11.1233778) (11.96578428, 10.76702573) (12.28771238, 10.45722696) (12.55074679, 10.12875479) (12.77313921, 9.903806547) (12.96578428, 9.774968209) (13.13570929, 9.621447519) (13.28771238, 9.462543171) (13.4252159, 9.291907403) (13.55074679, 9.124198874) (13.666224, 8.982137968) (13.77313921, 8.912200749) (13.87267488, 8.842601772) (13.96578428, 8.771753554) (14.05324713, 8.694148912) (14.13570929, 8.618238656) (14.2137118, 8.542335445) (14.28771238, 8.460947291)
        }; \addlegendentry{$n=2k$}
        
        \addplot [black,mark=square] coordinates{
            (9.965784285, 6.773073253) (10.96578428, 5.765004246) (11.55074679, 5.128045891) (11.96578428, 4.771885579) (12.28771238, 4.464668267) (12.55074679, 4.130107179) (12.77313921, 3.909773104) (12.96578428, 3.783456654) (13.13570929, 3.612352499) (13.28771238, 3.463360886) (13.4252159, 3.294253136) (13.55074679, 3.135863165) (13.666224, 3) (13.77313921, 2.942983598) (13.87267488, 2.809414444) (13.96578428, 2.807354922) (14.05324713, 2.698218478) (14.13570929, 2.584962501) (14.2137118, 2.584962501) (14.28771238, 2.46727948)
        }; \addlegendentry{$n=3k$}
    
        \addplot [black,mark=diamond] coordinates{
            (9.965784285, 0.918386234) (10.96578428, 0) (11.55074679, -0.217591435)
        }; \addlegendentry{$n=4k$}

        \addplot [black,mark=.] coordinates{
            (2.000, 27.037) (2.322, 26.695) (2.585, 26.487) (2.807, 26.218) (3.000, 25.985) (3.170, 25.889) (3.322, 25.699) (3.459, 25.535) (3.585, 25.426) (3.700, 25.286) (3.807, 25.170) (3.907, 25.048) (4.000, 24.924) (4.087, 24.892) (4.170, 24.773) (4.248, 24.664) (4.322, 24.622) (4.392, 24.531) (4.459, 24.439) (4.524, 24.388) (4.585, 24.330) (4.644, 24.272) (4.700, 24.211) (4.755, 24.137) (4.807, 24.101) (4.858, 24.044) (4.907, 23.988) (4.954, 23.953) (5.000, 23.871) (5.044, 23.831) (5.087, 23.785) (5.129, 23.719) (5.170, 23.679) (5.209, 23.651) (5.248, 23.585) (5.285, 23.549) (5.322, 23.507) (5.358, 23.481) (5.392, 23.439) (5.426, 23.405) (5.459, 23.386) (5.492, 23.339) (5.524, 23.323) (5.555, 23.298) (5.585, 23.256) (5.615, 23.238) (5.644, 23.216) (5.672, 23.172) (5.700, 23.141) (5.728, 23.109) (5.755, 23.098) (5.781, 23.062) (5.807, 23.025) (5.833, 23.000) (5.858, 22.973) (5.883, 22.953) (5.907, 22.938) (5.931, 22.889) (5.954, 22.889) (5.977, 22.846) (6.000, 22.803) (6.022, 22.780) (6.044, 22.765) (6.066, 22.741) (6.087, 22.719) (6.109, 22.677) (6.129, 22.661) (6.150, 22.662) (6.170, 22.632) (6.190, 22.602) (6.209, 22.579) (6.229, 22.551) (6.248, 22.548) (6.267, 22.523) (6.285, 22.497) (6.304, 22.491) (6.322, 22.473) (6.340, 22.457) (6.358, 22.426) (6.375, 22.420) (6.392, 22.409) (6.409, 22.384) (6.426, 22.379) (6.443, 22.347) (6.459, 22.350) (6.476, 22.312) (6.492, 22.317) (6.508, 22.295) (6.524, 22.283) (6.539, 22.262) (6.555, 22.245) (6.570, 22.229) (6.585, 22.224) (6.600, 22.207) (6.615, 22.189) (6.629, 22.191) (6.644, 22.167)
            (9.965784285, 18.74334721) (10.96578428, 17.7334931) (11.55074679, 17.16453301) (11.96578428, 16.72514615) (12.28771238, 16.43805092) (12.55074679, 16.16641771) (12.77313921, 15.93130932) (12.96578428, 15.73103365) (13.13570929, 15.58360934) (13.28771238, 15.43936796) (13.4252159, 15.29802425) (13.55074679, 15.16341775) (13.666224, 15.05148426) (13.77313921, 14.93815253) (13.87267488, 14.81621369) (13.96578428, 14.72865289) (14.05324713, 14.65280857) (14.13570929, 14.58121647) (14.2137118, 14.51142776) (14.28771238, 14.44037543)
        }; % naked, c=1.
        
        \addplot [black,mark=.] coordinates{
            (2.000, 22.019) (2.322, 21.631) (2.585, 21.267) (2.807, 20.928) (3.000, 20.656) (3.170, 20.471) (3.322, 20.215) (3.459, 20.127) (3.585, 19.899) (3.700, 19.730) (3.807, 19.622) (3.907, 19.477) (4.000, 19.338) (4.087, 19.216) (4.170, 19.163) (4.248, 19.054) (4.322, 18.923) (4.392, 18.852) (4.459, 18.790) (4.524, 18.678) (4.585, 18.609) (4.644, 18.538) (4.700, 18.457) (4.755, 18.449) (4.807, 18.357) (4.858, 18.274) (4.907, 18.205) (4.954, 18.161) (5.000, 18.090) (5.044, 18.042) (5.087, 17.995) (5.129, 17.960) (5.170, 17.908) (5.209, 17.879) (5.248, 17.814) (5.285, 17.752) (5.322, 17.722) (5.358, 17.666) (5.392, 17.647) (5.426, 17.627) (5.459, 17.546) (5.492, 17.521) (5.524, 17.482) (5.555, 17.466) (5.585, 17.420) (5.615, 17.392) (5.644, 17.328) (5.672, 17.308) (5.700, 17.287) (5.728, 17.249) (5.755, 17.216) (5.781, 17.183) (5.807, 17.157) (5.833, 17.127) (5.858, 17.114) (5.883, 17.072) (5.907, 17.059) (5.931, 17.000) (5.954, 16.967) (5.977, 16.956) (6.000, 16.936) (6.022, 16.917) (6.044, 16.870) (6.066, 16.863) (6.087, 16.826) (6.109, 16.834) (6.129, 16.805) (6.150, 16.778) (6.170, 16.707) (6.190, 16.706) (6.209, 16.687) (6.229, 16.678) (6.248, 16.667) (6.267, 16.632) (6.285, 16.634) (6.304, 16.613) (6.322, 16.564) (6.340, 16.547) (6.358, 16.543) (6.375, 16.535) (6.392, 16.484) (6.409, 16.464) (6.426, 16.468) (6.443, 16.458) (6.459, 16.438) (6.476, 16.421) (6.492, 16.390) (6.508, 16.375) (6.524, 16.356) (6.539, 16.340) (6.555, 16.329) (6.570, 16.298) (6.585, 16.316) (6.600, 16.279) (6.615, 16.266) (6.629, 16.240) (6.644, 16.226)
            (9.965784285, 12.77353898) (10.96578428, 11.77362552) (11.55074679, 11.1233778) (11.96578428, 10.76702573) (12.28771238, 10.45722696) (12.55074679, 10.12875479) (12.77313921, 9.903806547) (12.96578428, 9.774968209) (13.13570929, 9.621447519) (13.28771238, 9.462543171) (13.4252159, 9.291907403) (13.55074679, 9.124198874) (13.666224, 8.982137968) (13.77313921, 8.912200749) (13.87267488, 8.842601772) (13.96578428, 8.771753554) (14.05324713, 8.694148912) (14.13570929, 8.618238656) (14.2137118, 8.542335445) (14.28771238, 8.460947291)
        }; % naked, c=2.
        
        \addplot [black,mark=.] coordinates{
            (2.000, 16.904) (2.322, 16.443) (2.585, 16.022) (2.807, 15.632) (3.000, 15.346) (3.170, 15.101) (3.322, 14.830) (3.459, 14.601) (3.585, 14.445) (3.700, 14.213) (3.807, 14.068) (3.907, 13.930) (4.000, 13.773) (4.087, 13.605) (4.170, 13.460) (4.248, 13.429) (4.322, 13.259) (4.392, 13.191) (4.459, 13.087) (4.524, 13.034) (4.585, 12.919) (4.644, 12.834) (4.700, 12.729) (4.755, 12.650) (4.807, 12.594) (4.858, 12.544) (4.907, 12.457) (4.954, 12.391) (5.000, 12.336) (5.044, 12.242) (5.087, 12.202) (5.129, 12.189) (5.170, 12.105) (5.209, 12.058) (5.248, 12.011) (5.285, 11.994) (5.322, 11.909) (5.358, 11.858) (5.392, 11.800) (5.426, 11.747) (5.459, 11.722) (5.492, 11.693) (5.524, 11.614) (5.555, 11.620) (5.585, 11.595) (5.615, 11.527) (5.644, 11.499) (5.672, 11.481) (5.700, 11.452) (5.728, 11.396) (5.755, 11.361) (5.781, 11.330) (5.807, 11.271) (5.833, 11.271) (5.858, 11.238) (5.883, 11.196) (5.907, 11.169) (5.931, 11.123) (5.954, 11.110) (5.977, 11.072) (6.000, 11.037) (6.022, 11.032) (6.044, 10.995) (6.066, 10.986) (6.087, 10.975) (6.109, 10.928) (6.129, 10.855) (6.150, 10.855) (6.170, 10.815) (6.190, 10.803) (6.209, 10.791) (6.229, 10.760) (6.248, 10.753) (6.267, 10.740) (6.285, 10.723) (6.304, 10.675) (6.322, 10.638) (6.340, 10.643) (6.358, 10.650) (6.375, 10.584) (6.392, 10.603) (6.409, 10.590) (6.426, 10.516) (6.443, 10.526) (6.459, 10.523) (6.476, 10.493) (6.492, 10.470) (6.508, 10.477) (6.524, 10.431) (6.539, 10.435) (6.555, 10.418) (6.570, 10.380) (6.585, 10.355) (6.600, 10.322) (6.615, 10.368) (6.629, 10.301) (6.644, 10.301)
            (9.965784285, 6.773073253) (10.96578428, 5.765004246) (11.55074679, 5.128045891) (11.96578428, 4.771885579) (12.28771238, 4.464668267) (12.55074679, 4.130107179) (12.77313921, 3.909773104) (12.96578428, 3.783456654) (13.13570929, 3.612352499) (13.28771238, 3.463360886) (13.4252159, 3.294253136) (13.55074679, 3.135863165) (13.666224, 3) (13.77313921, 2.942983598) (13.87267488, 2.809414444) (13.96578428, 2.807354922) (14.05324713, 2.698218478) (14.13570929, 2.584962501) (14.2137118, 2.584962501) (14.28771238, 2.46727948)
        }; % naked, c=3.
    
        \addplot [black,mark=.] coordinates{
            (2.000, 11.857) (2.322, 11.389) (2.585, 10.740) (2.807, 10.311) (3.000, 10.031) (3.170, 9.697) (3.322, 9.390) (3.459, 9.084) (3.585, 8.867) (3.700, 8.641) (3.807, 8.531) (3.907, 8.358) (4.000, 8.135) (4.087, 8.009) (4.170, 7.810) (4.248, 7.764) (4.322, 7.614) (4.392, 7.493) (4.459, 7.410) (4.524, 7.271) (4.585, 7.185) (4.644, 7.116) (4.700, 7.025) (4.755, 6.888) (4.807, 6.823) (4.858, 6.771) (4.907, 6.717) (4.954, 6.625) (5.000, 6.561) (5.044, 6.489) (5.087, 6.434) (5.129, 6.355) (5.170, 6.280) (5.209, 6.219) (5.248, 6.163) (5.285, 6.130) (5.322, 6.073) (5.358, 5.983) (5.392, 6.009) (5.426, 5.928) (5.459, 5.918) (5.492, 5.824) (5.524, 5.796) (5.555, 5.754) (5.585, 5.739) (5.615, 5.684) (5.644, 5.685) (5.672, 5.587) (5.700, 5.574) (5.728, 5.505) (5.755, 5.491) (5.781, 5.467) (5.807, 5.427) (5.833, 5.390) (5.858, 5.349) (5.883, 5.329) (5.907, 5.293) (5.931, 5.242) (5.954, 5.226) (5.977, 5.215) (6.000, 5.181) (6.022, 5.143) (6.044, 5.124) (6.066, 5.071) (6.087, 5.063) (6.109, 5.029) (6.129, 5.014) (6.150, 4.997) (6.170, 4.937) (6.190, 4.946) (6.209, 4.926) (6.229, 4.896) (6.248, 4.867) (6.267, 4.824) (6.285, 4.779) (6.304, 4.813) (6.322, 4.750) (6.340, 4.762) (6.358, 4.709) (6.375, 4.679) (6.392, 4.675) (6.409, 4.646) (6.426, 4.632) (6.443, 4.626) (6.459, 4.629) (6.476, 4.591) (6.492, 4.576) (6.508, 4.525) (6.524, 4.511) (6.539, 4.492) (6.555, 4.503) (6.570, 4.478) (6.585, 4.439) (6.600, 4.417) (6.615, 4.424) (6.629, 4.393) (6.644, 4.395)
            (9.965784285, 0.918386234) (10.96578428, 0) (11.55074679, -0.217591435)
        }; % naked, c=4.
        
        \end{axis}
    \end{tikzpicture}
    \caption{Expected $\errLinf$ approximation error as a function of the number of targets $k$, for large
     values of $k$, specifically, for $k=1000x$ where $x \in [1,20]$. This graph shows the expected $\errLinf$ approximation error as a function of the number of targets, in log-log-scale, for  $W=32$  and $n/k = const$ rules. For $n/k \ge 4$ there is typically no error for large $k$. (The plot is extended to $\lg k < 7$ according to Fig.~\ref{figure_var_ratio_nk}.)}
    \label{figure_var_ratio_nk_large}
\end{figure}






\begin{figure}[t]
	%\centering
    \subfigure[$n=25$ Rules.] {
        \hspace*{-1.0em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of targets $k$,
        		style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		ymin=0, ymax = 160,
                ytick={32,64,96,128,160},
                ylabel=$(\text{approx.\ err.}) / 2^{20}$,
        		legend style={at={(0.01,0.99)}, anchor=north west,font=\footnotesize,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black] coordinates{
            (4, 0.000) (5, 0.000) (6, 0.001) (7, 0.006) (8, 0.025) (9, 0.075) (10, 0.184) (11, 0.376) (12, 0.694) (13, 1.165) (14, 1.744) (15, 2.568) (16, 3.546) (17, 4.660) (18, 5.872) (19, 7.711) (20, 9.292) (21, 10.917) (22, 12.987) (23, 15.124) (24, 17.194) (25, 19.514) (26, 21.270) (27, 23.370) (28, 25.707) (29, 27.906) (30, 30.483) (31, 33.143) (32, 35.725) (33, 38.471) (34, 40.324) (35, 42.541) (36, 44.682) (37, 47.117) (38, 49.099) (39, 51.049) (40, 52.418) (41, 54.987) (42, 56.188) (43, 59.531) (44, 60.893) (45, 63.211) (46, 65.749) (47, 67.510) (48, 68.895) (49, 71.632) (50, 73.455) (51, 75.359) (52, 77.116) (53, 79.149) (54, 81.623) (55, 83.416) (56, 86.457) (57, 88.171) (58, 88.829) (59, 90.995) (60, 93.638) (61, 95.821) (62, 96.697) (63, 98.801) (64, 101.033) (65, 102.585) (66, 104.044) (67, 105.569) (68, 106.887) (69, 108.518) (70, 110.642) (71, 111.676) (72, 112.102) (73, 114.511) (74, 116.100) (75, 116.739) (76, 118.520) (77, 119.024) (78, 121.080) (79, 121.400) (80, 123.217) (81, 123.723) (82, 124.604) (83, 126.482) (84, 127.274) (85, 128.371) (86, 130.427) (87, 130.289) (88, 131.685) (89, 132.892) (90, 133.769) (91, 134.775) (92, 135.716) (93, 136.642) (94, 136.771) (95, 138.313) (96, 139.145) (97, 139.888) (98, 141.111) (99, 141.090) (100, 142.006)
            }; %\addlegendentry{$n=25$ rules} 
            
            \addplot [black, style=dashed] coordinates{ (4, 7.37745E-07) (5, 4.72442E-05) (6, 0.000753882) (7, 0.00542188) (8, 0.023670763) (9, 0.074061684) (10, 0.183513401) (11, 0.38378457) (12, 0.706824218) (13, 1.18067132) (14, 1.826752096) (15, 2.658680653) (16, 3.68226575) (17, 4.896307865) (18, 6.293809237) (19, 7.8633163) (20, 9.590213977) (21, 11.45787227) (22, 13.4486026) (23, 15.54441738) (24, 17.72760701) (25, 19.98115788) (26, 22.28903842) (27, 24.63637957) (28, 27.00957302) (29, 29.39630767) (30, 31.78556078) (31, 34.1675572) (32, 36.53370717) (33, 38.87653064) (34, 41.1895742) (35, 43.467325) (36, 45.70512487) (37, 47.89908689) (38, 50.04601582) (39, 52.14333332) (40, 54.1890085) (41, 56.18149403) (42, 58.11966772) (43, 60.00277953) (44, 61.8304037) (45, 63.60239573) (46, 65.3188538) (47, 66.98008445) (48, 68.58657195) (49, 70.13895118) (50, 71.63798367) (51, 73.08453635) (52, 74.479563) (53, 75.82408782) (54, 77.11919114) (55, 78.36599687) (56, 79.56566162) (57, 80.71936518) (58, 81.82830236) (59, 82.89367586) (60, 83.9166902) (61, 84.8985465) (62, 85.84043802) (63, 86.74354638) (64, 87.60903846) (65, 88.43806365) (66, 89.23175175) (67, 89.99121114) (68, 90.71752735) (69, 91.41176194) (70, 92.07495165) (71, 92.70810772) (72, 93.31221553) (73, 93.88823426) (74, 94.43709684) (75, 94.95970993) (76, 95.45695409) (77, 95.92968391) (78, 96.37872841) (79, 96.8048913) (80, 97.20895148) (81, 97.59166341) (82, 97.95375768) (83, 98.2959415) (84, 98.61889921) (85, 98.9232929) (86, 99.20976295) (87, 99.47892861) (88, 99.73138856) (89, 99.96772156) (90, 100.188487) (91, 100.3942253) (92, 100.585459) (93, 100.7626926) (94, 100.9264137) (95, 101.0770933) (96, 101.2151864) (97, 101.3411323) (98, 101.4553556) (99, 101.5582663) (100, 101.6502602) }; %%% ANALYTIC FORMULA VALUES
        \end{axis}
    \end{tikzpicture} 
    \label{figure_var_k_and_equation_plot_sub1}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$n=50$ Rules.] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of targets $k$,
        		style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		ymin=0, ymax = 40,
                ytick={8,16,24,32,40},
                % ylabel=$(\text{approx.\ err.}) / 2^{20}$, % rely on the other figure
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black] coordinates{
            (4, 0.000) (5, 0.000) (6, 0.000) (7, 0.000) (8, 0.000) (9, 0.000) (10, 0.000) (11, 0.000) (12, 0.000) (13, 0.001) (14, 0.002) (15, 0.004) (16, 0.008) (17, 0.015) (18, 0.026) (19, 0.042) (20, 0.068) (21, 0.100) (22, 0.148) (23, 0.207) (24, 0.274) (25, 0.354) (26, 0.463) (27, 0.602) (28, 0.757) (29, 0.899) (30, 1.092) (31, 1.314) (32, 1.543) (33, 1.821) (34, 2.086) (35, 2.398) (36, 2.703) (37, 3.053) (38, 3.416) (39, 3.842) (40, 4.184) (41, 4.669) (42, 5.025) (43, 5.621) (44, 6.153) (45, 6.535) (46, 7.120) (47, 7.664) (48, 8.174) (49, 8.748) (50, 9.107) (51, 9.780) (52, 10.364) (53, 10.862) (54, 11.383) (55, 12.044) (56, 12.532) (57, 13.113) (58, 13.578) (59, 14.261) (60, 14.972) (61, 15.560) (62, 16.163) (63, 16.827) (64, 17.266) (65, 17.778) (66, 18.488) (67, 19.328) (68, 19.590) (69, 20.067) (70, 20.668) (71, 21.086) (72, 21.849) (73, 22.314) (74, 22.756) (75, 23.387) (76, 23.828) (77, 24.175) (78, 24.821) (79, 25.354) (80, 25.750) (81, 26.260) (82, 26.818) (83, 26.990) (84, 27.863) (85, 28.348) (86, 28.919) (87, 29.619) (88, 29.814) (89, 30.329) (90, 31.311) (91, 31.317) (92, 32.248) (93, 32.597) (94, 33.454) (95, 33.851) (96, 34.428) (97, 35.158) (98, 35.679) (99, 36.231) (100, 36.777)
            }; %\addlegendentry{$n=50$ rules} 
            
            \addplot [black, style=dashed] coordinates{ (4, 1.00076E-16) (5, 5.03202E-13) (6, 1.51351E-10) (7, 9.01226E-09) (8, 1.94059E-07) (9, 2.11556E-06) (10, 1.43012E-05) (11, 6.82377E-05) (12, 0.000250606) (13, 0.000752285) (14, 0.001927011) (15, 0.004347391) (16, 0.008845672) (17, 0.016530634) (18, 0.028777666) (19, 0.047194337) (20, 0.073567242) (21, 0.109797452) (22, 0.157831768) (23, 0.219595915) (24, 0.296934173) (25, 0.391558343) (26, 0.505007468) (27, 0.638618585) (28, 0.793507947) (29, 0.970561637) (30, 1.170434201) (31, 1.39355383) (32, 1.640132649) (33, 1.91018077) (34, 2.203522946) (35, 2.51981681) (36, 2.85857187) (37, 3.21916862) (38, 3.600877234) (39, 4.002875487) (40, 4.424265625) (41, 4.864090012) (42, 5.321345457) (43, 5.794996173) (44, 6.283985379) (45, 6.787245564) (46, 7.303707488) (47, 7.832307983) (48, 8.371996644) (49, 8.921741498) (50, 9.480533735) (51, 10.04739161) (52, 10.62136359) (53, 11.2015308) (54, 11.78700894) (55, 12.37694963) (56, 12.97054131) (57, 13.56700977) (58, 14.16561833) (59, 14.76566773) (60, 15.3664958) (61, 15.96747688) (62, 16.56802114) (63, 17.16757372) (64, 17.76561375) (65, 18.36165332) (66, 18.95523638) (67, 19.54593758) (68, 20.13336106) (69, 20.71713929) (70, 21.2969318) (71, 21.87242403) (72, 22.44332608) (73, 23.00937156) (74, 23.57031643) (75, 24.12593784) (76, 24.67603305) (77, 25.22041834) (78, 25.75892801) (79, 26.29141334) (80, 26.81774163) (81, 27.3377953) (82, 27.851471) (83, 28.35867873) (84, 28.85934106) (85, 29.35339233) (86, 29.84077794) (87, 30.32145361) (88, 30.79538474) (89, 31.26254577) (90, 31.72291957) (91, 32.17649686) (92, 32.62327567) (93, 33.06326087) (94, 33.4964636) (95, 33.92290091) (96, 34.34259523) (97, 34.75557404) (98, 35.16186944) (99, 35.5615178) (100, 35.95455943) }; %%% ANALYTIC FORMULA VALUES
        \end{axis}
    \end{tikzpicture}
    \label{figure_var_k_and_equation_plot_sub2}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$n=100$ Rules.] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of targets $k$,
        		style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		ymin=0, ymax = 5,
                ytick={1,2,3,4,5},
                % ylabel=$(\text{approx.\ err.}) / 2^{20}$, % rely on the other figure
        		legend style={at={(0.01,0.99)}, anchor=north west,font=\footnotesize,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black] coordinates{
            (4, 0.000) (5, 0.000) (6, 0.000) (7, 0.000) (8, 0.000) (9, 0.000) (10, 0.000) (11, 0.000) (12, 0.000) (13, 0.000) (14, 0.000) (15, 0.000) (16, 0.000) (17, 0.000) (18, 0.000) (19, 0.000) (20, 0.000) (21, 0.000) (22, 0.000) (23, 0.000) (24, 0.000) (25, 0.000) (26, 0.000) (27, 0.000) (28, 0.001) (29, 0.001) (30, 0.001) (31, 0.002) (32, 0.003) (33, 0.004) (34, 0.006) (35, 0.008) (36, 0.010) (37, 0.013) (38, 0.017) (39, 0.022) (40, 0.028) (41, 0.034) (42, 0.043) (43, 0.051) (44, 0.060) (45, 0.075) (46, 0.086) (47, 0.103) (48, 0.120) (49, 0.135) (50, 0.160) (51, 0.182) (52, 0.209) (53, 0.234) (54, 0.264) (55, 0.293) (56, 0.336) (57, 0.374) (58, 0.412) (59, 0.455) (60, 0.502) (61, 0.549) (62, 0.600) (63, 0.657) (64, 0.718) (65, 0.762) (66, 0.844) (67, 0.908) (68, 0.961) (69, 1.053) (70, 1.118) (71, 1.189) (72, 1.248) (73, 1.351) (74, 1.425) (75, 1.517) (76, 1.609) (77, 1.667) (78, 1.801) (79, 1.877) (80, 1.972) (81, 2.072) (82, 2.185) (83, 2.307) (84, 2.421) (85, 2.528) (86, 2.703) (87, 2.818) (88, 2.916) (89, 3.084) (90, 3.151) (91, 3.324) (92, 3.449) (93, 3.542) (94, 3.691) (95, 3.832) (96, 3.956) (97, 4.086) (98, 4.201) (99, 4.388) (100, 4.505)
            }; % \addlegendentry{$n=100$ rules}
            
            \addplot [black, style=dashed] coordinates{ (4, 1.84154E-36) (5, 5.70862E-29) (6, 6.10026E-24) (7, 2.49001E-20) (8, 1.3043E-17) (9, 1.72618E-15) (10, 8.68525E-14) (11, 2.15724E-12) (12, 3.15031E-11) (13, 3.05414E-10) (14, 2.14434E-09) (15, 1.1624E-08) (16, 5.10461E-08) (17, 1.88422E-07) (18, 6.01644E-07) (19, 1.70004E-06) (20, 4.32909E-06) (21, 1.00825E-05) (22, 2.17385E-05) (23, 4.38252E-05) (24, 8.33068E-05) (25, 0.000150365) (26, 0.000259245) (27, 0.000429112) (28, 0.000684886) (29, 0.001057995) (30, 0.001587016) (31, 0.00231816) (32, 0.003305593) (33, 0.004611566) (34, 0.006306351) (35, 0.008468004) (36, 0.01118195) (37, 0.014540412) (38, 0.018641718) (39, 0.023589496) (40, 0.029491793) (41, 0.036460132) (42, 0.044608551) (43, 0.054052617) (44, 0.064908464) (45, 0.077291856) (46, 0.091317288) (47, 0.107097144) (48, 0.12474092) (49, 0.144354515) (50, 0.166039592) (51, 0.189893018) (52, 0.216006384) (53, 0.244465593) (54, 0.275350524) (55, 0.308734772) (56, 0.344685447) (57, 0.383263038) (58, 0.42452134) (59, 0.468507424) (60, 0.515261665) (61, 0.564817804) (62, 0.61720306) (63, 0.67243826) (64, 0.730538013) (65, 0.791510899) (66, 0.855359683) (67, 0.922081543) (68, 0.991668316) (69, 1.06410675) (70, 1.139378766) (71, 1.217461725) (72, 1.298328696) (73, 1.381948723) (74, 1.468287101) (75, 1.557305634) (76, 1.6489629) (77, 1.743214507) (78, 1.840013342) (79, 1.939309815) (80, 2.041052094) (81, 2.145186332) (82, 2.251656883) (83, 2.360406514) (84, 2.471376604) (85, 2.584507335) (86, 2.69973787) (87, 2.817006532) (88, 2.936250957) (89, 3.057408256) (90, 3.180415155) (91, 3.305208132) (92, 3.431723542) (93, 3.559897738) (94, 3.689667182) (95, 3.820968546) (96, 3.953738807) (97, 4.087915338) (98, 4.223435985) (99, 4.360239146) (100, 4.498263838) }; %%% ANALYTIC FORMULA VALUES
        \end{axis}
    \end{tikzpicture}
    \label{figure_var_k_and_equation_plot_sub3}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \caption{Expected $\errLinf$ approximation error as a function of the number of targets $k \in [4,100]$, for  $W=32$ and $n=25,50,100$ rules. The dashed line plots Equation~(\ref{equation_empiric}) of Section~\ref{subsection_experiments_ratio_nk} for comparison.
    \label{figure_var_k_and_equation_plot}}
\end{figure}


\subsection{\texorpdfstring{$\errLinfPos$}{L-infinity+} error vs. \texorpdfstring{$\errLinf$}{L-infinity} error}
\label{subsection_experiments_onesided_vs_twosided}

In this section we compare the expectation of the $\errLinfPos$ error which we considered in Section~\ref{section_one_sided_metric} to
the expectation of the $\errLinf$ error, as a function of the number of rules $n$.
We note that there are partitions for which this difference is large. For example, let $c > k$ be a power of $2$, and define $P = [k-1, c-1, \ldots, c-1, 2^W - (k-2)c - 1]$, and 
 let $P' = [0, c, \ldots, c, 2^W - (k-2)c]$.  One can verify that the $\errLinf$ error of $P'$ is $k-1$, which is 
 the smallest possible with $k-1$ rules
since at least one weight of $P'$ must be $0$. The $\errLinfPos$ error of $P'$ is only $1$, which is also the smallest possible with $k-1$ rules. The example can be scaled-up by a factor of $2^d$ for any integer $d>0$, though the ratio of the errors will not change.

For a random partition the expected difference between these errors is much less noticeable. Fig.~\ref{figure_oneisded_two_sided_ratio} shows the ratio between the expected $\errLinfPos$ error and the expected $\errLinf$ error for fixed $k=10$, and $W=32$.
The $\errLinfPos$ error is, of course, never larger than the $\errLinf$ error, and we see that in fact the ratio is around $0.89$ for most values of $n$. It starts at $1.0$ since with one rule there is no difference:
The overload of the server that gets the rule is equal to the sum of the underloads of all the other servers.
As long as $n \le k$ it is still likely
for these errors to be equal, until the overloads and underloads spread over enough different weights. Even with two rules there can be a difference, for example $P=[2,3,3]$ is best approximated by $P'=[0,4,4]$ for both errors
(these partitions are obtained by substituting $k=3$, and $c=4$ in the general example at the beginning of this section), which yields $\errLinfPos$ error of $1$ compared to $\errLinf$ error of $2$. However, for $n > k$ (See Fig.~\ref{figure_oneisded_two_sided_ratio} for  $n > k=10$), there is enough freedom for the difference between the errors to show up. The ratio climbs back to  $1.0$ for $n \ge 55$ due to increasing probability to achieve exact representation of the partitions. We conclude that on average, when there are not too many or too few rules ($n$) compared to the number of targets ($k$), the $\errLinfPos$ error is approximately $11\%$ smaller than the $\errLinf$ error.

\begin{figure}[!t]%[!ht]
	\centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.45\textwidth,
    		height=0.17\textwidth,
    		xmin=0,
    		xmax=65,
    		xtick={10,20,30,40,50,60},
    		xlabel=$n$ TCAM rules,
    		ymin=0.85,
            ymax =1.0,
            ytick={0.85,0.9,0.95,1},
            ylabel= ratio of errors, %ratio of expected errors: 1sided/2sided,
    		legend style={at={(0.99,0.99)}, anchor=north east,font=\footnotesize,},
    		label style={font=\footnotesize},
    		grid=both
        ]
          
         \addplot [black,mark=o] coordinates{
            (1, 1.000000) (2, 1.000000) (3, 0.999458) (4, 0.984523) (5, 0.981701) (6, 0.952732) (7, 0.907828) (8, 0.893221) (9, 0.910348) (10, 0.900306) (11, 0.896299) (12, 0.888149) (13, 0.892425) (14, 0.876268) (15, 0.894018) (16, 0.896648) (17, 0.887059) (18, 0.896399) (19, 0.882834) (20, 0.885826) (21, 0.886754) (22, 0.894880) (23, 0.897189) (24, 0.888391) (25, 0.878349) (26, 0.883497) (27, 0.896134) (28, 0.889211) (29, 0.881904) (30, 0.890634) (31, 0.882112) (32, 0.896815) (33, 0.892864) (34, 0.881165) (35, 0.886521) (36, 0.876369) (37, 0.883481) (38, 0.882866) (39, 0.874994) (40, 0.894832) (41, 0.877543) (42, 0.894413) (43, 0.891436) (44, 0.882172) (45, 0.875610) (46, 0.883655) (47, 0.883596) (48, 0.884305) (49, 0.893497) (50, 0.906049) (51, 0.881170) (52, 0.889650) (53, 0.891278) (54, 0.905243) (55, 0.900136) (56, 0.906130) (57, 0.919802) (58, 0.928571) (59, 0.950867) (60, 0.945000) (61, 0.956522) (62, 1.000000) (63, 1.000000) (64, 1.000000) (65, 1.000000)
         };
     		
        \end{axis}
    \end{tikzpicture}
    \caption{Ratio between the expected $\errLinfPos$ error and the expected $\errLinf$ error,  as a function of $n \in [1,65]$  rules, for  $W=32$ and $k=10$ targets. When $n \le k=10$ or $n \ge 60$ the errors are close due to inability to approximate well or the ability to achieve zero-error, respectively. In between, the ratio is around $0.89$. \label{figure_oneisded_two_sided_ratio}}
\end{figure}

\subsection{Approximating with a prefix of Niagara}
\label{subsection_experiments_niagara_ratio}
In this subsection we evaluate the approximation error of following simple heuristic:
Compute a sequence of TCAM rules that induce the target partition exactly and use the last $n$  rules (with most don't-cares) in this sequence. 
\cite{BitMatcher} explains and shows experimentally that applying this heuristic to the sequence produced by Niagara gives better results than when applied to the sequence of Bit Matcher. For this reason, in this paper we only apply truncation to the sequence of Niagara.

Prefixes of the Niagara sequence may be sub-optimal. Fig.~\ref{figure_tcam_trie_all} shows the sub-optimality of a prefix of such a sequence. This example can be generalized by considering the partition $[2^{m+1},1,\ldots,1]$ with $k=2^{m+1}+1$ parts.
For this partition and $n=2$ rules, the ratio between the $\errLinf$ error of the truncated Niagara sequence and the optimal error is $2-\frac{1}{2^m}$. Namely, the error obtained by the truncated Niagara can be close to twice the optimal error. We conjecture that the error of such a truncation is at most twice the optimal error. Specifically, our conjecture is as follows.

\begin{conjecture}
\label{conjecture_approx2_error}
Let $P$ be a partition and let $P'$ be its optimal approximation in $\errLinf$, with $n$ TCAM rules. Choose $h$ such that $2^h \le |P-P'|_\infty < 2^{h+1}$. Then truncating a Niagara TCAM to $n$ rules induces a partition $P''$ such that $|P-P''|_\infty < 2^{h+1}$.
\end{conjecture}

Assuming this conjecture, it is not surprising that Niagara performs extremely well compared to the optimal algorithm, on a random partition.
For instance, Fig.~\ref{figure_ratio_1sided_2sided} shows that the expectation of the ratio between the error of a truncated Niagara sequence and the optimal error as a function of $n$, when $W=16$, and $k=16$, for both $\errLinfPos$ and $\errLinf$, is very close to $1$. The plotted values were averaged over $10,000$ random ordered-partitions. When $n \ge 16$, i.e.\ we have at least 1 rule per target, the ratios do not rise above $1.00015$ (less than $0.015\%$ extra error).\footnote{For $n < 16$, the approximation error is much more sensitive to the choices of Niagara, and as a result the expectation can get as high as $1.015$ ($\times 100$ the scale of $n \ge 16$). For clarity of the graphs in Fig.~\ref{figure_ratio_1sided_2sided} and Fig.~\ref{figure_ratio_1sided_2sided_w32} we limited the $y$-axis such that values of $n<16$ might not be presented.}
In the case of $\errLinfPosRel$, the approximation is not as good. The expectation of the ratio of errors can get up to $\approx 21$, as shown in Fig.~\ref{figure_ratio_relative}. This ratio is worse in $\errLinfPosRel$ than in $\errLinf$ and $\errLinfPos$ since Niagara reduces the sum of the deviations, regardless of the identity of the deviating target. Therefore, it may not differentiate between having some error in a target with small weight while it can have instead the same error in a target with larger weight. We note that while this leads to the conclusion that when approximating the partition for $\errLinfPosRel$ the Niagara-truncation heuristic is much worse, this should be taken with a grain of salt because the relative errors are quite small, even if their ratios are large.

Fig.~\ref{figure_ratio_1sided_2sided_w32} and Fig.~\ref{figure_ratio_relative_w32} shows the results for $W=32$ and $k=16$. 
The behaviour is similar.
When $16 \le n$, the ratios of $\errLinf$ and $\errLinfPos$ do not rise above $1.0001$ (less than $0.01\%$ difference), and the ratios of $\errLinfPosRel$ form a curve similar to Fig.~\ref{figure_ratio_relative}, but more noisy. The curve peaks at about $n=70$ with a ratio of $60$.
For $n=64$ and $n=69$ (excluded from the plot) we got much higher ratios of $119.1$ and $779.6$, respectively.

\begin{figure}[t]
	%\centering
    \subfigure[$\errLinf$,$\errLinfPos$ , $W=16$] {
        \hspace*{-1.0em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=60,
        		xtick={0,10,20,30,40,50,60},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 1.5,
                ytick={0,0.3,0.6,0.9,1.2,1.5},
                ylabel={$\mathbb{E} \Big [\frac{errNiagara}{errOPT}  - 1 \Big ] \cdot {10}^4$},
        		legend style={at={(0.00,1.35)}, anchor=north west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            %\addplot [black,mark=o] coordinates{ (32,0.989379085) }; \addlegendentry{$\errLinf$}
            %\addplot [blue,mark=square] coordinates{ (32,0.5) }; \addlegendentry{$\errLinfPos$} 
            \addplot [black] coordinates{ (32,0.989379085) }; \addlegendentry{$\errLinf$}
            \addplot [blue] coordinates{ (32,0.5) }; \addlegendentry{$\errLinfPos$} 
            
            \addplot [black] coordinates{ (1,0) (2,16.81446118) (3,2.28862606) (4,154.3576891) (5,56.80217883) (6,23.26155748) (7,17.82473539) (8,6.738601267) (9,0.607719695) (10,0.10081556) (11,0.426579191) (12,0.499660696) (13,0.455474639) (14,0.256931535) (15,0.392360121) (16,0.721879735) (17,0.098984826) (18,0.317075452) (19,0.337564276) (20,0.007042254) (21,0.404968281) (22,0.177504837) (23,0.191018836) (24,0.866314733) (25,0.159346847) (26,0.522330693) (27,0.184659091) (28,0.298411914) (29,0.27662656) (30,1.059659091) (31,0.766414141) (32,0.989379085) (33,0.683823529) (34,0.45) (35,0.75) (36,0.5) (37,1.25) (38,1) (39,0) (40,0) (41,0) (42,0) (43,0) (44,0) (45,0) (46,0) (47,0) (48,0) (49,0) (50,0) (51,0) (52,0) (53,0) (54,0) (55,0) (56,0) (57,0) (58,0) (59,0) (60,0) (61,0) (62,0) (63,0) (64,0) (65,0) (66,0) (67,0) (68,0) (69,0) (70,0) (71,0) (72,0) (73,0) (74,0) (75,0) (76,0) (77,0) (78,0) (79,0) (80,0) (81,0) (82,0) (83,0) (84,0) (85,0) (86,0) (87,0) (88,0) (89,0) (90,0) (91,0) (92,0) (93,0) (94,0) (95,0) (96,0) (97,0) (98,0) (99,0) (100,0) };
            
            \addplot [blue] coordinates{ (1,0) (2,16.81446118) (3,2.28862606) (4,154.3576891) (5,56.80217883) (6,23.26155748) (7,17.82473539) (8,6.738601267) (9,0.607719695) (10,0.10081556) (11,0.426579191) (12,0.487002468) (13,0.399008337) (14,0.256931535) (15,0.392360121) (16,0.721879735) (17,0.092470168) (18,0.105130156) (19,0.337564276) (20,0) (21,0.332200423) (22,0.177504837) (23,0.11375) (24,0.447280642) (25,0.128096847) (26,0.304979947) (27,0.03030303) (28,0.183712121) (29,0.0625) (30,0.403409091) (31,0.40530303) (32,0.5) (33,0.375) (34,0) (35,0.75) (36,0.25) (37,0.75) (38,0.5) (39,0) (40,0) (41,0) (42,0) (43,0) (44,0) (45,0) (46,0) (47,0) (48,0) (49,0) (50,0) (51,0) (52,0) (53,0) (54,0) (55,0) (56,0) (57,0) (58,0) (59,0) (60,0) (61,0) (62,0) (63,0) (64,0) (65,0) (66,0) (67,0) (68,0) (69,0) (70,0) (71,0) (72,0) (73,0) (74,0) (75,0) (76,0) (77,0) (78,0) (79,0) (80,0) (81,0) (82,0) (83,0) (84,0) (85,0) (86,0) (87,0) (88,0) (89,0) (90,0) (91,0) (92,0) (93,0) (94,0) (95,0) (96,0) (97,0) (98,0) (99,0) (100,0) }; 
            
        \end{axis}
    \end{tikzpicture} 
    \label{figure_ratio_1sided_2sided}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$\errLinfPosRel$ , $W=16$] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=60,
        		xtick={0,10,20,30,40,50,60},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 25,
                ytick={1,5,10,15,20,25},
                ylabel={$\mathbb{E} \Big [\frac{errNiagara}{errOPT} \Big ]$},
        		legend style={at={(0.00,1.35)}, anchor=north west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [purple,mark=*] coordinates{ (10,1.680585683) }; \addlegendentry{$\errLinfPosRel$}
            \addplot [purple] coordinates{ (1,1) (2,1.175133409) (3,1.09787264) (4,1.445871405) (5,1.323695651) (6,1.364065373) (7,1.479845948) (8,1.556778501) (9,1.578111293) (10,1.680585683) (11,1.882460916) (12,2.119955358) (13,2.369031145) (14,2.649321035) (15,3.013036285) (16,3.335528792) (17,3.745033534) (18,4.212176787) (19,4.544360526) (20,5.11561828) (21,5.670586241) (22,6.255260377) (23,6.879805921) (24,7.497152222) (25,8.311632908) (26,8.581045961) (27,9.613406763) (28,10.40185351) (29,11.24131202) (30,12.50416239) (31,13.43521012) (32,14.27429981) (33,15.02846765) (34,16.32102287) (35,18.62867119) (36,17.32594048) (37,20.05695193) (38,20.248786) (39,21.40273218) (40,19.1568527) (41,17.26511767) (42,14.83354594) (43,9.350585875) (44,7.499807427) (45,3.779141556) (46,2.045280685) (47,1.399050802) (48,1.095376756) (49,1.059314038) (50,1.00393177) (51,1.000785228) (52,1) (53,1) (54,1) (55,1) (56,1) (57,1) (58,1) (59,1) (60,1) (61,1) (62,1) (63,1) (64,1) (65,1) (66,1) (67,1) (68,1) (69,1) (70,1) (71,1) (72,1) (73,1) (74,1) (75,1) (76,1) (77,1) (78,1) (79,1) (80,1) (81,1) (82,1) (83,1) (84,1) (85,1) (86,1) (87,1) (88,1) (89,1) (90,1) (91,1) (92,1) (93,1) (94,1) (95,1) (96,1) (97,1) (98,1) (99,1) (100,1) }; 
        \end{axis}
    \end{tikzpicture}
    \label{figure_ratio_relative}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    
        \subfigure[$\errLinf$,$\errLinfPos$ , $W=32$] {
        \hspace*{-1.0em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 1.5,
                ytick={0,0.3,0.6,0.9,1.2,1.5},
                ylabel={$\mathbb{E} \Big [\frac{errNiagara}{errOPT}  - 1 \Big ] \cdot {10}^4$},
        		legend style={at={(0.00,1.35)}, anchor=north west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            %\addplot [black,mark=o] coordinates{ (78, 1.316176471) }; \addlegendentry{$\errLinf$}
            %\addplot [blue,mark=square] coordinates{ (78, 0) }; \addlegendentry{$\errLinfPos$}
            \addplot [black] coordinates{ (78, 1.316176471) }; \addlegendentry{$\errLinf$}
            \addplot [blue] coordinates{ (78, 0) }; \addlegendentry{$\errLinfPos$} 
            
            \addplot [black] coordinates{ (1, 0) (2, 16.83024335) (3, 2.291326631) (4, 154.2957953) (5, 56.89059852) (6, 23.09783296) (7, 17.87218466) (8, 6.673676571) (9, 0.606859014) (10, 0.100867171) (11, 0.430582273) (12, 0.503625708) (13, 0.457641601) (14, 0.261931168) (15, 0.391989152) (16, 0.721288104) (17, 0.046039738) (18, 0.261315932) (19, 0.476529595) (20, 0.010125895) (21, 0.37767638) (22, 0.191299246) (23, 0.186775588) (24, 0.324713227) (25, 0.042712734) (26, 0.265800336) (27, 0.101370739) (28, 0.228617828) (29, 0.066929484) (30, 0.372287525) (31, 0.19551523) (32, 0.374904443) (33, 0.287694659) (34, 0.10818096) (35, 0.111055101) (36, 0.083967211) (37, 0.220137624) (38, 0.250354849) (39, 0.140993878) (40, 0.371349626) (41, 0.393106034) (42, 0.688427429) (43, 0.308995225) (44, 0) (45, 0.584679065) (46, 0.141219549) (47, 0.47826228) (48, 0.39531394) (49, 0.28077723) (50, 0.281639918) (51, 0.432719338) (52, 0.161429384) (53, 0.139755223) (54, 0.322998626) (55, 0.280536581) (56, 0.275829303) (57, 0.255733625) (58, 0.304342158) (59, 0.134745121) (60, 0.408936866) (61, 0.28894911) (62, 0.528445391) (63, 0.321366327) (64, 0.026315789) (65, 0.198339495) (66, 0.49456345) (67, 0.224592075) (68, 0.19693498) (69, 0.493137828) (70, 0.413074406) (71, 0.358400178) (72, 0.247214795) (73, 0.863450683) (74, 0.338235294) (75, 0.867647059) (76, 0.53125) (77, 1.117647059) (78, 1.316176471) (79, 0.586111111) (80, 1) (81, 0.25) (82, 0) (83, 0.375) (84, 0.125) (85, 0.25) (86, 0.25) (87, 0) (88, 0) (89, 0) (90, 0.5) (91, 0) (92, 0) (93, 0) (94, 0) (95, 0) (96, 0) (97, 0) (98, 0) (99, 0) (100, 0) };
            
            \addplot [blue] coordinates{ (1, 0) (2, 16.83024335) (3, 2.291326631) (4, 154.2957953) (5, 56.89059852) (6, 23.09783296) (7, 17.87218466) (8, 6.673676571) (9, 0.606859014) (10, 0.100867171) (11, 0.430582273) (12, 0.491105423) (13, 0.399147414) (14, 0.261931168) (15, 0.391989152) (16, 0.721288104) (17, 0.034595424) (18, 0.102460129) (19, 0.341768665) (20, 0) (21, 0.312768164) (22, 0.175794963) (23, 0.121188593) (24, 0.227309297) (25, 0.042241358) (26, 0.242263316) (27, 0.029459733) (28, 0.19195041) (29, 0.066929484) (30, 0.234005913) (31, 0.089559593) (32, 0.123328281) (33, 0.175576473) (34, 0.10818096) (35, 0.080047162) (36, 0.017351244) (37, 0.220137624) (38, 0.185049954) (39, 0.091010828) (40, 0.238575321) (41, 0.162646127) (42, 0.324723826) (43, 0.109322475) (44, 0) (45, 0.346128078) (46, 0.091794262) (47, 0.237063209) (48, 0.224460696) (49, 0.183514968) (50, 0.196115426) (51, 0.162629068) (52, 0.019055845) (53, 0.106331555) (54, 0.211260791) (55, 0.038017932) (56, 0.062264151) (57, 0.106497953) (58, 0.146041) (59, 0.059273423) (60, 0.372384444) (61, 0.182485231) (62, 0.071263728) (63, 0.02962963) (64, 0) (65, 0.005042017) (66, 0.245225701) (67, 0.151515152) (68, 0.075722859) (69, 0.340384615) (70, 0.382771376) (71, 0.235294118) (72, 0.1875) (73, 0.388368984) (74, 0.338235294) (75, 0.867647059) (76, 0.4375) (77, 0.5) (78, 0) (79, 0.211111111) (80, 0.75) (81, 0.25) (82, 0) (83, 0.125) (84, 0) (85, 0.25) (86, 0.25) (87, 0) (88, 0) (89, 0) (90, 0.5) (91, 0) (92, 0) (93, 0) (94, 0) (95, 0) (96, 0) (97, 0) (98, 0) (99, 0) (100, 0) }; 
            
        \end{axis}
    \end{tikzpicture} 
    \label{figure_ratio_1sided_2sided_w32}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$\errLinfPosRel$ , $W=32$] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 60,
                ytick={1,15,30,45,60},
                ylabel={$\mathbb{E} \Big [\frac{errNiagara}{errOPT} \Big ]$},
        		legend style={at={(0.00,1.35)}, anchor=north west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [purple,mark=*] coordinates{ (10,1.680585683) }; \addlegendentry{$\errLinfPosRel$}
            \addplot [purple] coordinates{ (1, 1) (2, 1.175164476) (3, 1.097899161) (4, 1.445881236) (5, 1.323740684) (6, 1.36351253) (7, 1.479867646) (8, 1.556875277) (9, 1.578023944) (10, 1.68066007) (11, 1.882895476) (12, 2.121086636) (13, 2.369401995) (14, 2.650004957) (15, 3.009939943) (16, 3.330833599) (17, 3.736448557) (18, 4.200721194) (19, 4.545212224) (20, 5.113381647) (21, 5.653496631) (22, 6.207050042) (23, 6.836661955) (24, 7.417870722) (25, 8.167364103) (26, 8.51603331) (27, 9.476146536) (28, 10.15305622) (29, 11.03931887) (30, 11.94881966) (31, 12.84944513) (32, 13.3704769) (33, 14.68533011) (34, 15.38970141) (35, 16.24415257) (36, 16.8590372) (37, 17.38504957) (38, 19.12658901) (39, 20.23722953) (40, 20.41472256) (41, 21.54809782) (42, 22.19974332) (43, 25.92378207) (44, 23.44496755) (45, 26.76068775) (46, 26.21649914) (47, 26.97246857) (48, 35.93956281) (49, 31.13677335) (50, 31.69647671) (51, 26.75689406) (52, 40.82819799) (53, 24.74606973) (54, 38.30670286) (55, 28.07839508) (56, 29.87242114) (57, 33.19727138) (58, 29.42125203) (59, 29.91650249) (60, 33.8348624) (61, 24.37774657) (62, 44.68629415) (63, 42.98214063)
            %(64, 119.0844027)
            (65, 26.73362518) (66, 54.8812091) (67, 50.35539076) (68, 37.44272298)
            %(69, 779.5992748)
            (70, 46.38467605) (71, 45.14134299) (72, 29.48596058) (73, 56.76632559) (74, 30.78663094) (75, 50.37807742) (76, 34.9300725) (77, 42.25694647) (78, 25.67906442) (79, 43.66805864) (80, 33.56095856) (81, 28.46198605) (82, 28.82184288) (83, 48.55026991) (84, 24.25952216) (85, 22.28838939) (86, 20.95419562) (87, 19.82224672) (88, 10.44928207) (89, 28.86727057) (90, 5.565863852) (91, 3.659893351) (92, 2.056476414) (93, 1.628858106) (94, 2.041008787) (95, 1.153413757) (96, 1.098018857) (97, 1.022209649) (98, 1.019415077) (99, 1.001772014) (100, 1.000273283) }; 
        \end{axis}
    \end{tikzpicture}
    \label{figure_ratio_relative_w32}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.


    \caption{Comparing the error of heuristic of truncating a Niagara sequence to the optimal error, for $k=16$ and $W=16$ (a),(b) or $W=32$ (c),(d). The cases of $\errLinf$ and $\errLinfPos$ are very similar in both (a) and (c), and the ratio is almost $1$ except for when the number of rules is very small. In the relative error (b),(d), the ratio is not negligibly close to $1$, and it keeps rising until $n$ is sufficiently large to allow exact representation of the partitions. The slow drop in (b),(d) is because of an increasing percentage of partitions where both errors are $0$, and we consider the ratio to be $1$ in this case. In (d) two outlier points are omitted from the graph: (69, 779.6) and (64, 119.1)}
    \label{figure_ratio_niagara_all}
\end{figure}

\subsection{Running Time}
\label{subsection_experiments_running_time}
Theorem~\ref{theorem_runtime_l_infinity} and Theorem~\ref{theorem_runtime_one_sided} state an analytic bound on the running time. To put matters in practical perspective, we implemented the algorithms in C++ and measured their actual running time. The code was compiled by Visual Studio 2019 with Ox optimization, and ran on a Windows-10 computer with 64bit core i5-9300H processor. We emphasize that we did not try to optimize the code to improve the performance, so the resulting data should be regarded as a good estimation. %%% A real implementation on an actual switch may perform differently than ours...

Fig.~\ref{figure_running_time_micros_w16} shows the running time of each of the three algorithms for $\errLinf$, $\errLinfPos$ and $\errLinfPosRel$, in micro-seconds, for $W=16$ and $k=16$. The times were averaged over $10,000$ random ordered-partitions, the same partitions for each of the algorithms. The running time grows approximately linearly in $n$, until $n = 40$ where it rapidly drops.
Fig.~\ref{figure_running_time_relative_w16} shows the ratio between the average running time of each of the algorithms, versus the average time of the Niagara truncation heuristic.
We get similar results for $W=32$ (with $k=16$), as shown in Fig.~\ref{figure_running_time_micros_w32} and Fig.~\ref{figure_running_time_relative_w32}: for a fixed $n$ the running time is about twice slower, and the ratio compared to Niagara is approximately doubled as well.

To understand the graphs, we note that the rapid drop at about $n=40$ for $W=16$ and $n=80$ for $W=32$ happens because these values of $n$ are large enough to allow an exact representation of most of the partitions, and no lifting or binary-search happens (recall the reduction in Theorem~\ref{theorem_equivalent_rule_bound_error_bound1}). When $n$ is too small for an exact representation, then we execute a fixed number of binary-search iterations (for example, $W$ iterations for $\errLinf$). Each such iteration consists of solving a lifting problem which is independent of $n$, and then testing the solution by running $n$ steps of Niagara.
These lifting problems cause the running time to be far from $0$ even for a very small value of $n$. The subsequent tests make it increase linearly in $n$ for $n<40$ when $W=16$ and for $n<80$ when $W=32$. For the same reasons, if we divide the running time of our algorithm by the running time of Niagara for the same $n$ (Fig.~\ref{figure_running_time_relative_w16} and Fig.~\ref{figure_running_time_relative_w32}), the ratio is large for very small $n$, but stabilizes quickly. As expected, the stable ratio is around the number of binary-search iterations, in fact it is slightly larger because in each iteration we solve a lifting problem in addition to running Niagara.

It is important to note that our algorithms are  meant to run once in a period of time when either the traffic pattern or the load-balancing topology change (e.g. link failure or new server added). Such changes do not happen in the order of milliseconds, so the fact that the computation time of our algorithms takes in the order of a millisecond means that we should not be concerned of delay which they may cause. The only concern is due to remapping of addresses, which may require graceful transitioning of connections. This issue is orthogonal to the running-time question, and out of the scope of this paper.


\begin{figure}[t]
	%\centering
    \subfigure[$W=16$, Running Time] {
        \hspace*{-1.5em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=60,
        		xtick={0,10,20,30,40,50,60},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 350,
                ytick={0,50,100,150,200,250,300,350},
                ylabel=Running time ${\mu}s$,
        		legend style={at={(0.00,1.35)}, anchor=north west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black,mark=o] coordinates{ (10, 101.2432) }; \addlegendentry{$\errLinf$}
            \addplot [blue,mark=square] coordinates{ (1, 80.33169) }; \addlegendentry{$\errLinfPos$} 
            \addplot [purple,mark=*] coordinates{ (5, 182.99078) }; \addlegendentry{$\errLinfPosRel$} 
            
            \addplot [black] coordinates{ (1, 76.47261) (2, 76.29653) (3, 82.19798) (4, 83.37688) (5, 90.87292) (6, 91.53037) (7, 93.24698) (8, 96.51762) (9, 98.54793) (10, 101.2432) (11, 103.06503) (12, 109.45569) (13, 110.90822) (14, 112.29704) (15, 111.85443) (16, 113.81238) (17, 115.12773) (18, 118.81202) (19, 118.90799) (20, 121.38164) (21, 121.88423) (22, 124.74284) (23, 126.05962) (24, 127.61507) (25, 130.27323) (26, 130.54176) (27, 132.09013) (28, 133.39199) (29, 134.72207) (30, 136.15734) (31, 137.98953) (32, 138.53399) (33, 140.57383) (34, 140.64258) (35, 140.99751) (36, 142.09965) (37, 143.01682) (38, 141.91114) (39, 141.666) (40, 135.45549) (41, 125.4202) (42, 110.41623) (43, 88.96924) (44, 64.6365) (45, 43.9541) (46, 27.80583) (47, 17.3867) (48, 12.86432) (49, 10.77993) (50, 10.17731) (51, 9.97713) (52, 10.10959) (53, 9.85213) (54, 9.8682) (55, 10.03652) (56, 9.84802) (57, 9.82582) (58, 9.91262) (59, 9.73791) (60, 9.87208) (61, 9.89761) (62, 9.84588) (63, 9.75879) (64, 9.78252) (65, 9.86931) (66, 9.7726) (67, 9.87376) (68, 9.83454) (69, 9.83996) (70, 10.04253) (71, 9.72376) (72, 9.83232) (73, 10.05945) (74, 9.75966) (75, 9.84539) (76, 9.88262) (77, 10.15176) (78, 9.80105) (79, 9.79192) (80, 9.74715) (81, 9.88924) (82, 10.09338) (83, 9.83252) (84, 9.88088) (85, 9.76539) (86, 9.73948) (87, 9.80944) (88, 9.8753) (89, 9.85203) (90, 10.0982) (91, 9.81429) (92, 9.80795) (93, 9.89037) (94, 9.82327) (95, 9.86911) (96, 10.19399) (97, 9.85723) (98, 9.83723) (99, 9.80518) (100, 10.09856) };
            
            \addplot [blue] coordinates{ (1, 80.33169) (2, 86.18684) (3, 91.74168) (4, 91.93455) (5, 98.60003) (6, 99.75227) (7, 101.1638) (8, 103.34259) (9, 105.30903) (10, 106.97091) (11, 108.67537) (12, 114.6284) (13, 116.11259) (14, 116.48741) (15, 116.34678) (16, 117.80613) (17, 119.11079) (18, 122.33181) (19, 121.88421) (20, 123.98048) (21, 124.67411) (22, 127.4545) (23, 128.2983) (24, 129.61233) (25, 131.85396) (26, 132.87081) (27, 133.9316) (28, 135.28131) (29, 136.757) (30, 137.74777) (31, 139.32981) (32, 140.1199) (33, 141.39385) (34, 141.46333) (35, 142.59748) (36, 143.61403) (37, 144.1905) (38, 143.12614) (39, 142.73116) (40, 136.50446) (41, 127.07156) (42, 111.61012) (43, 89.82241) (44, 64.86775) (45, 44.34084) (46, 27.54614) (47, 16.97474) (48, 12.43558) (49, 10.37145) (50, 9.71895) (51, 9.54373) (52, 9.64554) (53, 9.36988) (54, 9.40049) (55, 9.55126) (56, 9.35716) (57, 9.3609) (58, 9.444) (59, 9.26629) (60, 9.34745) (61, 9.40387) (62, 9.36213) (63, 9.26825) (64, 9.34311) (65, 9.39266) (66, 9.2996) (67, 9.69713) (68, 9.33992) (69, 9.36284) (70, 9.56166) (71, 9.28774) (72, 9.3285) (73, 9.60434) (74, 9.25864) (75, 9.31008) (76, 9.42321) (77, 9.29923) (78, 9.3288) (79, 9.32637) (80, 9.26843) (81, 9.38669) (82, 9.61333) (83, 9.34444) (84, 9.4079) (85, 9.32933) (86, 9.65958) (87, 9.30317) (88, 9.43503) (89, 9.4368) (90, 9.31633) (91, 9.33709) (92, 9.33487) (93, 9.46744) (94, 9.33889) (95, 9.39934) (96, 9.39257) (97, 9.35473) (98, 9.3113) (99, 9.3643) (100, 9.57866) }; 
            
            \addplot [purple] coordinates{ (1, 148.85042) (2, 162.37942) (3, 170.38004) (4, 174.46248) (5, 182.99078) (6, 184.48581) (7, 187.43386) (8, 192.13722) (9, 196.16432) (10, 201.38137) (11, 206.57956) (12, 218.64197) (13, 222.78024) (14, 223.82574) (15, 224.55309) (16, 228.16538) (17, 231.89434) (18, 239.3537) (19, 239.82676) (20, 243.76086) (21, 247.75107) (22, 253.75717) (23, 256.49019) (24, 260.1583) (25, 266.48172) (26, 269.61051) (27, 274.51824) (28, 277.41204) (29, 281.81643) (30, 287.00059) (31, 292.6331) (32, 295.6521) (33, 299.46579) (34, 303.00377) (35, 307.09835) (36, 310.745) (37, 314.50736) (38, 315.47501) (39, 316.98145) (40, 303.65622) (41, 283.71724) (42, 250.12824) (43, 200.00097) (44, 141.85184) (45, 92.08632) (46, 52.83467) (47, 27.56744) (48, 16.50733) (49, 11.33285) (50, 10.13134) (51, 9.35342) (52, 9.3051) (53, 8.9964) (54, 9.05847) (55, 9.19489) (56, 9.30532) (57, 9.00077) (58, 9.0904) (59, 8.94894) (60, 8.98874) (61, 9.05121) (62, 9.05575) (63, 8.88787) (64, 8.932) (65, 9.03284) (66, 8.96375) (67, 9.02396) (68, 8.97127) (69, 9.00532) (70, 9.2026) (71, 8.88389) (72, 8.99647) (73, 9.27393) (74, 8.91391) (75, 8.93572) (76, 9.07681) (77, 8.91519) (78, 8.95951) (79, 8.99897) (80, 8.87123) (81, 9.01856) (82, 9.24062) (83, 8.96668) (84, 9.44579) (85, 8.91932) (86, 8.94957) (87, 8.93952) (88, 8.98448) (89, 9.01503) (90, 8.96317) (91, 8.976) (92, 8.95763) (93, 9.05418) (94, 8.95606) (95, 9.02755) (96, 9.03569) (97, 8.9828) (98, 8.94892) (99, 8.98945) (100, 9.21508) }; 
        \end{axis}
    \end{tikzpicture} 
    \label{figure_running_time_micros_w16}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-3.1em}  % reduces horizontal space!
    ~
    \subfigure[$W=16$, Time in ``Niagara-units''] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=60,
        		xtick={0,10,20,30,40,50,60},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 90,
                ytick={0,15,30,45,60,75,90},
                ylabel=Niagara time-units,
        		legend style={at={(0.01,0.99)}, anchor=north west,font=\footnotesize,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black,mark=o] coordinates{ (5, 35.950975) }; %\addlegendentry{$\errLinf$}
            \addplot [blue,mark=square] coordinates{ (1, 42.50106608) }; %\addlegendentry{$\errLinfPos$} 
            \addplot [purple,mark=*] coordinates{ (10, 58.40323713) }; %\addlegendentry{$\errLinfPosRel$} 
            
            \addplot [black] coordinates{ (1, 40.45934364) (2, 38.85958979) (3, 38.5726728) (4, 36.04956677) (5, 35.950975) (6, 33.9489229) (7, 32.99516645) (8, 31.76029142) (9, 30.47651048) (10, 29.36185516) (11, 28.2309616) (12, 27.77027099) (13, 26.99291519) (14, 26.59088735) (15, 25.79430634) (16, 25.1196541) (17, 24.63283873) (18, 24.04264507) (19, 23.65532587) (20, 23.29401921) (21, 22.73535348) (22, 22.37656129) (23, 21.96704063) (24, 21.71228998) (25, 21.31831363) (26, 20.92102556) (27, 20.66355621) (28, 20.2945457) (29, 19.83820888) (30, 19.67844708) (31, 19.39515281) (32, 19.08108089) (33, 18.87930974) (34, 18.58935256) (35, 18.25749347) (36, 17.33347442) (37, 17.85788295) (38, 17.52935102) (39, 17.06003273) (40, 16.42418264) (41, 14.52020983) (42, 13.13179819) (43, 10.53729657) (44, 7.654072604) (45, 5.22187017) (46, 3.256043495) (47, 2.041200393) (48, 1.465471596) (49, 1.267335451) (50, 1.194533973) (51, 1.159222888) (52, 1.14530175) (53, 1.149794599) (54, 1.157781488) (55, 1.157210341) (56, 1.159298442) (57, 1.155399764) (58, 1.152677144) (59, 1.157486408) (60, 1.162808338) (61, 1.15915125) (62, 1.159685423) (63, 1.161538086) (64, 1.157793327) (65, 1.155991253) (66, 1.15423955) (67, 1.155734097) (68, 1.151514016) (69, 1.117266954) (70, 1.149484636) (71, 1.157352117) (72, 1.160466579) (73, 1.11771915) (74, 1.161307135) (75, 1.167983686) (76, 1.149314258) (77, 1.204267707) (78, 1.155010559) (79, 1.160210337) (80, 1.164443621) (81, 1.160183297) (82, 1.154126651) (83, 1.15798635) (84, 1.150252963) (85, 1.161911527) (86, 1.156545757) (87, 1.158519561) (88, 1.160943633) (89, 1.156490861) (90, 1.197495011) (91, 1.154866913) (92, 1.151266482) (93, 1.15518359) (94, 1.158045323) (95, 1.158770583) (96, 1.196341496) (97, 1.151721817) (98, 1.161931996) (99, 1.156111716) (100, 1.150296899) };
            
            \addplot [blue] coordinates{ (1, 42.50106608) (2, 43.89695374) (3, 43.05120155) (4, 39.74963681) (5, 39.00795984) (6, 36.99845333) (7, 35.79650965) (8, 34.00613043) (9, 32.56741929) (10, 31.02296614) (11, 29.76771265) (12, 29.0826519) (13, 28.25955817) (14, 27.58312772) (15, 26.83026935) (16, 26.00111901) (17, 25.48505804) (18, 24.75490517) (19, 24.24740933) (20, 23.7927555) (21, 23.25575639) (22, 22.86298301) (23, 22.35715107) (24, 22.05210164) (25, 21.57698916) (26, 21.2942863) (27, 20.95162708) (28, 20.58199093) (29, 20.13785812) (30, 19.90830757) (31, 19.5835362) (32, 19.29951737) (33, 18.98943985) (34, 18.69783472) (35, 18.46467048) (36, 17.51820019) (37, 18.00443523) (38, 17.67943199) (39, 17.18830391) (40, 16.55137184) (41, 14.7113919) (42, 13.27378748) (43, 10.63834391) (44, 7.681456579) (45, 5.267815965) (46, 3.225633976) (47, 1.992836246) (48, 1.416630593) (49, 1.219312766) (50, 1.14073522) (51, 1.108867004) (52, 1.092730154) (53, 1.093513526) (54, 1.102907653) (55, 1.101259883) (56, 1.101514925) (57, 1.100730693) (58, 1.098184228) (59, 1.101427794) (60, 1.101013444) (61, 1.101327256) (62, 1.102707497) (63, 1.103151658) (64, 1.105787712) (65, 1.100161288) (66, 1.098373628) (67, 1.135059368) (68, 1.093599578) (69, 1.063092912) (70, 1.094443459) (71, 1.105455662) (72, 1.101002864) (73, 1.06715126) (74, 1.101690498) (75, 1.104478497) (76, 1.095886476) (77, 1.103135061) (78, 1.099357977) (79, 1.105048947) (80, 1.10725332) (81, 1.101225266) (82, 1.099235376) (83, 1.100504649) (84, 1.095192417) (85, 1.110027973) (86, 1.147057776) (87, 1.0987278) (88, 1.109185342) (89, 1.107748653) (90, 1.104776959) (91, 1.098713845) (92, 1.095735902) (93, 1.105785863) (94, 1.10094275) (95, 1.10361306) (96, 1.102288824) (97, 1.093009561) (98, 1.099811369) (99, 1.104128322) (100, 1.091076638) }; 
            
            \addplot [purple] coordinates{ (1, 78.75225251) (2, 82.70359939) (3, 79.95346764) (4, 75.43214403) (5, 72.39447084) (6, 68.42640906) (7, 66.32291372) (8, 63.22507848) (9, 60.6649369) (10, 58.40323713) (11, 56.58504758) (12, 55.47218931) (13, 54.22040065) (14, 52.99983898) (15, 51.78329721) (16, 50.35862903) (17, 49.61633378) (18, 48.43530188) (19, 47.71067243) (20, 46.77948127) (21, 46.21359261) (22, 45.51934899) (23, 44.69575923) (24, 44.26305178) (25, 43.60789152) (26, 43.20861286) (27, 42.9443372) (28, 42.20606743) (29, 41.49827272) (30, 41.47940848) (31, 41.13111837) (32, 40.72185921) (33, 40.21877619) (34, 40.04934997) (35, 39.76556835) (36, 37.90502306) (37, 39.27115442) (38, 38.96855588) (39, 38.17227784) (40, 36.81877507) (41, 32.84665354) (42, 29.74774241) (43, 23.68761984) (44, 16.79769608) (45, 10.9401127) (46, 6.186903379) (47, 3.23642033) (48, 1.880474307) (49, 1.332339131) (50, 1.18913837) (51, 1.086755264) (52, 1.054162168) (53, 1.049926476) (54, 1.062780332) (55, 1.060170436) (56, 1.095412375) (57, 1.058383681) (58, 1.057066276) (59, 1.06370632) (60, 1.058761864) (61, 1.060025742) (62, 1.066620888) (63, 1.057877002) (64, 1.057131495) (65, 1.058015609) (66, 1.058706462) (67, 1.056264105) (68, 1.050434809) (69, 1.022498714) (70, 1.053344856) (71, 1.057388181) (72, 1.061814787) (73, 1.030438957) (74, 1.060670892) (75, 1.060067217) (76, 1.055601363) (77, 1.057577742) (78, 1.055838778) (79, 1.066256466) (80, 1.059801808) (81, 1.058037086) (82, 1.056617883) (83, 1.056015452) (84, 1.099603268) (85, 1.061243916) (86, 1.062745363) (87, 1.055779819) (88, 1.056218531) (89, 1.05823874) (90, 1.062897482) (91, 1.056223671) (92, 1.051455113) (93, 1.057517581) (94, 1.0558117) (95, 1.059959751) (96, 1.060406268) (97, 1.049553144) (98, 1.057008576) (99, 1.059930411) (100, 1.049662323) }; 
        \end{axis}
    \end{tikzpicture}
    \label{figure_running_time_relative_w16}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    
    \subfigure[$W=32$, Running Time] {
        \hspace*{-1.5em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 1100,
                ytick={0,200,400,600,800,1000},
                ylabel=Running time ${\mu}s$,
        		legend style={at={(0.00,1.35)}, anchor=north west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black,mark=o] coordinates{ (5, 165.05593) }; %\addlegendentry{$\errLinf$}
            \addplot [blue,mark=square] coordinates{ (1, 148.93495) }; %\addlegendentry{$\errLinfPos$} 
            \addplot [purple,mark=*] coordinates{ (10, 368.45916) }; %\addlegendentry{$\errLinfPosRel$} 
            
            \addplot [black] coordinates{ (1, 136.81479) (2, 142.45338) (3, 154.31372) (4, 154.93881) (5, 165.05593) (6, 168.7069) (7, 174.50182) (8, 200.93901) (9, 211.65727) (10, 192.45977) (11, 194.26729) (12, 200.93081) (13, 208.01412) (14, 211.30305) (15, 214.04735) (16, 217.41275) (17, 221.08474) (18, 226.01619) (19, 230.11478) (20, 234.12943) (21, 239.79596) (22, 243.32662) (23, 248.1673) (24, 251.44946) (25, 255.44919) (26, 259.99979) (27, 265.42243) (28, 268.84813) (29, 273.02223) (30, 276.91753) (31, 279.82488) (32, 285.35715) (33, 289.74344) (34, 293.24313) (35, 297.25639) (36, 300.79816) (37, 317.69447) (38, 315.81252) (39, 316.05159) (40, 315.14702) (41, 320.99671) (42, 325.0727) (43, 327.03814) (44, 330.07365) (45, 334.34384) (46, 339.7822) (47, 339.86881) (48, 345.05709) (49, 346.82412) (50, 349.42882) (51, 353.23029) (52, 355.50431) (53, 358.26361) (54, 361.22269) (55, 364.16646) (56, 367.72208) (57, 369.13325) (58, 371.72685) (59, 374.63092) (60, 376.90614) (61, 379.51665) (62, 380.08211) (63, 383.46204) (64, 386.16597) (65, 387.49307) (66, 389.87912) (67, 391.28158) (68, 393.75626) (69, 395.23982) (70, 397.32877) (71, 398.9587) (72, 401.84153) (73, 401.86884) (74, 402.66328) (75, 403.126) (76, 406.37754) (77, 406.57785) (78, 407.98049) (79, 407.55482) (80, 407.95267) (81, 405.51573) (82, 402.46515) (83, 396.29454) (84, 381.85157) (85, 361.61999) (86, 330.92225) (87, 288.37388) (88, 242.81548) (89, 193.06991) (90, 148.04145) (91, 107.37695) (92, 73.66954) (93, 50.43711) (94, 35.71356) (95, 28.01387) (96, 23.05942) (97, 20.38499) (98, 19.27488) (99, 19.21971) (100, 18.62) };
            
            \addplot [blue] coordinates{ (1, 148.93495) (2, 169.80336) (3, 181.56012) (4, 181.91435) (5, 190.46236) (6, 194.6619) (7, 198.31484) (8, 227.32911) (9, 237.10528) (10, 215.06152) (11, 215.46645) (12, 220.64361) (13, 227.54833) (14, 231.21373) (15, 233.44506) (16, 236.87704) (17, 240.26219) (18, 244.27163) (19, 247.1847) (20, 250.81165) (21, 255.35377) (22, 259.57767) (23, 262.81252) (24, 266.97722) (25, 271.74925) (26, 274.56981) (27, 279.54925) (28, 282.81888) (29, 287.5818) (30, 291.29965) (31, 294.47813) (32, 298.74771) (33, 302.8215) (34, 306.43225) (35, 309.76289) (36, 313.36541) (37, 330.93685) (38, 328.04597) (39, 328.44723) (40, 327.19199) (41, 332.16545) (42, 336.47238) (43, 338.70961) (44, 340.09411) (45, 345.08397) (46, 348.94389) (47, 351.06569) (48, 354.79549) (49, 355.88065) (50, 359.98664) (51, 362.31826) (52, 365.10796) (53, 367.72687) (54, 370.80589) (55, 374.14355) (56, 377.01462) (57, 378.21581) (58, 380.48718) (59, 383.54651) (60, 385.84728) (61, 388.20076) (62, 388.48687) (63, 391.45596) (64, 393.86291) (65, 395.30015) (66, 397.6372) (67, 401.14865) (68, 400.81211) (69, 402.4633) (70, 404.00647) (71, 405.77504) (72, 409.50074) (73, 409.16173) (74, 409.88501) (75, 410.85912) (76, 412.40412) (77, 412.86939) (78, 414.84654) (79, 413.70134) (80, 415.27563) (81, 413.22165) (82, 409.52176) (83, 402.42761) (84, 387.67484) (85, 368.94793) (86, 335.84588) (87, 293.12193) (88, 247.30269) (89, 196.0505) (90, 150.36897) (91, 108.5088) (92, 73.85288) (93, 50.43389) (94, 35.62099) (95, 27.55902) (96, 22.54448) (97, 19.72429) (98, 18.64588) (99, 18.56001) (100, 17.96761) }; 
            
            \addplot [purple] coordinates{ (1, 238.32324) (2, 279.64704) (3, 296.0306) (4, 304.68877) (5, 313.72076) (6, 322.35931) (7, 333.66126) (8, 381.8363) (9, 403.89559) (10, 368.45916) (11, 372.93961) (12, 386.73408) (13, 403.11898) (14, 410.73362) (15, 416.89315) (16, 425.79915) (17, 436.00337) (18, 443.72967) (19, 454.7701) (20, 464.88017) (21, 478.39363) (22, 487.49399) (23, 497.28662) (24, 510.54332) (25, 521.00108) (26, 533.1096) (27, 546.07685) (28, 557.62633) (29, 568.40471) (30, 581.11112) (31, 591.08121) (32, 602.03235) (33, 612.31369) (34, 621.7447) (35, 633.44666) (36, 641.4068) (37, 677.43084) (38, 677.37554) (39, 678.08032) (40, 679.56819) (41, 692.08498) (42, 703.1355) (43, 708.2178) (44, 718.48428) (45, 727.89195) (46, 739.90074) (47, 745.24675) (48, 757.4221) (49, 763.67254) (50, 774.37312) (51, 784.67514) (52, 789.97573) (53, 799.55662) (54, 808.9567) (55, 817.96368) (56, 828.00523) (57, 834.20904) (58, 843.20856) (59, 852.05188) (60, 859.91964) (61, 869.24207) (62, 875.4893) (63, 886.38969) (64, 895.5684) (65, 900.68202) (66, 911.47093) (67, 918.39267) (68, 926.54927) (69, 933.39586) (70, 943.21033) (71, 950.70559) (72, 961.92467) (73, 965.6894) (74, 973.56838) (75, 979.754) (76, 987.49782) (77, 994.09217) (78, 1003.50576) (79, 1006.4694) (80, 1013.50131) (81, 1011.569) (82, 1008.74157) (83, 995.68677) (84, 962.42502) (85, 916.58938) (86, 835.89729) (87, 728.51203) (88, 610.10326) (89, 481.75821) (90, 361.42497) (91, 254.4793) (92, 164.06069) (93, 103.39515) (94, 64.01946) (95, 42.7172) (96, 29.44001) (97, 22.36452) (98, 19.34609) (99, 18.87257) (100, 17.52711) }; 
        \end{axis}
    \end{tikzpicture}
    \label{figure_running_time_micros_w32}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-1.6em}  % reduces horizontal space!
    ~
    \subfigure[$W=32$, Time in ``Niagara-units''] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.25\textwidth,
        		height=0.2\textwidth,
        		xmin=0, xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel=Number of rules $n$,
        		ymin=0, ymax = 140,
                ytick={0,20,40,60,80,100,120,140},
                ylabel=Niagara time-units,
        		legend style={at={(0.01,0.99)}, anchor=north west,font=\footnotesize,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black,mark=o] coordinates{ (5, 65.83311113) }; %\addlegendentry{$\errLinf$}
            \addplot [blue,mark=square] coordinates{ (10, 60.16043968) }; %\addlegendentry{$\errLinfPos$} 
            \addplot [purple,mark=*] coordinates{ (10, 103.8505581) }; %\addlegendentry{$\errLinfPosRel$} 
            
            \addplot [black] coordinates{ (1, 75.49587478) (2, 72.06044119) (3, 71.54419479) (4, 58.3874529) (5, 65.83311113) (6, 62.96133234) (7, 60.38027379) (8, 58.20964286) (9, 56.08524842) (10, 54.31430109) (11, 53.33175894) (12, 51.88427326) (13, 50.43119221) (14, 49.52154497) (15, 48.42012162) (16, 47.49578984) (17, 46.59105827) (18, 45.80329543) (19, 44.89235295) (20, 44.09515193) (21, 43.12964478) (22, 43.03922195) (23, 42.50389187) (24, 42.15022245) (25, 41.61709054) (26, 41.20241456) (27, 40.53541251) (28, 40.30940868) (29, 39.72415566) (30, 39.20090737) (31, 37.29508496) (32, 38.63567912) (33, 38.57179329) (34, 37.76775057) (35, 37.6625083) (36, 37.26902298) (37, 35.62022339) (38, 36.63306722) (39, 36.38473854) (40, 36.07189495) (41, 35.82492748) (42, 35.41811252) (43, 35.21393032) (44, 34.82747583) (45, 33.34924468) (46, 34.2310947) (47, 33.99405038) (48, 33.53647851) (49, 33.26002596) (50, 32.94718653) (51, 32.7570289) (52, 32.42967351) (53, 32.22668532) (54, 31.90584343) (55, 31.67790815) (56, 31.46624251) (57, 31.2153726) (58, 30.98284257) (59, 30.73752509) (60, 30.39150706) (61, 30.18072064) (62, 29.85144474) (63, 29.41827179) (64, 29.41503088) (65, 28.49462894) (66, 28.88849176) (67, 28.50122402) (68, 28.35831594) (69, 28.1102516) (70, 27.80009202) (71, 27.49167308) (72, 27.32918335) (73, 27.22612509) (74, 27.03337219) (75, 26.82044579) (76, 26.39678421) (77, 26.27760175) (78, 26.07112272) (79, 25.89530591) (80, 25.52984109) (81, 25.30081375) (82, 24.6309016) (83, 24.18263739) (84, 22.70550026) (85, 21.79649951) (86, 19.78823385) (87, 17.19326029) (88, 14.44715955) (89, 11.31711558) (90, 8.762813689) (91, 6.400971532) (92, 4.359731545) (93, 3.016825362) (94, 2.141705012) (95, 1.653863517) (96, 1.360930263) (97, 1.206618029) (98, 1.137864079) (99, 1.12101096) (100, 1.100653206) };
            
            \addplot [blue] coordinates{ (1, 81.38303901) (2, 85.16229346) (3, 83.55117413) (4, 67.54365808) (5, 75.2015716) (6, 71.57621565) (7, 67.93132786) (8, 65.13407191) (9, 62.22728141) (10, 60.16043968) (11, 58.53732829) (12, 56.40893595) (13, 55.0814749) (14, 53.63492624) (15, 52.42516316) (16, 51.14908798) (17, 49.95632597) (18, 48.87660272) (19, 48.02716592) (20, 46.99040451) (21, 45.79284972) (22, 45.62047053) (23, 44.88243665) (24, 44.48131033) (25, 43.81170503) (26, 43.35987962) (27, 42.49659872) (28, 42.1124583) (29, 41.62329872) (30, 40.9843184) (31, 38.92053194) (32, 40.27696473) (33, 39.97889492) (34, 39.30448964) (35, 39.00100196) (36, 38.7999052) (37, 36.86113199) (38, 37.85728098) (39, 37.58288874) (40, 37.12339575) (41, 36.88120727) (42, 36.50074423) (43, 36.18933853) (44, 35.83759287) (45, 34.31384317) (46, 35.1554262) (47, 34.86463396) (48, 34.37634902) (49, 34.09319963) (50, 33.77996546) (51, 33.54329169) (52, 33.19718707) (53, 33.05020432) (54, 32.68051953) (55, 32.3421825) (56, 32.1315478) (57, 31.88822902) (58, 31.61013767) (59, 31.27153312) (60, 31.00136033) (61, 30.6840431) (62, 30.4539815) (63, 29.97598687) (64, 29.92055742) (65, 28.91451812) (66, 29.49683634) (67, 28.99611347) (68, 28.91439841) (69, 28.59001838) (70, 28.18302367) (71, 27.96910087) (72, 27.80904615) (73, 27.67646684) (74, 27.38680506) (75, 27.13410969) (76, 26.77905415) (77, 26.61581446) (78, 26.40247315) (79, 26.1955221) (80, 25.91719674) (81, 25.72463656) (82, 25.00965434) (83, 24.55613403) (84, 23.01123599) (85, 22.14980341) (86, 20.08545196) (87, 17.40384669) (88, 14.70726835) (89, 11.42132769) (90, 8.867986242) (91, 6.453685813) (92, 4.381187993) (93, 3.006279772) (94, 2.104994321) (95, 1.622039147) (96, 1.329020651) (97, 1.177892383) (98, 1.10395434) (99, 1.096699515) (100, 1.060767603) }; 
            
            \addplot [purple] coordinates{ (1, 130.3609526) (2, 140.8129393) (3, 136.5294985) (4, 114.029939) (5, 124.7279532) (6, 119.39658) (7, 114.6887509) (8, 109.6922104) (9, 106.1909633) (10, 103.8505581) (11, 101.8230024) (12, 99.30982754) (13, 97.28404808) (14, 95.61630306) (15, 94.21082458) (16, 92.22472177) (17, 90.79346814) (18, 89.73595761) (19, 88.69491339) (20, 87.38398999) (21, 86.05780231) (22, 85.96866656) (23, 85.36280431) (24, 84.86004926) (25, 84.53049848) (26, 83.92700542) (27, 83.4533367) (28, 83.0764159) (29, 82.66539322) (30, 81.86639521) (31, 78.36071654) (32, 81.54210327) (33, 81.06151419) (34, 80.05657004) (35, 79.93768709) (36, 79.33054982) (37, 76.06731165) (38, 78.3406728) (39, 77.75940452) (40, 77.34906599) (41, 77.02699996) (42, 76.59267234) (43, 76.06636136) (44, 75.57423564) (45, 72.54264518) (46, 74.72846269) (47, 74.3563101) (48, 73.74261503) (49, 73.31771692) (50, 72.95326709) (51, 72.61041323) (52, 72.22746849) (53, 72.07476932) (54, 71.48118707) (55, 71.18579064) (56, 70.97645327) (57, 70.50977612) (58, 70.21053923) (59, 69.79623432) (60, 69.46249971) (61, 69.23801105) (62, 68.59573889) (63, 68.07610694) (64, 68.15673882) (65, 66.21367301) (66, 67.5255518) (67, 66.85541869) (68, 66.8544023) (69, 66.48479279) (70, 65.99521021) (71, 65.60524747) (72, 65.50592318) (73, 65.50190878) (74, 65.24475185) (75, 64.76765156) (76, 64.55107122) (77, 64.27660834) (78, 64.13906768) (79, 63.83382137) (80, 63.45212069) (81, 63.05134369) (82, 61.84147968) (83, 60.91473033) (84, 57.27767185) (85, 55.25506357) (86, 50.29335726) (87, 43.48114267) (88, 36.60048923) (89, 28.1544804) (90, 21.41755698) (91, 15.17862688) (92, 9.784921211) (93, 6.14692986) (94, 3.77900055) (95, 2.514342717) (96, 1.762873119) (97, 1.348940816) (98, 1.168752331) (99, 1.094845842) (100, 1.045118239) }; 
        \end{axis}
    \end{tikzpicture}
    \label{figure_running_time_relative_w32}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    
    
    \caption{Running time of the algorithms, for fixed $k=16$, $W=16$ (top) or $W=32$ (bottom) and $n \in [1,60]$ or $n \in [1,100]$ respectively. For each $n$, the running time was averaged over $10,000$ random ordered-partitions (same set for all three algorithm). (a)+(c) show the running time in $\mu$s, (b)+(d) normalize the running time in ``units'' of Niagara, to show the loss in running time compared to the heuristic of truncating a Niagara sequence. These units grow from $0.8{\mu}s$ ($n\approx 1$) to $18{\mu}s$ ($n\approx 100$), monotonous in $n$, not affected much by $W$. At about $n \ge 40$ for $W=16$ and $n \ge 80$ for $W=32$ many partitions can be represented exactly for, so the approximation-logic is not required and the running-time drops.}
    \label{figure_running_time_all}
\end{figure}


\subsection{Unreachable Targets (Degeneracy Concerns)}
\label{subsection_experiments_degeneracy}
Our algorithms find the closest partition (in one of $\errLinf$, $\errLinfPos$ or $\errLinfPosRel$) that can be represented by $n$ rules to a given partition. As in Example~\ref{figure_tcam_trie_all}, such an optimal partition may be ``degenerate'' in the sense that it does not map any address to some of the $k$ targets.

Such a degeneracy is likely only when $\frac{n}{k}$ is very small. Fig.~\ref{figure_degeneracy} shows that for $n < 2k$ there is high probability to encounter such a degeneracy, but for $n \ge 3k$ this probability is already low. We note that if the objective is $\errLinfPosRel$ then it is slightly more likely to get a degenerate partition than for $\errLinfPos$, which in turn has higher chances for degeneracy than $\errLinf$, but overall these chances for the different objectives are  similar, and the degeneracy happens mostly when $\frac{n}{k}$ is no more than $2.5$. One can avoid degenerate partitions by incorporating various heuristics that postprocess the rules.

We note that in real-life situations the desired partitions are likely to be more balanced than in a uniform ordered-partition (which is skewed toward having few heavy parts), and therefore the probability of degeneracy is even smaller because loosely speaking each target is more likely to get ``its fair share'' of rules.

\begin{figure}[!t]%[!ht]
	\centering
	
	\subfigure[$\errLinf$]{
    \includegraphics[width=1.0\linewidth]{BW-degeneracy_twoSided-withAxes.png}
    \label{figure_degeneracy_2sided}
    }
    ~
    \subfigure[$\errLinfPos$]{
    \includegraphics[width=1.0\linewidth]{BW-degeneracy_oneSided-withAxes.png}
    \label{figure_degeneracy_1sided}
    }
    ~
    \subfigure[$\errLinfPosRel$]{
    \includegraphics[width=1.0\linewidth]{BW-degeneracy_oneSidedRelative-withAxes.png}
    \label{figure_degeneracy_1sidedRelative}
    }
	
	
    \caption{A visualization of the probability that approximating a partition $P$ with $k$ targets using $n$ rules will result in a partition $P'$ with less than $k$ targets. $W=32$ is fixed, each large pixel represent a pair of $n$ and $k$ for $k=5,10,\ldots,100$ and $n=5,10,\ldots,600$. The dashed blue lines mark a constant integer ratio $\frac{n}{k} = c$ for $c=1,\ldots,6$. White ``pixels'' represent 100\% degeneracy, black represent 0\%, gray are intermediate values. Each pixel was computed by sampling 100 random ordered-partitions, note that when $n<k$ degeneracy is guaranteed for any partition.}
    \label{figure_degeneracy}
\end{figure}

\subsection{Real Data Partitions}
\label{subsection_experiments_real_data_partitions}
In this section we provide results for ``real data partitions''. 
%As we do not have a data-center of our own with actual details of the relative power of each target (CPU power, memory, etc.), we resorted to consider public captures, from which we derived partitions according to some arbitrary assumptions. 
We use the data of \cite{ftp_packet_captures},\footnote{Available for download at: https://ee.lbl.gov/anonymized-traces.html} containing 3.2 million packets in 22 thousand connections between 5832 distinct clients to 320 distinct servers. %%% 10 day traffic of FTP from January 2003.

We made the assumption that the data traffic approximates the target partition in the following concrete sense.\footnote{Using any captured data can only be done if we assume that the data represents closely enough a desired partition.} We sliced the data into windows of one hour each, to get a total of 240 time frames. From each frame we extracted three partitions, according to three types of loads on the servers that communicated in the particular frame as follows: (1) the number of unique clients per server (``load balancing sessions''); (2) the number of incoming packets (``load balancing requests''); (3) the number of outgoing bytes (``load balancing data-processing''). Overall, we get 720 partitions with sums that range in $[18,298]$ (connections), $[2143,16306]$ (packets) and $[196637,1618691]$ (sent bytes). The number of parts in the partitions (targets) varies among $k \in \{4{-}18, 20, 21, 23, 28, 58, 64, 67, 260\}$.

Most of the partitions do not sum to a power of $2$, as could be expected. Since our model requires a universe of $2^W$ addresses, we normalized the partitions to be non-integer partitions that sum to a power of $2$ as explained in Section~\ref{section_non_integer_partitions_approximation} (Problem \ref{problem_tcam_approx_by_rules_non_integer}). On one hand we didn't want to normalize partitions with small sums using a large $W$, and on the other hand we wanted to have only a few values of $W$, to be able to compare partitions with similar parameters. Therefore, we normalized the sum of each partition to a multiple of $256$. All but one of the connections-partitions end up with $W=8$ (all sums are $\le 112$ except for one exception of $298$), all packets-partitions end up with $W=16$, and all bytes-partitions end up with $W=24$.

For each normalized partition we check the trade-off between error and percentage of rules out of the maximum necessary $n^*(P)$ for the best possible integer representation.\footnote{$n^*(P) = \lambda(P)$ if $P$ is integer, or $n^*(P) = \lambda(P')$ for an integer partition $P'$ closest to $P$.} The percentages that we sampled were multiples of $10$, that is, $\floor{\frac{i \cdot n^*(P)}{10}}$ for $i=1,\ldots,10$. Fig.~\ref{figure_real_data_all} shows this trade-off. To reduce cluttering, the data in the figure only relies on 72 out of the 240 time-frames, covering the first three days. The $x$-axis is the number of rules used to approximate a partition, in percentage ($100$ means ``best representation''). The $y$-axis for $\errLinf$ and $\errLinfPos$ is $\frac{\lg (\text{error})}{W}$, where we divide by $W$ to normalize the presentation for partitions with different sums. We see that just like the results for randomly ordered-partitions, the error decreases exponentially with the increase in the number of rules (linear in the graph, due to log-scale). The division by $W=8$, $W=16$ or $W=24$ (depending on the case) can be thought of as ``error per width unit''.

Regarding $\errLinfPosRel$, in all of the 720 partitions we derived, $\max_{1 \le i \le k}{p_i} > 0.0838 \sum_{i=1}^{k}{p_i}$, which means that even if we only use one rule, the $\errLinfPosRel$ error would be less than $\frac{\sum_{i=1}^{k}{p_i} - \max_{1 \le i \le k}{p_i}}{\max_{1 \le i \le k}{p_i}} \le \frac{1}{0.0838} - 1 < 11$ (allocating the match-all rule to the maximum weight). In each of the approximations that we computed, the maximum relative error is less than $2.6$, so taking $\lg$ of the relative error yields values that are mostly negative. Since the relative error is computed by dividing the absolute error by a part of the partition, which can be of the order of $2^W$, a non-zero relative error can get as low as $\approx 2^{-W}$. This is why its logarithm, divided by $W$, reaches values of approximately $-1$. (when the error is zero, its logarithm is undefined no matter whether the error is relative or absolute).

\begin{figure}[t]
	%\centering
    \subfigure {
        \hspace*{-1.0em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		%xlabel={\% of required rules},
        		ymin=-0.2, ymax = 1,
                ytick={-0.2,0,0.2,0.4,0.6,0.8,1.0},
                ylabel={$(\lg{\text{error}})/W$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.99,0.99)}, anchor=north east,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black,mark=*,only marks,mark size=1pt] coordinates{
            (10.000,0.790) (20.000,0.625) (30.000,0.500) (40.000,0.500) (50.000,0.375) (60.000,0.250) (70.000,0.250) (80.000,0.250) (90.000,0.250) (100.000,-100.000) (9.091,0.802) (18.182,0.613) (27.273,0.552) (36.364,0.474) (45.455,0.319) (54.545,0.314) (63.636,0.151) (72.727,0.113) (81.818,0.052) (100.000,-0.073) (6.250,0.849) (18.750,0.586) (25.000,0.508) (37.500,0.411) (50.000,0.346) (56.250,0.273) (68.750,0.242) (75.000,0.242) (87.500,0.032) (100.000,-0.080) (7.692,0.871) (15.385,0.736) (23.077,0.596) (38.462,0.438) (46.154,0.330) (53.846,0.330) (69.231,0.146) (76.923,0.146) (84.615,0.043) (100.000,-0.121) (7.692,0.871) (15.385,0.741) (23.077,0.606) (38.462,0.461) (46.154,0.352) (53.846,0.330) (69.231,0.146) (76.923,0.121) (84.615,0.043) (100.000,-0.121) (10.000,0.861) (20.000,0.721) (30.000,0.563) (40.000,0.352) (50.000,0.341) (60.000,0.181) (70.000,0.102) (80.000,0.080) (90.000,-0.056) (100.000,-0.104) (10.000,0.813) (20.000,0.622) (30.000,0.592) (40.000,0.425) (50.000,0.378) (60.000,0.253) (70.000,0.253) (80.000,0.223) (90.000,0.063) (100.000,-0.128) (7.692,0.859) (15.385,0.717) (23.077,0.552) (38.462,0.354) (46.154,0.302) (53.846,0.302) (69.231,0.104) (76.923,-0.021) (84.615,-0.073) (100.000,-0.106) (7.143,0.852) (14.286,0.701) (28.571,0.509) (35.714,0.484) (50.000,0.390) (57.143,0.220) (64.286,0.197) (78.571,-0.003) (85.714,-0.070) (100.000,-0.170) (9.524,0.734) (19.048,0.591) (28.571,0.469) (38.095,0.399) (47.619,0.285) (57.143,0.263) (66.667,0.263) (76.190,0.236) (85.714,0.097) (100.000,-0.062) (10.000,0.705) (20.000,0.519) (30.000,0.463) (40.000,0.338) (50.000,0.259) (60.000,0.208) (70.000,0.208) (80.000,0.027) (90.000,0.027) (100.000,-0.070) (10.000,0.708) (20.000,0.529) (30.000,0.428) (40.000,0.355) (50.000,0.268) (60.000,0.268) (70.000,0.183) (80.000,0.029) (90.000,-0.034) (100.000,-0.096) (7.692,0.821) (15.385,0.618) (23.077,0.486) (38.462,0.338) (46.154,0.281) (53.846,0.281) (69.231,0.104) (76.923,-0.037) (84.615,-0.045) (100.000,-0.132) (10.000,0.828) (20.000,0.638) (30.000,0.578) (40.000,0.412) (50.000,0.361) (60.000,0.236) (70.000,0.162) (80.000,-0.014) (90.000,-0.088) (100.000,-0.112) (7.143,0.827) (14.286,0.636) (28.571,0.416) (35.714,0.407) (50.000,0.306) (57.143,0.306) (64.286,0.192) (78.571,0.077) (85.714,0.067) (100.000,-0.107) (7.692,0.866) (15.385,0.733) (23.077,0.588) (38.462,0.417) (46.154,0.287) (53.846,0.263) (69.231,0.253) (76.923,0.247) (84.615,0.116) (100.000,-0.066) (12.500,0.807) (12.500,0.807) (25.000,0.570) (37.500,0.469) (50.000,0.365) (50.000,0.365) (62.500,0.307) (75.000,0.134) (87.500,0.070) (100.000,-0.116) (6.250,0.879) (18.750,0.640) (25.000,0.488) (37.500,0.354) (50.000,0.314) (56.250,0.314) (68.750,0.151) (75.000,0.151) (87.500,0.012) (100.000,-0.067) (7.692,0.856) (15.385,0.711) (23.077,0.535) (38.462,0.395) (46.154,0.291) (53.846,0.291) (69.231,0.004) (76.923,0.004) (84.615,0.004) (100.000,-0.144) (9.091,0.817) (18.182,0.605) (27.273,0.544) (36.364,0.457) (45.455,0.306) (54.545,0.306) (63.636,0.306) (72.727,0.169) (81.818,0.067) (100.000,-0.107) (12.500,0.839) (12.500,0.839) (25.000,0.668) (37.500,0.443) (50.000,0.391) (50.000,0.391) (62.500,0.233) (75.000,0.193) (87.500,-0.017) (100.000,-0.182) (10.000,0.881) (20.000,0.730) (30.000,0.583) (40.000,0.404) (50.000,0.393) (60.000,0.268) (70.000,0.091) (80.000,0.058) (90.000,-0.034) (100.000,-0.096) (12.500,0.742) (12.500,0.742) (25.000,0.535) (37.500,0.423) (50.000,0.310) (50.000,0.310) (62.500,0.185) (75.000,0.160) (87.500,-0.044) (100.000,-0.103) (11.111,0.830) (11.111,0.830) (22.222,0.644) (33.333,0.519) (44.444,0.394) (55.556,0.354) (66.667,0.205) (77.778,0.019) (88.889,-0.021) (100.000,-0.045) (14.286,0.851) (14.286,0.851) (28.571,0.698) (28.571,0.698) (42.857,0.500) (57.143,0.500) (57.143,0.500) (71.429,0.375) (85.714,0.375) (100.000,-100.000) (8.333,0.821) (16.667,0.620) (25.000,0.597) (33.333,0.439) (50.000,0.390) (58.333,0.359) (66.667,0.216) (75.000,0.049) (83.333,-0.016) (100.000,-0.068) (9.091,0.852) (18.182,0.702) (27.273,0.562) (36.364,0.510) (45.455,0.404) (54.545,0.340) (63.636,0.171) (72.727,0.029) (81.818,-0.011) (100.000,-0.115) (8.333,0.875) (16.667,0.750) (25.000,0.625) (33.333,0.445) (50.000,0.344) (58.333,0.344) (66.667,0.219) (75.000,0.182) (83.333,0.042) (100.000,-0.083) (10.000,0.855) (20.000,0.707) (30.000,0.594) (40.000,0.432) (50.000,0.344) (60.000,0.195) (70.000,0.182) (80.000,0.009) (90.000,-0.055) (100.000,-0.135) (5.882,0.883) (17.647,0.607) (29.412,0.462) (35.294,0.414) (47.059,0.326) (58.824,0.326) (64.706,0.133) (76.471,0.133) (88.235,0.116) (100.000,-0.061) (12.500,0.772) (12.500,0.772) (25.000,0.578) (37.500,0.464) (50.000,0.380) (50.000,0.380) (62.500,0.295) (75.000,0.065) (87.500,0.022) (100.000,-0.150) (11.111,0.802) (11.111,0.802) (22.222,0.552) (33.333,0.552) (44.444,0.387) (55.556,0.387) (66.667,0.302) (77.778,0.052) (88.889,0.052) (100.000,-0.113) (5.263,0.861) (15.789,0.559) (26.316,0.522) (36.842,0.405) (47.368,0.339) (57.895,0.339) (68.421,0.170) (78.947,0.111) (89.474,0.065) (100.000,-0.103) (9.091,0.915) (18.182,0.790) (27.273,0.625) (36.364,0.573) (45.455,0.500) (54.545,0.500) (63.636,0.375) (72.727,0.375) (81.818,0.375) (100.000,-100.000) (8.333,0.853) (16.667,0.702) (25.000,0.512) (33.333,0.478) (50.000,0.322) (58.333,0.322) (66.667,0.159) (75.000,0.129) (83.333,0.112) (100.000,-0.098) (12.500,0.875) (12.500,0.875) (25.000,0.750) (37.500,0.552) (50.000,0.387) (50.000,0.387) (62.500,0.387) (75.000,0.262) (87.500,0.052) (100.000,-0.113) (10.000,0.730) (20.000,0.582) (30.000,0.425) (40.000,0.400) (50.000,0.306) (60.000,0.306) (70.000,0.169) (80.000,0.121) (90.000,0.067) (100.000,-0.107) (8.696,0.765) (17.391,0.548) (26.087,0.492) (39.130,0.359) (47.826,0.310) (56.522,0.310) (69.565,0.160) (78.261,0.160) (86.957,0.081) (100.000,-0.103) (12.500,0.808) (12.500,0.808) (25.000,0.575) (37.500,0.393) (50.000,0.393) (50.000,0.393) (62.500,0.143) (75.000,0.029) (87.500,-0.034) (100.000,-0.058) (14.286,0.812) (14.286,0.812) (28.571,0.590) (28.571,0.590) (42.857,0.421) (57.143,0.364) (57.143,0.364) (71.429,0.227) (85.714,0.077) (100.000,-0.115) (10.000,0.798) (20.000,0.581) (30.000,0.535) (40.000,0.397) (50.000,0.310) (60.000,0.310) (70.000,0.100) (80.000,0.081) (90.000,-0.025) (100.000,-0.117) (9.091,0.346) (19.318,0.200) (29.545,0.200) (39.773,0.200) (50.000,0.200) (59.091,0.200) (69.318,0.200) (79.545,0.200) (89.773,0.200) (100.000,0.200) (7.143,0.854) (14.286,0.705) (28.571,0.460) (35.714,0.401) (50.000,0.314) (57.143,0.314) (64.286,0.151) (78.571,0.095) (85.714,0.095) (100.000,-0.067) (11.111,0.900) (11.111,0.900) (22.222,0.677) (33.333,0.535) (44.444,0.427) (55.556,0.369) (66.667,0.239) (77.778,0.052) (88.889,-0.090) (100.000,-0.120) (5.556,0.857) (16.667,0.539) (27.778,0.491) (38.889,0.414) (50.000,0.326) (55.556,0.326) (66.667,0.133) (77.778,0.133) (88.889,0.116) (100.000,-0.038) (11.111,0.849) (11.111,0.849) (22.222,0.694) (33.333,0.488) (44.444,0.488) (55.556,0.387) (66.667,0.210) (77.778,0.069) (88.889,-0.012) (100.000,-0.113) (7.692,0.865) (15.385,0.729) (23.077,0.580) (38.462,0.394) (46.154,0.394) (53.846,0.354) (69.231,0.144) (76.923,0.019) (84.615,0.019) (100.000,-0.045) (9.091,0.923) (18.182,0.725) (27.273,0.660) (36.364,0.522) (45.455,0.435) (54.545,0.435) (63.636,0.285) (72.727,0.206) (81.818,0.022) (100.000,-0.190) (14.286,0.875) (14.286,0.875) (28.571,0.750) (28.571,0.750) (42.857,0.552) (57.143,0.354) (57.143,0.354) (71.429,0.177) (85.714,-0.021) (100.000,-0.198) (12.500,0.750) (12.500,0.750) (25.000,0.625) (37.500,0.472) (50.000,0.399) (50.000,0.399) (62.500,0.274) (75.000,0.097) (87.500,0.024) (100.000,-0.101) (10.000,0.855) (20.000,0.708) (30.000,0.529) (40.000,0.393) (50.000,0.393) (60.000,0.183) (70.000,0.143) (80.000,0.029) (90.000,-0.034) (100.000,-0.131) (8.696,0.786) (17.391,0.604) (26.087,0.479) (39.130,0.394) (47.826,0.354) (56.522,0.354) (69.565,0.104) (78.261,0.019) (86.957,0.019) (100.000,-0.073) (20.000,0.823) (20.000,0.823) (20.000,0.823) (40.000,0.625) (40.000,0.625) (60.000,0.375) (60.000,0.375) (80.000,0.375) (80.000,0.375) (100.000,-100.000) (6.667,0.918) (20.000,0.641) (26.667,0.589) (40.000,0.418) (46.667,0.391) (60.000,0.380) (66.667,0.380) (80.000,0.239) (86.667,0.102) (100.000,-0.050) (12.500,0.880) (12.500,0.880) (25.000,0.712) (37.500,0.547) (50.000,0.349) (50.000,0.349) (62.500,0.281) (75.000,0.224) (87.500,0.014) (100.000,-0.111) (5.263,0.922) (15.789,0.656) (26.316,0.523) (36.842,0.429) (47.368,0.349) (57.895,0.349) (68.421,0.193) (78.947,0.031) (89.474,0.014) (100.000,-0.050) (11.111,0.855) (11.111,0.855) (22.222,0.708) (33.333,0.529) (44.444,0.393) (55.556,0.216) (66.667,0.143) (77.778,-0.034) (88.889,-0.034) (100.000,-0.211) (14.286,0.858) (14.286,0.858) (28.571,0.693) (28.571,0.693) (42.857,0.483) (57.143,0.443) (57.143,0.443) (71.429,0.266) (85.714,0.068) (100.000,-0.142) (7.143,0.855) (14.286,0.707) (28.571,0.526) (35.714,0.417) (50.000,0.344) (57.143,0.182) (64.286,0.182) (78.571,0.070) (85.714,-0.055) (100.000,-0.116) (9.091,0.863) (18.182,0.724) (27.273,0.569) (36.364,0.488) (45.455,0.387) (54.545,0.387) (63.636,0.262) (72.727,0.148) (81.818,-0.012) (100.000,-0.113) (6.667,0.898) (20.000,0.634) (26.667,0.514) (40.000,0.398) (46.667,0.349) (60.000,0.193) (66.667,0.193) (80.000,0.014) (86.667,0.014) (100.000,-0.071) (11.111,0.827) (11.111,0.827) (22.222,0.635) (33.333,0.529) (44.444,0.385) (55.556,0.364) (66.667,0.227) (77.778,0.114) (88.889,0.029) (100.000,-0.115) (10.000,0.871) (20.000,0.708) (30.000,0.527) (40.000,0.478) (50.000,0.327) (60.000,0.197) (70.000,0.129) (80.000,0.129) (90.000,-0.004) (100.000,-0.167) (6.667,0.863) (20.000,0.572) (26.667,0.419) (40.000,0.371) (46.667,0.306) (60.000,0.306) (66.667,0.169) (80.000,0.077) (86.667,0.067) (100.000,-0.107) (6.250,0.864) (18.750,0.574) (25.000,0.444) (37.500,0.319) (50.000,0.298) (56.250,0.298) (68.750,0.114) (75.000,0.079) (87.500,0.037) (100.000,-0.046) (9.091,0.847) (18.182,0.689) (27.273,0.472) (36.364,0.366) (45.455,0.326) (54.545,0.326) (63.636,0.133) (72.727,0.133) (81.818,0.116) (100.000,-0.086) (9.091,0.792) (18.182,0.570) (27.273,0.509) (36.364,0.393) (45.455,0.365) (54.545,0.344) (63.636,0.182) (72.727,0.070) (81.818,0.042) (100.000,-0.135) (10.000,0.855) (20.000,0.707) (30.000,0.525) (40.000,0.496) (50.000,0.367) (60.000,0.306) (70.000,0.169) (80.000,0.157) (90.000,0.056) (100.000,-0.107) (14.286,0.828) (14.286,0.828) (28.571,0.638) (28.571,0.638) (42.857,0.453) (57.143,0.287) (57.143,0.287) (71.429,0.162) (85.714,-0.014) (100.000,-0.112) (9.091,0.885) (18.182,0.687) (27.273,0.510) (36.364,0.465) (45.455,0.385) (54.545,0.364) (63.636,0.364) (72.727,0.187) (81.818,0.010) (100.000,-0.115) (8.333,0.883) (16.667,0.725) (25.000,0.570) (33.333,0.435) (50.000,0.310) (58.333,0.285) (66.667,0.206) (75.000,0.081) (83.333,0.022) (100.000,-0.103) (9.677,0.691) (19.355,0.546) (29.032,0.421) (38.710,0.421) (48.387,0.314) (58.065,0.314) (67.742,0.151) (77.419,0.151) (87.097,0.113) (100.000,-0.067) 
            }; \addlegendentry{$\errLinf$}
            
        \end{axis}
    \end{tikzpicture} 
    \label{figure_real_data_two_sided_sessions}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		%xlabel={\% of required rules},
        		ymin=-0.2, ymax = 1,
                ytick={-0.2,0,0.2,0.4,0.6,0.8,1.0},
                %ylabel={$(\lg{\text{error}})/W$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.99,0.99)}, anchor=north east,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black,mark=*,only marks,mark size=1pt] coordinates{
            (8.696,0.852) (17.391,0.746) (26.087,0.614) (39.130,0.515) (47.826,0.438) (56.522,0.345) (69.565,0.227) (78.261,0.157) (86.957,0.100) (100.000,-0.054) (5.263,0.818) (15.789,0.606) (26.316,0.518) (36.842,0.451) (47.368,0.373) (57.895,0.258) (68.421,0.195) (78.947,0.048) (89.474,-0.009) (100.000,-0.069) (9.091,0.797) (18.182,0.639) (27.273,0.538) (39.394,0.422) (48.485,0.342) (57.576,0.322) (69.697,0.205) (78.788,0.130) (87.879,0.105) (100.000,-0.047) (5.263,0.809) (15.789,0.614) (26.316,0.539) (36.842,0.463) (47.368,0.342) (57.895,0.228) (68.421,0.192) (78.947,0.130) (89.474,0.032) (100.000,-0.052) (9.091,0.851) (18.182,0.697) (27.273,0.576) (36.364,0.480) (50.000,0.362) (59.091,0.261) (68.182,0.230) (77.273,0.142) (86.364,0.032) (100.000,-0.051) (5.556,0.898) (16.667,0.764) (27.778,0.681) (38.889,0.531) (50.000,0.448) (55.556,0.408) (66.667,0.301) (77.778,0.205) (88.889,0.083) (100.000,-0.063) (9.524,0.777) (19.048,0.661) (28.571,0.548) (38.095,0.480) (47.619,0.391) (57.143,0.299) (66.667,0.227) (76.190,0.132) (85.714,0.080) (100.000,-0.052) (9.524,0.840) (19.048,0.719) (28.571,0.654) (38.095,0.484) (47.619,0.437) (57.143,0.361) (66.667,0.277) (76.190,0.183) (85.714,0.085) (100.000,-0.056) (9.524,0.810) (19.048,0.692) (28.571,0.569) (38.095,0.512) (47.619,0.419) (57.143,0.350) (66.667,0.302) (76.190,0.252) (85.714,0.183) (100.000,-0.049) (8.571,0.796) (20.000,0.568) (28.571,0.477) (40.000,0.383) (48.571,0.344) (60.000,0.235) (68.571,0.199) (80.000,0.127) (88.571,0.071) (100.000,-0.060) (8.333,0.727) (19.444,0.632) (27.778,0.539) (38.889,0.466) (50.000,0.373) (58.333,0.283) (69.444,0.202) (77.778,0.156) (88.889,0.035) (100.000,-0.060) (8.333,0.724) (16.667,0.626) (29.167,0.475) (37.500,0.397) (50.000,0.317) (58.333,0.250) (66.667,0.199) (79.167,0.066) (87.500,0.039) (100.000,-0.042) (5.556,0.860) (16.667,0.691) (27.778,0.573) (38.889,0.470) (50.000,0.370) (55.556,0.356) (66.667,0.249) (77.778,0.145) (88.889,0.019) (100.000,-0.099) (5.263,0.930) (15.789,0.758) (26.316,0.699) (36.842,0.569) (47.368,0.456) (57.895,0.325) (68.421,0.211) (78.947,0.098) (89.474,-0.020) (100.000,-0.047) (9.091,0.765) (18.182,0.683) (27.273,0.594) (36.364,0.483) (50.000,0.378) (59.091,0.274) (68.182,0.224) (77.273,0.121) (86.364,0.013) (100.000,-0.063) (7.143,0.861) (17.857,0.675) (28.571,0.594) (39.286,0.469) (50.000,0.365) (57.143,0.308) (67.857,0.196) (78.571,0.091) (89.286,0.015) (100.000,-0.050) (6.250,0.889) (18.750,0.717) (25.000,0.604) (37.500,0.513) (50.000,0.358) (56.250,0.333) (68.750,0.241) (75.000,0.191) (87.500,0.061) (100.000,-0.078) (10.000,0.726) (20.000,0.582) (30.000,0.500) (40.000,0.416) (50.000,0.293) (60.000,0.158) (70.000,0.129) (80.000,0.051) (90.000,0.009) (100.000,-0.046) (9.524,0.776) (19.048,0.677) (28.571,0.633) (38.095,0.522) (47.619,0.423) (57.143,0.314) (66.667,0.224) (76.190,0.153) (85.714,0.103) (100.000,-0.052) (10.000,0.832) (20.000,0.654) (30.000,0.505) (40.000,0.430) (50.000,0.310) (60.000,0.245) (70.000,0.194) (80.000,0.051) (90.000,-0.020) (100.000,-0.083) (6.667,0.948) (20.000,0.795) (26.667,0.711) (40.000,0.577) (46.667,0.526) (60.000,0.377) (66.667,0.289) (80.000,0.194) (86.667,0.126) (100.000,-0.087) (6.667,0.846) (20.000,0.682) (26.667,0.613) (40.000,0.515) (46.667,0.435) (60.000,0.344) (66.667,0.243) (80.000,0.126) (86.667,0.094) (100.000,-0.128) (8.333,0.820) (16.667,0.595) (25.000,0.491) (33.333,0.461) (50.000,0.285) (58.333,0.181) (66.667,0.161) (75.000,0.060) (83.333,-0.018) (100.000,-0.067) (6.667,0.944) (20.000,0.702) (26.667,0.628) (40.000,0.450) (46.667,0.418) (60.000,0.294) (66.667,0.259) (80.000,0.120) (86.667,0.061) (100.000,-0.103) (6.250,0.824) (18.750,0.689) (25.000,0.613) (37.500,0.475) (50.000,0.378) (56.250,0.317) (68.750,0.141) (75.000,0.089) (87.500,-0.021) (100.000,-0.081) (9.524,0.809) (19.048,0.596) (28.571,0.536) (38.095,0.470) (47.619,0.363) (57.143,0.310) (66.667,0.197) (76.190,0.104) (85.714,0.013) (100.000,-0.065) (5.556,0.797) (16.667,0.610) (27.778,0.541) (38.889,0.452) (50.000,0.367) (55.556,0.291) (66.667,0.247) (77.778,0.151) (88.889,0.009) (100.000,-0.080) (9.524,0.824) (19.048,0.658) (28.571,0.551) (38.095,0.508) (47.619,0.386) (57.143,0.318) (66.667,0.195) (76.190,0.163) (85.714,0.055) (100.000,-0.109) (6.667,0.905) (20.000,0.687) (26.667,0.667) (40.000,0.493) (46.667,0.407) (60.000,0.295) (66.667,0.212) (80.000,0.124) (86.667,0.037) (100.000,-0.061) (7.407,0.702) (18.519,0.532) (29.630,0.479) (37.037,0.387) (48.148,0.322) (59.259,0.240) (66.667,0.203) (77.778,0.112) (88.889,0.037) (100.000,-0.060) (5.882,0.955) (17.647,0.799) (29.412,0.621) (35.294,0.613) (47.059,0.435) (58.824,0.285) (64.706,0.283) (76.471,0.175) (88.235,0.064) (100.000,-0.056) (6.250,0.904) (18.750,0.771) (25.000,0.690) (37.500,0.624) (50.000,0.410) (56.250,0.357) (68.750,0.237) (75.000,0.191) (87.500,0.068) (100.000,-0.080) (8.333,0.826) (16.667,0.648) (29.167,0.515) (37.500,0.455) (50.000,0.361) (58.333,0.313) (66.667,0.253) (79.167,0.185) (87.500,0.027) (100.000,-0.062) (7.692,0.828) (19.231,0.677) (26.923,0.567) (38.462,0.435) (50.000,0.304) (57.692,0.233) (69.231,0.139) (76.923,0.092) (88.462,0.018) (100.000,-0.094) (8.696,0.767) (17.391,0.606) (26.087,0.525) (39.130,0.390) (47.826,0.343) (56.522,0.231) (69.565,0.139) (78.261,0.117) (86.957,-0.002) (100.000,-0.038) (5.882,0.913) (17.647,0.725) (29.412,0.551) (35.294,0.549) (47.059,0.394) (58.824,0.290) (64.706,0.284) (76.471,0.175) (88.235,0.007) (100.000,-0.113) (6.897,0.716) (17.241,0.580) (27.586,0.442) (37.931,0.381) (48.276,0.340) (58.621,0.244) (68.966,0.167) (79.310,0.094) (89.655,-0.015) (100.000,-0.058) (7.407,0.803) (18.519,0.616) (29.630,0.462) (37.037,0.360) (48.148,0.298) (59.259,0.208) (66.667,0.208) (77.778,0.065) (88.889,0.038) (100.000,-0.052) (6.667,0.873) (20.000,0.686) (26.667,0.622) (40.000,0.526) (46.667,0.409) (60.000,0.323) (66.667,0.273) (80.000,0.125) (86.667,0.076) (100.000,-0.058) (6.667,0.879) (20.000,0.664) (26.667,0.598) (40.000,0.454) (46.667,0.344) (60.000,0.232) (66.667,0.210) (80.000,0.082) (86.667,0.037) (100.000,-0.063) (5.882,0.941) (17.647,0.685) (29.412,0.583) (35.294,0.509) (47.059,0.438) (58.824,0.275) (64.706,0.181) (76.471,0.094) (88.235,-0.017) (100.000,-0.068) (9.804,0.489) (19.608,0.399) (29.412,0.326) (39.869,0.306) (49.673,0.215) (59.477,0.148) (69.935,0.148) (79.739,0.054) (89.542,0.011) (100.000,-0.061) (5.556,0.828) (16.667,0.564) (27.778,0.454) (38.889,0.319) (50.000,0.293) (55.556,0.214) (66.667,0.190) (77.778,0.092) (88.889,0.060) (100.000,-0.033) (6.667,0.864) (20.000,0.694) (26.667,0.630) (40.000,0.446) (46.667,0.409) (60.000,0.232) (66.667,0.216) (80.000,0.096) (86.667,0.036) (100.000,-0.065) (8.333,0.782) (16.667,0.632) (29.167,0.470) (37.500,0.398) (50.000,0.362) (58.333,0.262) (66.667,0.187) (79.167,0.047) (87.500,0.013) (100.000,-0.059) (7.143,0.842) (14.286,0.773) (28.571,0.619) (35.714,0.559) (50.000,0.383) (57.143,0.324) (64.286,0.275) (78.571,0.147) (85.714,0.060) (100.000,-0.112) (5.263,0.926) (15.789,0.745) (26.316,0.628) (36.842,0.482) (47.368,0.404) (57.895,0.287) (68.421,0.232) (78.947,0.186) (89.474,0.081) (100.000,-0.055) (5.882,0.798) (17.647,0.638) (29.412,0.532) (35.294,0.489) (47.059,0.407) (58.824,0.304) (64.706,0.269) (76.471,0.138) (88.235,0.028) (100.000,-0.046) (6.250,0.905) (18.750,0.699) (25.000,0.654) (37.500,0.548) (50.000,0.430) (56.250,0.355) (68.750,0.267) (75.000,0.185) (87.500,0.108) (100.000,-0.048) (5.882,0.923) (17.647,0.757) (29.412,0.567) (35.294,0.535) (47.059,0.406) (58.824,0.285) (64.706,0.182) (76.471,0.106) (88.235,0.020) (100.000,-0.058) (6.667,0.898) (20.000,0.670) (26.667,0.585) (40.000,0.481) (46.667,0.420) (60.000,0.282) (66.667,0.243) (80.000,0.044) (86.667,0.030) (100.000,-0.049) (9.091,0.791) (18.182,0.595) (27.273,0.490) (39.394,0.422) (48.485,0.386) (57.576,0.294) (69.697,0.207) (78.788,0.149) (87.879,0.072) (100.000,-0.033) (8.333,0.901) (16.667,0.783) (25.000,0.676) (33.333,0.655) (50.000,0.494) (58.333,0.426) (66.667,0.376) (75.000,0.253) (83.333,0.196) (100.000,-0.058) (6.897,0.764) (17.241,0.561) (27.586,0.465) (37.931,0.360) (48.276,0.341) (58.621,0.245) (68.966,0.158) (79.310,0.071) (89.655,-0.048) (100.000,-0.056) (6.250,0.902) (18.750,0.772) (25.000,0.671) (37.500,0.557) (50.000,0.463) (56.250,0.338) (68.750,0.211) (75.000,0.186) (87.500,0.076) (100.000,-0.051) (7.143,0.797) (17.857,0.595) (28.571,0.483) (39.286,0.399) (50.000,0.315) (57.143,0.290) (67.857,0.233) (78.571,0.150) (89.286,0.021) (100.000,-0.051) (7.143,0.874) (14.286,0.793) (28.571,0.556) (35.714,0.533) (50.000,0.421) (57.143,0.339) (64.286,0.236) (78.571,0.077) (85.714,0.066) (100.000,-0.095) (9.091,0.901) (18.182,0.778) (27.273,0.660) (36.364,0.557) (45.455,0.451) (54.545,0.335) (63.636,0.275) (72.727,0.181) (81.818,0.146) (100.000,-0.059) (10.000,0.808) (20.000,0.696) (30.000,0.575) (40.000,0.478) (50.000,0.391) (60.000,0.360) (70.000,0.262) (80.000,0.186) (90.000,0.078) (100.000,-0.078) (9.524,0.832) (19.048,0.687) (28.571,0.631) (38.095,0.552) (47.619,0.442) (57.143,0.387) (66.667,0.260) (76.190,0.196) (85.714,0.061) (100.000,-0.120) (5.263,0.920) (15.789,0.699) (26.316,0.506) (36.842,0.436) (47.368,0.359) (57.895,0.277) (68.421,0.191) (78.947,0.085) (89.474,0.019) (100.000,-0.074) (5.882,0.906) (17.647,0.714) (29.412,0.596) (35.294,0.559) (47.059,0.446) (58.824,0.293) (64.706,0.271) (76.471,0.128) (88.235,0.047) (100.000,-0.088) (6.667,0.869) (20.000,0.750) (26.667,0.711) (40.000,0.577) (46.667,0.459) (60.000,0.320) (66.667,0.287) (80.000,0.133) (86.667,0.096) (100.000,-0.046) (8.000,0.793) (20.000,0.581) (28.000,0.504) (40.000,0.428) (48.000,0.356) (60.000,0.258) (68.000,0.211) (80.000,0.106) (88.000,0.052) (100.000,-0.058) (7.407,0.794) (18.519,0.591) (29.630,0.512) (37.037,0.431) (48.148,0.337) (59.259,0.265) (66.667,0.167) (77.778,0.093) (88.889,0.003) (100.000,-0.085) (5.263,0.835) (15.789,0.588) (26.316,0.522) (36.842,0.462) (47.368,0.384) (57.895,0.331) (68.421,0.196) (78.947,0.177) (89.474,0.006) (100.000,-0.078) (5.882,0.896) (17.647,0.629) (29.412,0.493) (35.294,0.476) (47.059,0.380) (58.824,0.264) (64.706,0.233) (76.471,0.121) (88.235,0.025) (100.000,-0.059) (5.263,0.862) (15.789,0.712) (26.316,0.617) (36.842,0.441) (47.368,0.426) (57.895,0.326) (68.421,0.176) (78.947,0.134) (89.474,0.002) (100.000,-0.076) (9.091,0.865) (18.182,0.792) (27.273,0.672) (36.364,0.583) (45.455,0.537) (54.545,0.441) (63.636,0.380) (72.727,0.152) (81.818,0.069) (100.000,-0.081) (10.000,0.739) (20.000,0.640) (30.000,0.506) (40.000,0.397) (50.000,0.295) (60.000,0.256) (70.000,0.207) (80.000,0.082) (90.000,0.026) (100.000,-0.052) (5.556,0.883) (16.667,0.754) (27.778,0.616) (38.889,0.511) (50.000,0.417) (55.556,0.328) (66.667,0.205) (77.778,0.161) (88.889,0.056) (100.000,-0.035) (9.756,0.606) (19.512,0.521) (29.268,0.428) (39.024,0.377) (48.780,0.318) (58.537,0.232) (68.293,0.148) (78.049,0.067) (87.805,0.050) (100.000,-0.029) 
            }; \addlegendentry{$\errLinf$}
        \end{axis}
    \end{tikzpicture}
    \label{figure_real_data_two_sided_packets}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		%xlabel={\% of required rules},
        		ymin=-0.2, ymax = 1,
                ytick={-0.2,0,0.2,0.4,0.6,0.8,1.0},
                %ylabel={$(\lg{\text{error}})/W$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.99,0.99)}, anchor=north east,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [black,mark=*,only marks,mark size=1pt] coordinates{
            (8.333,0.801) (19.444,0.679) (27.778,0.606) (38.889,0.525) (50.000,0.454) (58.333,0.374) (69.444,0.269) (77.778,0.136) (88.889,0.040) (100.000,-0.038) (7.692,0.888) (19.231,0.735) (26.923,0.668) (38.462,0.549) (50.000,0.454) (57.692,0.331) (69.231,0.204) (76.923,0.143) (88.462,0.042) (100.000,-0.036) (8.163,0.842) (18.367,0.700) (28.571,0.593) (38.776,0.516) (48.980,0.369) (59.184,0.305) (69.388,0.207) (79.592,0.130) (89.796,0.034) (100.000,-0.028) (9.677,0.799) (19.355,0.679) (29.032,0.607) (38.710,0.535) (48.387,0.431) (58.065,0.342) (67.742,0.250) (77.419,0.147) (87.097,0.067) (100.000,-0.038) (10.000,0.875) (20.000,0.743) (30.000,0.663) (40.000,0.559) (50.000,0.475) (60.000,0.346) (70.000,0.261) (80.000,0.172) (90.000,0.055) (100.000,-0.041) (7.692,0.878) (19.231,0.784) (26.923,0.673) (38.462,0.558) (50.000,0.470) (57.692,0.368) (69.231,0.266) (76.923,0.178) (88.462,0.071) (100.000,-0.081) (9.091,0.799) (18.182,0.689) (27.273,0.623) (39.394,0.531) (48.485,0.438) (57.576,0.364) (69.697,0.252) (78.788,0.129) (87.879,0.057) (100.000,-0.038) (8.824,0.835) (17.647,0.767) (29.412,0.628) (38.235,0.549) (50.000,0.423) (58.824,0.331) (67.647,0.253) (79.412,0.105) (88.235,0.025) (100.000,-0.044) (8.108,0.829) (18.919,0.694) (29.730,0.625) (37.838,0.551) (48.649,0.434) (59.459,0.318) (67.568,0.259) (78.378,0.158) (89.189,0.083) (100.000,-0.047) (9.091,0.781) (19.697,0.648) (28.788,0.559) (39.394,0.471) (50.000,0.365) (59.091,0.273) (69.697,0.200) (78.788,0.130) (89.394,0.060) (100.000,-0.039) (8.475,0.783) (18.644,0.694) (28.814,0.595) (38.983,0.518) (49.153,0.425) (59.322,0.333) (69.492,0.277) (79.661,0.187) (89.831,0.086) (100.000,-0.039) (8.163,0.757) (18.367,0.623) (28.571,0.528) (38.776,0.479) (48.980,0.368) (59.184,0.319) (69.388,0.233) (79.592,0.113) (89.796,0.048) (100.000,-0.044) (10.000,0.784) (20.000,0.696) (30.000,0.621) (40.000,0.539) (50.000,0.441) (60.000,0.347) (70.000,0.285) (80.000,0.156) (90.000,0.048) (100.000,-0.035) (8.696,0.871) (17.391,0.779) (26.087,0.706) (39.130,0.591) (47.826,0.498) (56.522,0.375) (69.565,0.297) (78.261,0.208) (86.957,0.091) (100.000,-0.038) (8.108,0.849) (18.919,0.722) (29.730,0.625) (37.838,0.567) (48.649,0.448) (59.459,0.316) (67.568,0.278) (78.378,0.183) (89.189,0.035) (100.000,-0.040) (9.302,0.806) (18.605,0.711) (27.907,0.608) (39.535,0.469) (48.837,0.367) (58.140,0.314) (69.767,0.223) (79.070,0.129) (88.372,0.029) (100.000,-0.040) (8.696,0.883) (17.391,0.757) (26.087,0.672) (39.130,0.548) (47.826,0.458) (56.522,0.379) (69.565,0.230) (78.261,0.158) (86.957,0.081) (100.000,-0.086) (7.895,0.801) (18.421,0.681) (28.947,0.536) (39.474,0.431) (50.000,0.358) (57.895,0.308) (68.421,0.208) (78.947,0.130) (89.474,0.044) (100.000,-0.045) (9.091,0.837) (18.182,0.741) (27.273,0.652) (39.394,0.549) (48.485,0.474) (57.576,0.387) (69.697,0.258) (78.788,0.166) (87.879,0.064) (100.000,-0.042) (9.091,0.825) (18.182,0.706) (27.273,0.630) (39.394,0.515) (48.485,0.425) (57.576,0.356) (69.697,0.256) (78.788,0.155) (87.879,0.083) (100.000,-0.044) (8.000,0.909) (20.000,0.793) (28.000,0.719) (40.000,0.580) (48.000,0.525) (60.000,0.404) (68.000,0.298) (80.000,0.161) (88.000,0.064) (100.000,-0.045) (8.696,0.886) (17.391,0.777) (26.087,0.717) (39.130,0.584) (47.826,0.501) (56.522,0.385) (69.565,0.255) (78.261,0.160) (86.957,0.045) (100.000,-0.041) (10.000,0.827) (20.000,0.696) (30.000,0.596) (40.000,0.497) (50.000,0.356) (60.000,0.288) (70.000,0.144) (80.000,0.111) (90.000,0.000) (100.000,-0.030) (8.333,0.908) (16.667,0.776) (29.167,0.628) (37.500,0.521) (50.000,0.390) (58.333,0.347) (66.667,0.282) (79.167,0.170) (87.500,0.056) (100.000,-0.035) (7.143,0.854) (17.857,0.714) (28.571,0.643) (39.286,0.528) (50.000,0.419) (57.143,0.351) (67.857,0.254) (78.571,0.114) (89.286,0.043) (100.000,-0.050) (8.824,0.812) (17.647,0.722) (29.412,0.625) (38.235,0.546) (50.000,0.424) (58.824,0.339) (67.647,0.267) (79.412,0.136) (88.235,0.087) (100.000,-0.039) (7.692,0.853) (19.231,0.709) (26.923,0.648) (38.462,0.500) (50.000,0.425) (57.692,0.326) (69.231,0.231) (76.923,0.161) (88.462,0.071) (100.000,-0.065) (9.677,0.832) (19.355,0.711) (29.032,0.604) (38.710,0.528) (48.387,0.429) (58.065,0.360) (67.742,0.269) (77.419,0.191) (87.097,0.120) (100.000,-0.041) (9.524,0.858) (19.048,0.776) (28.571,0.660) (38.095,0.565) (47.619,0.497) (57.143,0.388) (66.667,0.319) (76.190,0.231) (85.714,0.141) (100.000,-0.053) (7.692,0.751) (17.949,0.662) (28.205,0.550) (38.462,0.473) (48.718,0.378) (58.974,0.293) (69.231,0.211) (79.487,0.138) (89.744,0.073) (100.000,-0.039) (10.000,0.851) (20.000,0.724) (30.000,0.549) (40.000,0.438) (50.000,0.395) (60.000,0.271) (70.000,0.201) (80.000,0.116) (90.000,0.050) (100.000,-0.044) (7.407,0.847) (18.519,0.734) (29.630,0.628) (37.037,0.529) (48.148,0.399) (59.259,0.333) (66.667,0.285) (77.778,0.156) (88.889,0.019) (100.000,-0.047) (9.302,0.757) (18.605,0.651) (27.907,0.575) (39.535,0.478) (48.837,0.402) (58.140,0.333) (69.767,0.222) (79.070,0.167) (88.372,0.059) (100.000,-0.047) (9.375,0.888) (18.750,0.767) (28.125,0.631) (37.500,0.552) (50.000,0.443) (59.375,0.346) (68.750,0.232) (78.125,0.166) (87.500,0.060) (100.000,-0.032) (8.571,0.845) (20.000,0.696) (28.571,0.606) (40.000,0.532) (48.571,0.453) (60.000,0.348) (68.571,0.295) (80.000,0.183) (88.571,0.060) (100.000,-0.034) (7.407,0.893) (18.519,0.737) (29.630,0.653) (37.037,0.587) (48.148,0.488) (59.259,0.354) (66.667,0.281) (77.778,0.191) (88.889,0.073) (100.000,-0.028) (8.333,0.752) (18.750,0.624) (29.167,0.541) (39.583,0.475) (50.000,0.374) (58.333,0.298) (68.750,0.225) (79.167,0.139) (89.583,0.047) (100.000,-0.030) (9.091,0.802) (18.182,0.625) (29.545,0.513) (38.636,0.446) (50.000,0.356) (59.091,0.287) (68.182,0.202) (79.545,0.119) (88.636,0.021) (100.000,-0.041) (9.091,0.872) (18.182,0.736) (27.273,0.668) (36.364,0.582) (50.000,0.457) (59.091,0.367) (68.182,0.250) (77.273,0.176) (86.364,0.060) (100.000,-0.032) (9.091,0.889) (18.182,0.752) (27.273,0.642) (36.364,0.536) (50.000,0.418) (59.091,0.337) (68.182,0.247) (77.273,0.187) (86.364,0.113) (100.000,-0.041) (6.897,0.922) (17.241,0.748) (27.586,0.682) (37.931,0.561) (48.276,0.481) (58.621,0.396) (68.966,0.269) (79.310,0.190) (89.655,0.077) (100.000,-0.045) (9.633,0.632) (19.725,0.554) (29.817,0.524) (39.908,0.407) (50.000,0.320) (59.633,0.262) (69.725,0.193) (79.817,0.125) (89.908,0.005) (100.000,-0.029) (9.677,0.725) (19.355,0.545) (29.032,0.467) (38.710,0.395) (48.387,0.346) (58.065,0.305) (67.742,0.241) (77.419,0.131) (87.097,0.087) (100.000,-0.035) (8.000,0.874) (20.000,0.747) (28.000,0.656) (40.000,0.587) (48.000,0.520) (60.000,0.404) (68.000,0.346) (80.000,0.248) (88.000,0.158) (100.000,-0.048) (7.692,0.806) (17.949,0.580) (28.205,0.526) (38.462,0.424) (48.718,0.369) (58.974,0.285) (69.231,0.189) (79.487,0.145) (89.744,0.043) (100.000,-0.059) (10.000,0.877) (20.000,0.707) (30.000,0.555) (40.000,0.486) (50.000,0.427) (60.000,0.320) (70.000,0.249) (80.000,0.160) (90.000,0.028) (100.000,-0.032) (9.677,0.848) (19.355,0.710) (29.032,0.619) (38.710,0.522) (48.387,0.481) (58.065,0.356) (67.742,0.254) (77.419,0.149) (87.097,0.084) (100.000,-0.049) (7.692,0.878) (19.231,0.723) (26.923,0.641) (38.462,0.541) (50.000,0.413) (57.692,0.320) (69.231,0.237) (76.923,0.167) (88.462,0.080) (100.000,-0.062) (10.000,0.882) (20.000,0.784) (30.000,0.743) (40.000,0.621) (50.000,0.505) (60.000,0.413) (70.000,0.305) (80.000,0.208) (90.000,0.039) (100.000,-0.065) (9.091,0.880) (18.182,0.777) (27.273,0.686) (36.364,0.623) (50.000,0.493) (59.091,0.416) (68.182,0.318) (77.273,0.171) (86.364,0.102) (100.000,-0.052) (7.407,0.918) (18.519,0.720) (29.630,0.614) (37.037,0.559) (48.148,0.443) (59.259,0.341) (66.667,0.241) (77.778,0.172) (88.889,0.022) (100.000,-0.036) (8.511,0.805) (19.149,0.667) (29.787,0.584) (38.298,0.526) (48.936,0.431) (59.574,0.317) (68.085,0.244) (78.723,0.145) (89.362,0.029) (100.000,-0.039) (8.696,0.886) (17.391,0.778) (26.087,0.713) (39.130,0.559) (47.826,0.477) (56.522,0.408) (69.565,0.198) (78.261,0.139) (86.957,0.046) (100.000,-0.100) (7.692,0.840) (17.949,0.693) (28.205,0.592) (38.462,0.525) (48.718,0.424) (58.974,0.302) (69.231,0.242) (79.487,0.172) (89.744,0.058) (100.000,-0.038) (8.696,0.890) (17.391,0.783) (26.087,0.675) (39.130,0.549) (47.826,0.493) (56.522,0.421) (69.565,0.263) (78.261,0.179) (86.957,0.076) (100.000,-0.043) (9.302,0.823) (18.605,0.686) (27.907,0.596) (39.535,0.501) (48.837,0.391) (58.140,0.302) (69.767,0.203) (79.070,0.112) (88.372,0.035) (100.000,-0.042) (7.692,0.907) (19.231,0.705) (26.923,0.659) (38.462,0.540) (50.000,0.387) (57.692,0.318) (69.231,0.199) (76.923,0.118) (88.462,0.060) (100.000,-0.042) (5.263,0.951) (15.789,0.828) (26.316,0.689) (36.842,0.618) (47.368,0.494) (57.895,0.360) (68.421,0.294) (78.947,0.169) (89.474,0.047) (100.000,-0.036) (9.375,0.887) (18.750,0.692) (28.125,0.613) (37.500,0.524) (50.000,0.364) (59.375,0.302) (68.750,0.227) (78.125,0.157) (87.500,0.083) (100.000,-0.044) (9.677,0.871) (19.355,0.774) (29.032,0.705) (38.710,0.605) (48.387,0.485) (58.065,0.408) (67.742,0.279) (77.419,0.161) (87.097,0.062) (100.000,-0.038) (8.824,0.771) (17.647,0.684) (29.412,0.556) (38.235,0.521) (50.000,0.392) (58.824,0.312) (67.647,0.230) (79.412,0.150) (88.235,0.077) (100.000,-0.045) (7.407,0.869) (18.519,0.724) (29.630,0.636) (37.037,0.586) (48.148,0.469) (59.259,0.395) (66.667,0.318) (77.778,0.208) (88.889,0.059) (100.000,-0.068) (8.333,0.897) (16.667,0.715) (29.167,0.594) (37.500,0.485) (50.000,0.392) (58.333,0.306) (66.667,0.241) (79.167,0.173) (87.500,0.061) (100.000,-0.042) (8.108,0.801) (18.919,0.689) (29.730,0.594) (37.838,0.532) (48.649,0.424) (59.459,0.337) (67.568,0.236) (78.378,0.121) (89.189,0.052) (100.000,-0.034) (8.108,0.839) (18.919,0.708) (29.730,0.621) (37.838,0.545) (48.649,0.432) (59.459,0.334) (67.568,0.254) (78.378,0.167) (89.189,0.082) (100.000,-0.048) (6.897,0.845) (17.241,0.712) (27.586,0.625) (37.931,0.536) (48.276,0.408) (58.621,0.328) (68.966,0.197) (79.310,0.130) (89.655,0.034) (100.000,-0.055) (7.143,0.862) (17.857,0.704) (28.571,0.605) (39.286,0.506) (50.000,0.416) (57.143,0.362) (67.857,0.265) (78.571,0.136) (89.286,0.052) (100.000,-0.031) (9.375,0.835) (18.750,0.704) (28.125,0.603) (37.500,0.526) (50.000,0.432) (59.375,0.344) (68.750,0.267) (78.125,0.180) (87.500,0.092) (100.000,-0.029) (5.556,0.951) (16.667,0.825) (27.778,0.728) (38.889,0.586) (50.000,0.442) (55.556,0.399) (66.667,0.278) (77.778,0.160) (88.889,0.039) (100.000,-0.038) (9.091,0.812) (18.182,0.731) (27.273,0.641) (39.394,0.527) (48.485,0.448) (57.576,0.377) (69.697,0.271) (78.788,0.200) (87.879,0.088) (100.000,-0.025) (10.000,0.836) (20.000,0.719) (30.000,0.649) (40.000,0.542) (50.000,0.422) (60.000,0.284) (70.000,0.252) (80.000,0.166) (90.000,0.070) (100.000,-0.044) (9.375,0.699) (18.750,0.594) (29.688,0.540) (39.062,0.444) (50.000,0.346) (59.375,0.262) (68.750,0.146) (79.688,0.076) (89.062,0.044) (100.000,-0.036) 
            }; \addlegendentry{$\errLinf$}
        \end{axis}
    \end{tikzpicture}
    \label{figure_real_data_two_sided_bytes}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    
    \subfigure {
        \hspace*{-1.0em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		%xlabel={\% of required rules},
        		ymin=-0.2, ymax = 1,
                ytick={-0.2,0,0.2,0.4,0.6,0.8,1.0},
                ylabel={$(\lg{\text{error}})/W$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.99,0.99)}, anchor=north east,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [blue,mark=*,only marks,mark size=1pt] coordinates{
            (10.000,0.790) (20.000,0.625) (30.000,0.500) (40.000,0.500) (50.000,0.375) (60.000,0.250) (70.000,0.250) (80.000,0.250) (90.000,0.250) (100.000,-100.000) (9.091,0.802) (18.182,0.613) (27.273,0.552) (36.364,0.474) (45.455,0.319) (54.545,0.302) (63.636,0.151) (72.727,0.113) (81.818,0.052) (100.000,-0.211) (6.250,0.849) (18.750,0.586) (25.000,0.508) (37.500,0.411) (50.000,0.346) (56.250,0.273) (68.750,0.186) (75.000,0.105) (87.500,-0.112) (100.000,-0.185) (7.692,0.871) (15.385,0.736) (23.077,0.596) (38.462,0.438) (46.154,0.300) (53.846,0.227) (69.231,0.102) (76.923,0.102) (84.615,0.043) (100.000,-0.121) (7.692,0.871) (15.385,0.741) (23.077,0.606) (38.462,0.461) (46.154,0.352) (53.846,0.286) (69.231,0.102) (76.923,0.102) (84.615,0.075) (100.000,-0.121) (10.000,0.861) (20.000,0.721) (30.000,0.563) (40.000,0.352) (50.000,0.341) (60.000,0.102) (70.000,0.102) (80.000,0.080) (90.000,-0.050) (100.000,-0.104) (10.000,0.813) (20.000,0.604) (30.000,0.592) (40.000,0.425) (50.000,0.378) (60.000,0.253) (70.000,0.253) (80.000,0.171) (90.000,-0.107) (100.000,-0.128) (7.692,0.859) (15.385,0.717) (23.077,0.552) (38.462,0.302) (46.154,0.302) (53.846,0.302) (69.231,0.052) (76.923,-0.021) (84.615,-0.146) (100.000,-0.146) (7.143,0.852) (14.286,0.701) (28.571,0.509) (35.714,0.484) (50.000,0.276) (57.143,0.197) (64.286,0.197) (78.571,-0.003) (85.714,-0.079) (100.000,-0.204) (9.524,0.734) (19.048,0.591) (28.571,0.469) (38.095,0.399) (47.619,0.285) (57.143,0.263) (66.667,0.263) (76.190,0.152) (85.714,0.027) (100.000,-0.223) (10.000,0.705) (20.000,0.519) (30.000,0.463) (40.000,0.338) (50.000,0.259) (60.000,0.104) (70.000,0.093) (80.000,-0.032) (90.000,-0.032) (100.000,-0.070) (10.000,0.708) (20.000,0.529) (30.000,0.428) (40.000,0.355) (50.000,0.230) (60.000,0.208) (70.000,0.183) (80.000,0.029) (90.000,-0.050) (100.000,-0.096) (7.692,0.821) (15.385,0.618) (23.077,0.486) (38.462,0.338) (46.154,0.243) (53.846,0.213) (69.231,0.104) (76.923,-0.037) (84.615,-0.045) (100.000,-0.243) (10.000,0.828) (20.000,0.638) (30.000,0.578) (40.000,0.388) (50.000,0.361) (60.000,0.203) (70.000,0.162) (80.000,-0.088) (90.000,-0.139) (100.000,-0.172) (7.143,0.827) (14.286,0.636) (28.571,0.416) (35.714,0.407) (50.000,0.169) (57.143,0.169) (64.286,0.169) (78.571,0.077) (85.714,0.018) (100.000,-0.107) (7.692,0.866) (15.385,0.733) (23.077,0.588) (38.462,0.417) (46.154,0.287) (53.846,0.263) (69.231,0.253) (76.923,0.133) (84.615,-0.014) (100.000,-0.305) (12.500,0.807) (12.500,0.807) (25.000,0.570) (37.500,0.417) (50.000,0.365) (50.000,0.365) (62.500,0.167) (75.000,0.134) (87.500,0.042) (100.000,-0.116) (6.250,0.879) (18.750,0.640) (25.000,0.488) (37.500,0.354) (50.000,0.276) (56.250,0.189) (68.750,0.151) (75.000,0.151) (87.500,-0.086) (100.000,-0.211) (7.692,0.856) (15.385,0.711) (23.077,0.535) (38.462,0.395) (46.154,0.223) (53.846,0.197) (69.231,-0.004) (76.923,-0.004) (84.615,-0.004) (100.000,-0.144) (9.091,0.817) (18.182,0.605) (27.273,0.544) (36.364,0.457) (45.455,0.294) (54.545,0.275) (63.636,0.268) (72.727,0.169) (81.818,0.018) (100.000,-0.107) (12.500,0.839) (12.500,0.839) (25.000,0.668) (37.500,0.443) (50.000,0.391) (50.000,0.391) (62.500,0.233) (75.000,0.141) (87.500,-0.057) (100.000,-0.182) (10.000,0.881) (20.000,0.730) (30.000,0.583) (40.000,0.404) (50.000,0.308) (60.000,0.268) (70.000,0.075) (80.000,0.058) (90.000,-0.159) (100.000,-0.175) (12.500,0.742) (12.500,0.742) (25.000,0.535) (37.500,0.423) (50.000,0.225) (50.000,0.225) (62.500,0.160) (75.000,0.160) (87.500,-0.150) (100.000,-0.150) (11.111,0.830) (11.111,0.830) (22.222,0.644) (33.333,0.519) (44.444,0.394) (55.556,0.229) (66.667,0.104) (77.778,-0.021) (88.889,-0.021) (100.000,-0.045) (14.286,0.851) (14.286,0.851) (28.571,0.698) (28.571,0.698) (42.857,0.500) (57.143,0.500) (57.143,0.500) (71.429,0.375) (85.714,0.375) (100.000,-100.000) (8.333,0.821) (16.667,0.620) (25.000,0.597) (33.333,0.439) (50.000,0.390) (58.333,0.222) (66.667,0.130) (75.000,-0.068) (83.333,-0.068) (100.000,-0.068) (9.091,0.852) (18.182,0.702) (27.273,0.529) (36.364,0.510) (45.455,0.404) (54.545,0.187) (63.636,0.062) (72.727,-0.011) (81.818,-0.011) (100.000,-0.136) (8.333,0.875) (16.667,0.750) (25.000,0.625) (33.333,0.445) (50.000,0.240) (58.333,0.240) (66.667,0.219) (75.000,0.042) (83.333,0.042) (100.000,-0.241) (10.000,0.855) (20.000,0.707) (30.000,0.526) (40.000,0.417) (50.000,0.292) (60.000,0.167) (70.000,0.134) (80.000,0.009) (90.000,-0.116) (100.000,-0.241) (5.882,0.883) (17.647,0.607) (29.412,0.462) (35.294,0.414) (47.059,0.314) (58.824,0.116) (64.706,0.116) (76.471,0.116) (88.235,0.116) (100.000,-0.018) (12.500,0.772) (12.500,0.772) (25.000,0.578) (37.500,0.388) (50.000,0.380) (50.000,0.380) (62.500,0.190) (75.000,0.065) (87.500,-0.025) (100.000,-0.150) (11.111,0.802) (11.111,0.802) (22.222,0.552) (33.333,0.552) (44.444,0.363) (55.556,0.302) (66.667,0.302) (77.778,0.052) (88.889,0.052) (100.000,-0.137) (5.263,0.861) (15.789,0.559) (26.316,0.522) (36.842,0.405) (47.368,0.328) (57.895,0.130) (68.421,0.065) (78.947,0.065) (89.474,0.065) (100.000,-0.150) (9.091,0.915) (18.182,0.790) (27.273,0.625) (36.364,0.573) (45.455,0.500) (54.545,0.500) (63.636,0.375) (72.727,0.375) (81.818,0.375) (100.000,-100.000) (8.333,0.853) (16.667,0.702) (25.000,0.512) (33.333,0.478) (50.000,0.254) (58.333,0.254) (66.667,0.159) (75.000,0.129) (83.333,0.020) (100.000,-0.355) (12.500,0.875) (12.500,0.875) (25.000,0.750) (37.500,0.552) (50.000,0.363) (50.000,0.363) (62.500,0.302) (75.000,0.262) (87.500,0.052) (100.000,-0.137) (10.000,0.730) (20.000,0.582) (30.000,0.425) (40.000,0.400) (50.000,0.169) (60.000,0.169) (70.000,0.169) (80.000,0.121) (90.000,-0.107) (100.000,-0.107) (8.696,0.765) (17.391,0.548) (26.087,0.492) (39.130,0.359) (47.826,0.285) (56.522,0.160) (69.565,0.160) (78.261,0.160) (86.957,-0.025) (100.000,-0.150) (12.500,0.808) (12.500,0.808) (25.000,0.575) (37.500,0.381) (50.000,0.355) (50.000,0.355) (62.500,0.143) (75.000,0.029) (87.500,-0.232) (100.000,-0.284) (14.286,0.812) (14.286,0.812) (28.571,0.590) (28.571,0.590) (42.857,0.421) (57.143,0.239) (57.143,0.239) (71.429,0.154) (85.714,-0.011) (100.000,-0.136) (10.000,0.798) (20.000,0.581) (30.000,0.535) (40.000,0.397) (50.000,0.285) (60.000,0.225) (70.000,0.100) (80.000,0.008) (90.000,-0.025) (100.000,-0.150) (9.091,0.697) (19.318,0.534) (29.545,0.346) (39.773,0.346) (50.000,0.235) (59.091,0.063) (69.318,0.063) (79.545,0.063) (89.773,0.063) (100.000,-0.210) (7.143,0.854) (14.286,0.705) (28.571,0.460) (35.714,0.401) (50.000,0.276) (57.143,0.151) (64.286,0.151) (78.571,0.039) (85.714,-0.040) (100.000,-0.211) (11.111,0.900) (11.111,0.900) (22.222,0.677) (33.333,0.535) (44.444,0.427) (55.556,0.220) (66.667,0.177) (77.778,-0.006) (88.889,-0.131) (100.000,-0.168) (5.556,0.857) (16.667,0.539) (27.778,0.491) (38.889,0.414) (50.000,0.241) (55.556,0.241) (66.667,0.116) (77.778,0.116) (88.889,0.116) (100.000,-0.038) (11.111,0.849) (11.111,0.849) (22.222,0.694) (33.333,0.488) (44.444,0.488) (55.556,0.349) (66.667,0.210) (77.778,0.069) (88.889,-0.012) (100.000,-0.137) (7.692,0.865) (15.385,0.729) (23.077,0.580) (38.462,0.394) (46.154,0.394) (53.846,0.104) (69.231,-0.021) (76.923,-0.021) (84.615,-0.021) (100.000,-0.045) (9.091,0.923) (18.182,0.706) (27.273,0.660) (36.364,0.522) (45.455,0.383) (54.545,0.350) (63.636,0.285) (72.727,0.133) (81.818,-0.025) (100.000,-0.025) (14.286,0.875) (14.286,0.875) (28.571,0.750) (28.571,0.750) (42.857,0.552) (57.143,0.302) (57.143,0.302) (71.429,0.104) (85.714,-0.021) (100.000,-0.045) (12.500,0.750) (12.500,0.750) (25.000,0.625) (37.500,0.472) (50.000,0.314) (50.000,0.314) (62.500,0.274) (75.000,0.097) (87.500,-0.028) (100.000,-0.101) (10.000,0.855) (20.000,0.708) (30.000,0.529) (40.000,0.355) (50.000,0.308) (60.000,0.183) (70.000,0.143) (80.000,0.029) (90.000,-0.050) (100.000,-0.284) (8.696,0.786) (17.391,0.604) (26.087,0.479) (39.130,0.394) (47.826,0.330) (56.522,0.177) (69.565,-0.021) (78.261,-0.021) (86.957,-0.021) (100.000,-0.045) (20.000,0.823) (20.000,0.823) (20.000,0.823) (40.000,0.625) (40.000,0.625) (60.000,0.375) (60.000,0.375) (80.000,0.375) (80.000,0.375) (100.000,-100.000) (6.667,0.918) (20.000,0.641) (26.667,0.589) (40.000,0.418) (46.667,0.391) (60.000,0.380) (66.667,0.380) (80.000,0.141) (86.667,-0.057) (100.000,-0.256) (12.500,0.880) (12.500,0.880) (25.000,0.712) (37.500,0.539) (50.000,0.264) (50.000,0.264) (62.500,0.245) (75.000,0.224) (87.500,0.014) (100.000,-0.203) (5.263,0.922) (15.789,0.656) (26.316,0.523) (36.842,0.429) (47.368,0.325) (57.895,0.186) (68.421,0.139) (78.947,0.014) (89.474,0.014) (100.000,-0.328) (11.111,0.855) (11.111,0.855) (22.222,0.708) (33.333,0.529) (44.444,0.355) (55.556,0.183) (66.667,0.143) (77.778,-0.050) (88.889,-0.067) (100.000,-0.284) (14.286,0.858) (14.286,0.858) (28.571,0.693) (28.571,0.693) (42.857,0.483) (57.143,0.391) (57.143,0.391) (71.429,0.266) (85.714,-0.057) (100.000,-0.182) (7.143,0.855) (14.286,0.707) (28.571,0.526) (35.714,0.417) (50.000,0.167) (57.143,0.167) (64.286,0.167) (78.571,0.042) (85.714,-0.116) (100.000,-0.116) (9.091,0.863) (18.182,0.724) (27.273,0.569) (36.364,0.488) (45.455,0.363) (54.545,0.349) (63.636,0.262) (72.727,0.148) (81.818,-0.012) (100.000,-0.137) (6.667,0.898) (20.000,0.634) (26.667,0.514) (40.000,0.398) (46.667,0.264) (60.000,0.099) (66.667,0.047) (80.000,0.014) (86.667,0.014) (100.000,-0.219) (11.111,0.827) (11.111,0.827) (22.222,0.635) (33.333,0.529) (44.444,0.385) (55.556,0.187) (66.667,0.114) (77.778,0.114) (88.889,-0.136) (100.000,-0.136) (10.000,0.871) (20.000,0.708) (30.000,0.527) (40.000,0.478) (50.000,0.327) (60.000,0.173) (70.000,0.129) (80.000,0.129) (90.000,-0.091) (100.000,-0.355) (6.667,0.863) (20.000,0.572) (26.667,0.419) (40.000,0.371) (46.667,0.294) (60.000,0.169) (66.667,0.169) (80.000,0.077) (86.667,0.018) (100.000,-0.107) (6.250,0.864) (18.750,0.574) (25.000,0.444) (37.500,0.319) (50.000,0.239) (56.250,0.184) (68.750,0.114) (75.000,0.079) (87.500,-0.046) (100.000,-0.046) (9.091,0.847) (18.182,0.689) (27.273,0.472) (36.364,0.366) (45.455,0.314) (54.545,0.201) (63.636,0.116) (72.727,0.116) (81.818,0.116) (100.000,-0.086) (9.091,0.792) (18.182,0.570) (27.273,0.509) (36.364,0.393) (45.455,0.365) (54.545,0.167) (63.636,0.042) (72.727,0.042) (81.818,0.042) (100.000,-0.241) (10.000,0.855) (20.000,0.707) (30.000,0.525) (40.000,0.496) (50.000,0.367) (60.000,0.169) (70.000,0.169) (80.000,0.157) (90.000,-0.107) (100.000,-0.107) (14.286,0.828) (14.286,0.828) (28.571,0.638) (28.571,0.638) (42.857,0.453) (57.143,0.263) (57.143,0.263) (71.429,0.162) (85.714,-0.139) (100.000,-0.213) (9.091,0.885) (18.182,0.687) (27.273,0.510) (36.364,0.465) (45.455,0.385) (54.545,0.364) (63.636,0.296) (72.727,-0.011) (81.818,-0.136) (100.000,-0.136) (8.333,0.883) (16.667,0.725) (25.000,0.570) (33.333,0.410) (50.000,0.310) (58.333,0.285) (66.667,0.100) (75.000,0.081) (83.333,-0.025) (100.000,-0.103) (9.677,0.691) (19.355,0.546) (29.032,0.421) (38.710,0.421) (48.387,0.276) (58.065,0.151) (67.742,0.151) (77.419,0.151) (87.097,0.113) (100.000,-0.211) 
            }; \addlegendentry{$\errLinfPos$}
            
        \end{axis}
    \end{tikzpicture} 
    \label{figure_real_data_one_sided_sessions}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		%xlabel={\% of required rules},
        		ymin=-0.2, ymax = 1,
                ytick={-0.2,0,0.2,0.4,0.6,0.8,1.0},
                %ylabel={$(\lg{\text{error}})/W$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.99,0.99)}, anchor=north east,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [blue,mark=*,only marks,mark size=1pt] coordinates{
            (8.696,0.852) (17.391,0.746) (26.087,0.614) (39.130,0.515) (47.826,0.438) (56.522,0.345) (69.565,0.189) (78.261,0.157) (86.957,0.084) (100.000,-0.054) (5.263,0.818) (15.789,0.606) (26.316,0.518) (36.842,0.365) (47.368,0.346) (57.895,0.240) (68.421,0.195) (78.947,0.022) (89.474,-0.009) (100.000,-0.096) (9.091,0.797) (18.182,0.639) (27.273,0.519) (39.394,0.422) (48.485,0.340) (57.576,0.322) (69.697,0.197) (78.788,0.120) (87.879,0.105) (100.000,-0.047) (5.263,0.809) (15.789,0.614) (26.316,0.539) (36.842,0.446) (47.368,0.342) (57.895,0.228) (68.421,0.192) (78.947,0.130) (89.474,-0.050) (100.000,-0.078) (9.091,0.851) (18.182,0.697) (27.273,0.572) (36.364,0.480) (50.000,0.362) (59.091,0.256) (68.182,0.230) (77.273,0.142) (86.364,0.008) (100.000,-0.051) (5.556,0.898) (16.667,0.764) (27.778,0.654) (38.889,0.460) (50.000,0.448) (55.556,0.297) (66.667,0.263) (77.778,0.200) (88.889,0.083) (100.000,-0.063) (9.524,0.777) (19.048,0.655) (28.571,0.541) (38.095,0.480) (47.619,0.391) (57.143,0.266) (66.667,0.227) (76.190,0.132) (85.714,0.080) (100.000,-0.077) (9.524,0.840) (19.048,0.719) (28.571,0.610) (38.095,0.478) (47.619,0.437) (57.143,0.338) (66.667,0.226) (76.190,0.183) (85.714,0.075) (100.000,-0.071) (9.524,0.810) (19.048,0.692) (28.571,0.569) (38.095,0.466) (47.619,0.419) (57.143,0.332) (66.667,0.302) (76.190,0.196) (85.714,0.183) (100.000,-0.049) (8.571,0.796) (20.000,0.568) (28.571,0.477) (40.000,0.383) (48.571,0.311) (60.000,0.222) (68.571,0.169) (80.000,0.086) (88.571,0.071) (100.000,-0.078) (8.333,0.727) (19.444,0.632) (27.778,0.539) (38.889,0.404) (50.000,0.373) (58.333,0.240) (69.444,0.202) (77.778,0.156) (88.889,0.019) (100.000,-0.081) (8.333,0.724) (16.667,0.626) (29.167,0.475) (37.500,0.397) (50.000,0.290) (58.333,0.247) (66.667,0.199) (79.167,0.066) (87.500,0.016) (100.000,-0.089) (5.556,0.860) (16.667,0.691) (27.778,0.571) (38.889,0.470) (50.000,0.362) (55.556,0.356) (66.667,0.249) (77.778,0.121) (88.889,0.019) (100.000,-0.102) (5.263,0.930) (15.789,0.758) (26.316,0.659) (36.842,0.536) (47.368,0.456) (57.895,0.304) (68.421,0.211) (78.947,0.079) (89.474,-0.048) (100.000,-0.082) (9.091,0.765) (18.182,0.683) (27.273,0.594) (36.364,0.483) (50.000,0.378) (59.091,0.274) (68.182,0.196) (77.273,0.093) (86.364,-0.016) (100.000,-0.063) (7.143,0.861) (17.857,0.675) (28.571,0.594) (39.286,0.469) (50.000,0.365) (57.143,0.290) (67.857,0.196) (78.571,0.052) (89.286,0.001) (100.000,-0.050) (6.250,0.889) (18.750,0.717) (25.000,0.604) (37.500,0.513) (50.000,0.352) (56.250,0.333) (68.750,0.214) (75.000,0.191) (87.500,0.041) (100.000,-0.096) (10.000,0.712) (20.000,0.582) (30.000,0.500) (40.000,0.416) (50.000,0.293) (60.000,0.158) (70.000,0.089) (80.000,0.051) (90.000,0.003) (100.000,-0.046) (9.524,0.774) (19.048,0.655) (28.571,0.633) (38.095,0.496) (47.619,0.415) (57.143,0.314) (66.667,0.224) (76.190,0.124) (85.714,0.103) (100.000,-0.052) (10.000,0.832) (20.000,0.654) (30.000,0.505) (40.000,0.412) (50.000,0.278) (60.000,0.210) (70.000,0.194) (80.000,0.010) (90.000,-0.020) (100.000,-0.108) (6.667,0.948) (20.000,0.750) (26.667,0.701) (40.000,0.554) (46.667,0.526) (60.000,0.377) (66.667,0.270) (80.000,0.124) (86.667,0.119) (100.000,-0.087) (6.667,0.846) (20.000,0.682) (26.667,0.613) (40.000,0.507) (46.667,0.435) (60.000,0.279) (66.667,0.243) (80.000,0.126) (86.667,0.094) (100.000,-0.128) (8.333,0.820) (16.667,0.595) (25.000,0.486) (33.333,0.461) (50.000,0.285) (58.333,0.181) (66.667,0.161) (75.000,0.060) (83.333,-0.028) (100.000,-0.067) (6.667,0.944) (20.000,0.702) (26.667,0.628) (40.000,0.424) (46.667,0.418) (60.000,0.294) (66.667,0.207) (80.000,0.120) (86.667,0.061) (100.000,-0.103) (6.250,0.824) (18.750,0.636) (25.000,0.586) (37.500,0.451) (50.000,0.351) (56.250,0.299) (68.750,0.141) (75.000,0.089) (87.500,-0.021) (100.000,-0.081) (9.524,0.809) (19.048,0.596) (28.571,0.536) (38.095,0.457) (47.619,0.354) (57.143,0.310) (66.667,0.197) (76.190,0.085) (85.714,-0.012) (100.000,-0.065) (5.556,0.797) (16.667,0.610) (27.778,0.526) (38.889,0.418) (50.000,0.367) (55.556,0.270) (66.667,0.247) (77.778,0.125) (88.889,-0.038) (100.000,-0.080) (9.524,0.824) (19.048,0.658) (28.571,0.551) (38.095,0.485) (47.619,0.386) (57.143,0.291) (66.667,0.195) (76.190,0.144) (85.714,0.014) (100.000,-0.112) (6.667,0.905) (20.000,0.687) (26.667,0.667) (40.000,0.493) (46.667,0.407) (60.000,0.295) (66.667,0.212) (80.000,0.082) (86.667,0.027) (100.000,-0.094) (7.407,0.702) (18.519,0.532) (29.630,0.422) (37.037,0.359) (48.148,0.322) (59.259,0.240) (66.667,0.159) (77.778,0.112) (88.889,0.034) (100.000,-0.065) (5.882,0.955) (17.647,0.799) (29.412,0.615) (35.294,0.613) (47.059,0.435) (58.824,0.285) (64.706,0.283) (76.471,0.175) (88.235,0.064) (100.000,-0.056) (6.250,0.904) (18.750,0.771) (25.000,0.690) (37.500,0.624) (50.000,0.380) (56.250,0.353) (68.750,0.223) (75.000,0.160) (87.500,0.066) (100.000,-0.080) (8.333,0.826) (16.667,0.648) (29.167,0.515) (37.500,0.455) (50.000,0.347) (58.333,0.301) (66.667,0.202) (79.167,0.185) (87.500,0.027) (100.000,-0.090) (7.692,0.828) (19.231,0.660) (26.923,0.524) (38.462,0.435) (50.000,0.304) (57.692,0.232) (69.231,0.092) (76.923,0.092) (88.462,-0.022) (100.000,-0.094) (8.696,0.767) (17.391,0.606) (26.087,0.519) (39.130,0.371) (47.826,0.343) (56.522,0.231) (69.565,0.139) (78.261,0.117) (86.957,-0.002) (100.000,-0.038) (5.882,0.913) (17.647,0.705) (29.412,0.551) (35.294,0.549) (47.059,0.394) (58.824,0.290) (64.706,0.244) (76.471,0.161) (88.235,0.004) (100.000,-0.144) (6.897,0.716) (17.241,0.580) (27.586,0.442) (37.931,0.351) (48.276,0.340) (58.621,0.219) (68.966,0.167) (79.310,0.094) (89.655,-0.015) (100.000,-0.058) (7.407,0.803) (18.519,0.616) (29.630,0.462) (37.037,0.334) (48.148,0.298) (59.259,0.203) (66.667,0.184) (77.778,0.054) (88.889,0.038) (100.000,-0.052) (6.667,0.873) (20.000,0.686) (26.667,0.622) (40.000,0.526) (46.667,0.409) (60.000,0.305) (66.667,0.273) (80.000,0.125) (86.667,0.038) (100.000,-0.058) (6.667,0.879) (20.000,0.638) (26.667,0.598) (40.000,0.454) (46.667,0.340) (60.000,0.219) (66.667,0.203) (80.000,0.082) (86.667,0.037) (100.000,-0.066) (5.882,0.941) (17.647,0.674) (29.412,0.583) (35.294,0.498) (47.059,0.438) (58.824,0.232) (64.706,0.181) (76.471,0.069) (88.235,-0.026) (100.000,-0.068) (9.804,0.489) (19.608,0.399) (29.412,0.311) (39.869,0.297) (49.673,0.215) (59.477,0.111) (69.935,0.095) (79.739,0.054) (89.542,-0.013) (100.000,-0.061) (5.556,0.828) (16.667,0.559) (27.778,0.454) (38.889,0.319) (50.000,0.293) (55.556,0.207) (66.667,0.190) (77.778,0.075) (88.889,0.058) (100.000,-0.109) (6.667,0.864) (20.000,0.694) (26.667,0.630) (40.000,0.446) (46.667,0.373) (60.000,0.232) (66.667,0.191) (80.000,0.079) (86.667,0.002) (100.000,-0.080) (8.333,0.782) (16.667,0.632) (29.167,0.470) (37.500,0.398) (50.000,0.362) (58.333,0.262) (66.667,0.178) (79.167,0.047) (87.500,0.013) (100.000,-0.104) (7.143,0.842) (14.286,0.726) (28.571,0.609) (35.714,0.559) (50.000,0.383) (57.143,0.294) (64.286,0.275) (78.571,0.147) (85.714,0.059) (100.000,-0.155) (5.263,0.926) (15.789,0.721) (26.316,0.617) (36.842,0.482) (47.368,0.398) (57.895,0.287) (68.421,0.226) (78.947,0.166) (89.474,0.081) (100.000,-0.103) (5.882,0.798) (17.647,0.638) (29.412,0.510) (35.294,0.460) (47.059,0.361) (58.824,0.304) (64.706,0.269) (76.471,0.138) (88.235,0.018) (100.000,-0.046) (6.250,0.905) (18.750,0.699) (25.000,0.654) (37.500,0.513) (50.000,0.391) (56.250,0.332) (68.750,0.215) (75.000,0.185) (87.500,0.093) (100.000,-0.048) (5.882,0.923) (17.647,0.735) (29.412,0.567) (35.294,0.535) (47.059,0.406) (58.824,0.285) (64.706,0.182) (76.471,0.089) (88.235,-0.027) (100.000,-0.058) (6.667,0.898) (20.000,0.670) (26.667,0.585) (40.000,0.447) (46.667,0.420) (60.000,0.258) (66.667,0.243) (80.000,0.031) (86.667,0.030) (100.000,-0.085) (9.091,0.791) (18.182,0.595) (27.273,0.490) (39.394,0.417) (48.485,0.336) (57.576,0.269) (69.697,0.158) (78.788,0.119) (87.879,0.049) (100.000,-0.033) (8.333,0.901) (16.667,0.777) (25.000,0.662) (33.333,0.655) (50.000,0.494) (58.333,0.426) (66.667,0.350) (75.000,0.253) (83.333,0.192) (100.000,-0.073) (6.897,0.759) (17.241,0.561) (27.586,0.465) (37.931,0.360) (48.276,0.341) (58.621,0.245) (68.966,0.158) (79.310,0.071) (89.655,-0.048) (100.000,-0.078) (6.250,0.902) (18.750,0.772) (25.000,0.663) (37.500,0.526) (50.000,0.419) (56.250,0.305) (68.750,0.189) (75.000,0.186) (87.500,0.041) (100.000,-0.051) (7.143,0.797) (17.857,0.595) (28.571,0.483) (39.286,0.399) (50.000,0.315) (57.143,0.290) (67.857,0.198) (78.571,0.122) (89.286,-0.002) (100.000,-0.051) (7.143,0.874) (14.286,0.793) (28.571,0.556) (35.714,0.533) (50.000,0.421) (57.143,0.339) (64.286,0.215) (78.571,0.077) (85.714,0.066) (100.000,-0.095) (9.091,0.901) (18.182,0.778) (27.273,0.659) (36.364,0.555) (45.455,0.451) (54.545,0.299) (63.636,0.275) (72.727,0.173) (81.818,0.146) (100.000,-0.059) (10.000,0.808) (20.000,0.696) (30.000,0.575) (40.000,0.478) (50.000,0.391) (60.000,0.313) (70.000,0.225) (80.000,0.186) (90.000,0.065) (100.000,-0.092) (9.524,0.832) (19.048,0.687) (28.571,0.607) (38.095,0.552) (47.619,0.408) (57.143,0.387) (66.667,0.217) (76.190,0.196) (85.714,0.060) (100.000,-0.120) (5.263,0.920) (15.789,0.699) (26.316,0.506) (36.842,0.436) (47.368,0.333) (57.895,0.263) (68.421,0.191) (78.947,0.085) (89.474,-0.024) (100.000,-0.083) (5.882,0.906) (17.647,0.707) (29.412,0.596) (35.294,0.559) (47.059,0.446) (58.824,0.264) (64.706,0.257) (76.471,0.127) (88.235,0.018) (100.000,-0.102) (6.667,0.869) (20.000,0.722) (26.667,0.711) (40.000,0.577) (46.667,0.459) (60.000,0.320) (66.667,0.287) (80.000,0.133) (86.667,0.096) (100.000,-0.094) (8.000,0.793) (20.000,0.581) (28.000,0.479) (40.000,0.428) (48.000,0.356) (60.000,0.258) (68.000,0.142) (80.000,0.106) (88.000,0.021) (100.000,-0.058) (7.407,0.794) (18.519,0.591) (29.630,0.475) (37.037,0.431) (48.148,0.321) (59.259,0.265) (66.667,0.159) (77.778,0.093) (88.889,0.003) (100.000,-0.099) (5.263,0.835) (15.789,0.588) (26.316,0.466) (36.842,0.462) (47.368,0.347) (57.895,0.331) (68.421,0.196) (78.947,0.177) (89.474,0.006) (100.000,-0.153) (5.882,0.896) (17.647,0.629) (29.412,0.472) (35.294,0.465) (47.059,0.344) (58.824,0.264) (64.706,0.233) (76.471,0.087) (88.235,0.025) (100.000,-0.103) (5.263,0.862) (15.789,0.693) (26.316,0.617) (36.842,0.441) (47.368,0.426) (57.895,0.326) (68.421,0.155) (78.947,0.134) (89.474,0.002) (100.000,-0.076) (9.091,0.865) (18.182,0.792) (27.273,0.672) (36.364,0.574) (45.455,0.537) (54.545,0.437) (63.636,0.380) (72.727,0.108) (81.818,0.069) (100.000,-0.105) (10.000,0.739) (20.000,0.627) (30.000,0.506) (40.000,0.389) (50.000,0.263) (60.000,0.256) (70.000,0.155) (80.000,0.082) (90.000,0.008) (100.000,-0.052) (5.556,0.883) (16.667,0.754) (27.778,0.595) (38.889,0.497) (50.000,0.417) (55.556,0.328) (66.667,0.187) (77.778,0.161) (88.889,0.056) (100.000,-0.101) (9.756,0.606) (19.512,0.521) (29.268,0.428) (39.024,0.377) (48.780,0.318) (58.537,0.209) (68.293,0.058) (78.049,0.058) (87.805,0.022) (100.000,-0.118) 
            }; \addlegendentry{$\errLinfPos$}
        \end{axis}
    \end{tikzpicture}
    \label{figure_real_data_one_sided_packets}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		%xlabel={\% of required rules},
        		ymin=-0.2, ymax = 1,
                ytick={-0.2,0,0.2,0.4,0.6,0.8,1.0},
                %ylabel={$(\lg{\text{error}})/W$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.99,0.99)}, anchor=north east,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [blue,mark=*,only marks,mark size=1pt] coordinates{
            (8.333,0.801) (19.444,0.679) (27.778,0.606) (38.889,0.525) (50.000,0.441) (58.333,0.353) (69.444,0.269) (77.778,0.121) (88.889,0.040) (100.000,-0.038) (7.692,0.888) (19.231,0.729) (26.923,0.654) (38.462,0.513) (50.000,0.454) (57.692,0.331) (69.231,0.184) (76.923,0.134) (88.462,0.042) (100.000,-0.073) (8.163,0.842) (18.367,0.691) (28.571,0.585) (38.776,0.516) (48.980,0.367) (59.184,0.302) (69.388,0.207) (79.592,0.110) (89.796,0.034) (100.000,-0.063) (9.677,0.799) (19.355,0.679) (29.032,0.607) (38.710,0.535) (48.387,0.431) (58.065,0.339) (67.742,0.250) (77.419,0.140) (87.097,0.050) (100.000,-0.068) (10.000,0.875) (20.000,0.726) (30.000,0.644) (40.000,0.559) (50.000,0.475) (60.000,0.346) (70.000,0.248) (80.000,0.172) (90.000,0.022) (100.000,-0.047) (7.692,0.874) (19.231,0.784) (26.923,0.673) (38.462,0.558) (50.000,0.470) (57.692,0.364) (69.231,0.244) (76.923,0.163) (88.462,0.047) (100.000,-0.100) (9.091,0.799) (18.182,0.689) (27.273,0.619) (39.394,0.514) (48.485,0.421) (57.576,0.362) (69.697,0.252) (78.788,0.121) (87.879,0.057) (100.000,-0.038) (8.824,0.835) (17.647,0.720) (29.412,0.618) (38.235,0.549) (50.000,0.423) (58.824,0.331) (67.647,0.253) (79.412,0.099) (88.235,0.013) (100.000,-0.044) (8.108,0.829) (18.919,0.694) (29.730,0.625) (37.838,0.510) (48.649,0.427) (59.459,0.318) (67.568,0.251) (78.378,0.158) (89.189,0.083) (100.000,-0.056) (9.091,0.781) (19.697,0.648) (28.788,0.559) (39.394,0.471) (50.000,0.361) (59.091,0.272) (69.697,0.200) (78.788,0.130) (89.394,0.033) (100.000,-0.039) (8.475,0.783) (18.644,0.683) (28.814,0.595) (38.983,0.506) (49.153,0.408) (59.322,0.325) (69.492,0.277) (79.661,0.151) (89.831,0.086) (100.000,-0.048) (8.163,0.744) (18.367,0.623) (28.571,0.528) (38.776,0.468) (48.980,0.354) (59.184,0.319) (69.388,0.233) (79.592,0.113) (89.796,0.048) (100.000,-0.048) (10.000,0.784) (20.000,0.690) (30.000,0.606) (40.000,0.527) (50.000,0.441) (60.000,0.347) (70.000,0.253) (80.000,0.156) (90.000,0.036) (100.000,-0.035) (8.696,0.871) (17.391,0.776) (26.087,0.706) (39.130,0.568) (47.826,0.498) (56.522,0.375) (69.565,0.289) (78.261,0.208) (86.957,0.081) (100.000,-0.051) (8.108,0.849) (18.919,0.722) (29.730,0.625) (37.838,0.567) (48.649,0.421) (59.459,0.316) (67.568,0.257) (78.378,0.179) (89.189,0.035) (100.000,-0.045) (9.302,0.799) (18.605,0.693) (27.907,0.608) (39.535,0.464) (48.837,0.350) (58.140,0.314) (69.767,0.223) (79.070,0.129) (88.372,0.029) (100.000,-0.040) (8.696,0.883) (17.391,0.757) (26.087,0.672) (39.130,0.525) (47.826,0.444) (56.522,0.379) (69.565,0.218) (78.261,0.143) (86.957,0.045) (100.000,-0.108) (7.895,0.801) (18.421,0.681) (28.947,0.524) (39.474,0.426) (50.000,0.358) (57.895,0.308) (68.421,0.208) (78.947,0.130) (89.474,0.020) (100.000,-0.045) (9.091,0.837) (18.182,0.741) (27.273,0.652) (39.394,0.549) (48.485,0.463) (57.576,0.364) (69.697,0.252) (78.788,0.155) (87.879,0.064) (100.000,-0.042) (9.091,0.823) (18.182,0.706) (27.273,0.630) (39.394,0.478) (48.485,0.405) (57.576,0.356) (69.697,0.256) (78.788,0.148) (87.879,0.061) (100.000,-0.044) (8.000,0.909) (20.000,0.793) (28.000,0.704) (40.000,0.580) (48.000,0.525) (60.000,0.404) (68.000,0.258) (80.000,0.135) (88.000,0.026) (100.000,-0.053) (8.696,0.886) (17.391,0.777) (26.087,0.717) (39.130,0.584) (47.826,0.490) (56.522,0.375) (69.565,0.231) (78.261,0.160) (86.957,0.045) (100.000,-0.070) (10.000,0.827) (20.000,0.696) (30.000,0.596) (40.000,0.497) (50.000,0.354) (60.000,0.278) (70.000,0.127) (80.000,0.111) (90.000,0.000) (100.000,-0.067) (8.333,0.908) (16.667,0.776) (29.167,0.591) (37.500,0.506) (50.000,0.361) (58.333,0.347) (66.667,0.262) (79.167,0.162) (87.500,0.056) (100.000,-0.035) (7.143,0.854) (17.857,0.714) (28.571,0.643) (39.286,0.528) (50.000,0.396) (57.143,0.351) (67.857,0.254) (78.571,0.111) (89.286,0.027) (100.000,-0.062) (8.824,0.812) (17.647,0.713) (29.412,0.609) (38.235,0.546) (50.000,0.395) (58.824,0.317) (67.647,0.267) (79.412,0.122) (88.235,0.087) (100.000,-0.047) (7.692,0.853) (19.231,0.709) (26.923,0.617) (38.462,0.484) (50.000,0.425) (57.692,0.320) (69.231,0.206) (76.923,0.150) (88.462,0.071) (100.000,-0.065) (9.677,0.817) (19.355,0.711) (29.032,0.591) (38.710,0.516) (48.387,0.429) (58.065,0.327) (67.742,0.269) (77.419,0.191) (87.097,0.120) (100.000,-0.041) (9.524,0.853) (19.048,0.776) (28.571,0.613) (38.095,0.565) (47.619,0.497) (57.143,0.366) (66.667,0.319) (76.190,0.231) (85.714,0.141) (100.000,-0.062) (7.692,0.751) (17.949,0.662) (28.205,0.550) (38.462,0.462) (48.718,0.378) (58.974,0.293) (69.231,0.211) (79.487,0.138) (89.744,0.067) (100.000,-0.050) (10.000,0.831) (20.000,0.724) (30.000,0.549) (40.000,0.438) (50.000,0.365) (60.000,0.271) (70.000,0.197) (80.000,0.116) (90.000,0.050) (100.000,-0.048) (7.407,0.837) (18.519,0.701) (29.630,0.628) (37.037,0.529) (48.148,0.397) (59.259,0.327) (66.667,0.285) (77.778,0.156) (88.889,0.014) (100.000,-0.067) (9.302,0.757) (18.605,0.651) (27.907,0.575) (39.535,0.478) (48.837,0.402) (58.140,0.333) (69.767,0.218) (79.070,0.167) (88.372,0.038) (100.000,-0.051) (9.375,0.888) (18.750,0.767) (28.125,0.604) (37.500,0.525) (50.000,0.429) (59.375,0.329) (68.750,0.214) (78.125,0.134) (87.500,0.052) (100.000,-0.059) (8.571,0.845) (20.000,0.685) (28.571,0.606) (40.000,0.532) (48.571,0.453) (60.000,0.348) (68.571,0.261) (80.000,0.156) (88.571,0.043) (100.000,-0.065) (7.407,0.893) (18.519,0.737) (29.630,0.653) (37.037,0.582) (48.148,0.488) (59.259,0.340) (66.667,0.245) (77.778,0.191) (88.889,0.065) (100.000,-0.028) (8.333,0.742) (18.750,0.624) (29.167,0.541) (39.583,0.442) (50.000,0.350) (58.333,0.297) (68.750,0.184) (79.167,0.134) (89.583,0.047) (100.000,-0.076) (9.091,0.802) (18.182,0.625) (29.545,0.513) (38.636,0.425) (50.000,0.345) (59.091,0.241) (68.182,0.202) (79.545,0.097) (88.636,0.011) (100.000,-0.051) (9.091,0.856) (18.182,0.736) (27.273,0.668) (36.364,0.567) (50.000,0.457) (59.091,0.356) (68.182,0.250) (77.273,0.176) (86.364,0.060) (100.000,-0.032) (9.091,0.889) (18.182,0.752) (27.273,0.610) (36.364,0.536) (50.000,0.418) (59.091,0.337) (68.182,0.222) (77.273,0.175) (86.364,0.067) (100.000,-0.076) (6.897,0.898) (17.241,0.748) (27.586,0.643) (37.931,0.561) (48.276,0.481) (58.621,0.395) (68.966,0.261) (79.310,0.154) (89.655,0.077) (100.000,-0.045) (9.633,0.632) (19.725,0.554) (29.817,0.503) (39.908,0.407) (50.000,0.320) (59.633,0.262) (69.725,0.169) (79.817,0.100) (89.908,0.001) (100.000,-0.057) (9.677,0.725) (19.355,0.545) (29.032,0.464) (38.710,0.395) (48.387,0.323) (58.065,0.305) (67.742,0.235) (77.419,0.112) (87.097,0.087) (100.000,-0.056) (8.000,0.865) (20.000,0.736) (28.000,0.646) (40.000,0.556) (48.000,0.520) (60.000,0.394) (68.000,0.316) (80.000,0.230) (88.000,0.158) (100.000,-0.057) (7.692,0.806) (17.949,0.580) (28.205,0.508) (38.462,0.424) (48.718,0.369) (58.974,0.275) (69.231,0.168) (79.487,0.145) (89.744,-0.010) (100.000,-0.059) (10.000,0.877) (20.000,0.707) (30.000,0.535) (40.000,0.486) (50.000,0.427) (60.000,0.315) (70.000,0.245) (80.000,0.160) (90.000,0.004) (100.000,-0.067) (9.677,0.848) (19.355,0.710) (29.032,0.613) (38.710,0.486) (48.387,0.481) (58.065,0.334) (67.742,0.254) (77.419,0.147) (87.097,0.074) (100.000,-0.049) (7.692,0.878) (19.231,0.721) (26.923,0.641) (38.462,0.541) (50.000,0.413) (57.692,0.320) (69.231,0.237) (76.923,0.167) (88.462,0.078) (100.000,-0.073) (10.000,0.855) (20.000,0.784) (30.000,0.733) (40.000,0.621) (50.000,0.487) (60.000,0.413) (70.000,0.305) (80.000,0.208) (90.000,0.039) (100.000,-0.065) (9.091,0.861) (18.182,0.777) (27.273,0.686) (36.364,0.605) (50.000,0.483) (59.091,0.404) (68.182,0.314) (77.273,0.171) (86.364,0.088) (100.000,-0.066) (7.407,0.886) (18.519,0.720) (29.630,0.614) (37.037,0.559) (48.148,0.443) (59.259,0.330) (66.667,0.241) (77.778,0.172) (88.889,0.022) (100.000,-0.058) (8.511,0.805) (19.149,0.667) (29.787,0.584) (38.298,0.475) (48.936,0.431) (59.574,0.317) (68.085,0.224) (78.723,0.142) (89.362,0.029) (100.000,-0.053) (8.696,0.886) (17.391,0.778) (26.087,0.713) (39.130,0.555) (47.826,0.459) (56.522,0.408) (69.565,0.198) (78.261,0.139) (86.957,0.046) (100.000,-0.109) (7.692,0.840) (17.949,0.693) (28.205,0.592) (38.462,0.502) (48.718,0.375) (58.974,0.292) (69.231,0.230) (79.487,0.150) (89.744,0.058) (100.000,-0.048) (8.696,0.870) (17.391,0.783) (26.087,0.673) (39.130,0.533) (47.826,0.493) (56.522,0.383) (69.565,0.249) (78.261,0.179) (86.957,0.076) (100.000,-0.043) (9.302,0.823) (18.605,0.686) (27.907,0.596) (39.535,0.498) (48.837,0.382) (58.140,0.298) (69.767,0.203) (79.070,0.112) (88.372,0.035) (100.000,-0.047) (7.692,0.907) (19.231,0.705) (26.923,0.639) (38.462,0.540) (50.000,0.387) (57.692,0.303) (69.231,0.194) (76.923,0.100) (88.462,0.014) (100.000,-0.072) (5.263,0.951) (15.789,0.819) (26.316,0.689) (36.842,0.618) (47.368,0.451) (57.895,0.360) (68.421,0.294) (78.947,0.169) (89.474,0.026) (100.000,-0.036) (9.375,0.887) (18.750,0.692) (28.125,0.613) (37.500,0.501) (50.000,0.353) (59.375,0.268) (68.750,0.227) (78.125,0.157) (87.500,0.083) (100.000,-0.071) (9.677,0.871) (19.355,0.773) (29.032,0.705) (38.710,0.583) (48.387,0.485) (58.065,0.365) (67.742,0.279) (77.419,0.157) (87.097,0.062) (100.000,-0.038) (8.824,0.771) (17.647,0.684) (29.412,0.554) (38.235,0.521) (50.000,0.392) (58.824,0.306) (67.647,0.213) (79.412,0.150) (88.235,0.056) (100.000,-0.045) (7.407,0.842) (18.519,0.724) (29.630,0.636) (37.037,0.557) (48.148,0.469) (59.259,0.363) (66.667,0.293) (77.778,0.208) (88.889,0.039) (100.000,-0.068) (8.333,0.897) (16.667,0.715) (29.167,0.582) (37.500,0.482) (50.000,0.392) (58.333,0.306) (66.667,0.213) (79.167,0.134) (87.500,0.052) (100.000,-0.060) (8.108,0.801) (18.919,0.688) (29.730,0.594) (37.838,0.495) (48.649,0.424) (59.459,0.308) (67.568,0.236) (78.378,0.121) (89.189,0.052) (100.000,-0.056) (8.108,0.839) (18.919,0.699) (29.730,0.621) (37.838,0.545) (48.649,0.432) (59.459,0.334) (67.568,0.235) (78.378,0.167) (89.189,0.078) (100.000,-0.048) (6.897,0.845) (17.241,0.712) (27.586,0.621) (37.931,0.535) (48.276,0.398) (58.621,0.313) (68.966,0.189) (79.310,0.104) (89.655,0.028) (100.000,-0.078) (7.143,0.862) (17.857,0.704) (28.571,0.605) (39.286,0.506) (50.000,0.386) (57.143,0.362) (67.857,0.248) (78.571,0.136) (89.286,0.042) (100.000,-0.031) (9.375,0.808) (18.750,0.704) (28.125,0.541) (37.500,0.517) (50.000,0.432) (59.375,0.344) (68.750,0.237) (78.125,0.180) (87.500,0.064) (100.000,-0.070) (5.556,0.951) (16.667,0.822) (27.778,0.710) (38.889,0.579) (50.000,0.442) (55.556,0.377) (66.667,0.267) (77.778,0.160) (88.889,0.039) (100.000,-0.053) (9.091,0.812) (18.182,0.731) (27.273,0.641) (39.394,0.527) (48.485,0.441) (57.576,0.352) (69.697,0.251) (78.788,0.200) (87.879,0.060) (100.000,-0.025) (10.000,0.824) (20.000,0.705) (30.000,0.649) (40.000,0.542) (50.000,0.421) (60.000,0.271) (70.000,0.252) (80.000,0.153) (90.000,0.060) (100.000,-0.052) (9.375,0.697) (18.750,0.594) (29.688,0.534) (39.062,0.444) (50.000,0.336) (59.375,0.262) (68.750,0.146) (79.688,0.076) (89.062,0.037) (100.000,-0.047) 
            }; \addlegendentry{$\errLinfPos$}
            
        \end{axis}
    \end{tikzpicture}
    \label{figure_real_data_one_sided_bytes}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    
    \addtocounter{subfigure}{-6} % adjusted the 'W=x' labels from (g)-(i) to (a)-(c).
    \subfigure[$W=8$ (left)]{
        \hspace*{-1.0em}  % reduces horizontal space!
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel={\% of required rules},
        		ymin=-1.2, ymax = 0.2,
                ytick={-1.2,-1.0,-0.8,-0.6,-0.4,-0.2,0,0.2},
                ylabel={$(\lg{\text{error}})/W$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.01,0.01)}, anchor=south west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [purple,mark=*,only marks,mark size=1pt] coordinates{
            (10.000,-0.142) (20.000,-0.234) (30.000,-0.267) (40.000,-0.307) (50.000,-0.359) (60.000,-0.432) (70.000,-0.484) (80.000,-0.557) (90.000,-0.682)
            (9.091,-0.125) (18.182,-0.210) (27.273,-0.274) (36.364,-0.375) (45.455,-0.412) (54.545,-0.460) (63.636,-0.524) (72.727,-0.625) (81.818,-0.662) (100.000,-0.710) (6.250,-0.049) (18.750,-0.204) (25.000,-0.238) (37.500,-0.280) (50.000,-0.412) (56.250,-0.469) (68.750,-0.552) (75.000,-0.552) (87.500,-0.552) (100.000,-0.552) (7.692,-0.009) (15.385,-0.138) (23.077,-0.193) (38.462,-0.325) (46.154,-0.331) (53.846,-0.418) (69.231,-0.486) (76.923,-0.546) (84.615,-0.594) (100.000,-0.766) (7.692,-0.009) (15.385,-0.138) (23.077,-0.229) (38.462,-0.273) (46.154,-0.381) (53.846,-0.381) (69.231,-0.486) (76.923,-0.594) (84.615,-0.689) (100.000,-0.766) (10.000,-0.026) (20.000,-0.166) (30.000,-0.229) (40.000,-0.325) (50.000,-0.404) (60.000,-0.546) (70.000,-0.665) (80.000,-0.713) (90.000,-0.850) (100.000,-0.850) (10.000,-0.109) (20.000,-0.187) (30.000,-0.330) (40.000,-0.394) (50.000,-0.438) (60.000,-0.496) (70.000,-0.581) (80.000,-0.750) (90.000,-0.750) (100.000,-0.750) (7.692,-0.030) (15.385,-0.172) (23.077,-0.226) (38.462,-0.375) (46.154,-0.422) (53.846,-0.452) (69.231,-0.561) (76.923,-0.588) (84.615,-0.672) (100.000,-0.737) (7.143,-0.043) (14.286,-0.134) (28.571,-0.266) (35.714,-0.266) (50.000,-0.386) (57.143,-0.404) (64.286,-0.503) (78.571,-0.654) (85.714,-0.769) (100.000,-0.769) (9.524,-0.070) (19.048,-0.149) (28.571,-0.221) (38.095,-0.244) (47.619,-0.322) (57.143,-0.401) (66.667,-0.460) (76.190,-0.460) (85.714,-0.460) (100.000,-0.460) (10.000,-0.100) (20.000,-0.189) (30.000,-0.259) (40.000,-0.308) (50.000,-0.356) (60.000,-0.397) (70.000,-0.483) (80.000,-0.524) (90.000,-0.578) (100.000,-0.790) (10.000,-0.144) (20.000,-0.237) (30.000,-0.283) (40.000,-0.311) (50.000,-0.364) (60.000,-0.439) (70.000,-0.548) (80.000,-0.611) (90.000,-0.710) (100.000,-0.710) (7.692,-0.096) (15.385,-0.267) (23.077,-0.298) (38.462,-0.430) (46.154,-0.470) (53.846,-0.487) (69.231,-0.633) (76.923,-0.730) (84.615,-0.730) (100.000,-0.730) (10.000,-0.085) (20.000,-0.156) (30.000,-0.274) (40.000,-0.274) (50.000,-0.387) (60.000,-0.489) (70.000,-0.750) (80.000,-0.750) (90.000,-0.750) (100.000,-0.750) (7.143,-0.086) (14.286,-0.277) (28.571,-0.325) (35.714,-0.391) (50.000,-0.412) (57.143,-0.436) (64.286,-0.497) (78.571,-0.621) (85.714,-0.644) (100.000,-0.784) (7.692,-0.017) (15.385,-0.151) (23.077,-0.209) (38.462,-0.295) (46.154,-0.361) (53.846,-0.448) (69.231,-0.557) (76.923,-0.750) (84.615,-0.750) (100.000,-0.750) (12.500,-0.118) (12.500,-0.118) (25.000,-0.302) (37.500,-0.355) (50.000,-0.429) (50.000,-0.429) (62.500,-0.559) (75.000,-0.585) (87.500,-0.695) (100.000,-0.754) (6.250,0.008) (18.750,-0.162) (25.000,-0.231) (37.500,-0.341) (50.000,-0.384) (56.250,-0.441) (68.750,-0.524) (75.000,-0.524) (87.500,-0.586) (100.000,-0.682) (7.692,-0.035) (15.385,-0.181) (23.077,-0.248) (38.462,-0.409) (46.154,-0.452) (53.846,-0.500) (69.231,-0.530) (76.923,-0.668) (84.615,-0.807) (100.000,-1.035) (9.091,-0.102) (18.182,-0.179) (27.273,-0.314) (36.364,-0.374) (45.455,-0.412) (54.545,-0.412) (63.636,-0.462) (72.727,-0.531) (81.818,-0.644) (100.000,-0.747) (12.500,-0.066) (12.500,-0.066) (25.000,-0.237) (37.500,-0.271) (50.000,-0.481) (50.000,-0.481) (62.500,-0.514) (75.000,-0.625) (87.500,-0.625) (100.000,-0.668) (10.000,0.012) (20.000,-0.107) (30.000,-0.220) (40.000,-0.283) (50.000,-0.364) (60.000,-0.601) (70.000,-0.710) (80.000,-0.710) (90.000,-0.710) (100.000,-0.710) (12.500,-0.209) (12.500,-0.209) (25.000,-0.342) (37.500,-0.460) (50.000,-0.485) (50.000,-0.485) (62.500,-0.550) (75.000,-0.653) (87.500,-0.691) (100.000,-0.691) (11.111,-0.082) (11.111,-0.082) (22.222,-0.267) (33.333,-0.375) (44.444,-0.375) (55.556,-0.470) (66.667,-0.546) (77.778,-0.682) (88.889,-0.790) (100.000,-1.017) (14.286,-0.045) (14.286,-0.045) (28.571,-0.198) (28.571,-0.198) (42.857,-0.290) (57.143,-0.396) (57.143,-0.396) (71.429,-0.415) (85.714,-0.521)
            (8.333,-0.095) (16.667,-0.169) (25.000,-0.222) (33.333,-0.296) (50.000,-0.427) (58.333,-0.427) (66.667,-0.427) (75.000,-0.427) (83.333,-0.427) (100.000,-0.563) (9.091,-0.043) (18.182,-0.158) (27.273,-0.193) (36.364,-0.265) (45.455,-0.385) (54.545,-0.500) (63.636,-0.500) (72.727,-0.500) (81.818,-0.500) (100.000,-0.775) (8.333,0.000) (16.667,-0.125) (25.000,-0.177) (33.333,-0.250) (50.000,-0.302) (58.333,-0.375) (66.667,-0.427) (75.000,-0.500) (83.333,-0.521) (100.000,-0.684) (10.000,-0.038) (20.000,-0.186) (30.000,-0.302) (40.000,-0.302) (50.000,-0.367) (60.000,-0.585) (70.000,-0.585) (80.000,-0.726) (90.000,-0.817) (100.000,-0.817) (5.882,0.017) (17.647,-0.151) (29.412,-0.230) (35.294,-0.252) (47.059,-0.308) (58.824,-0.363) (64.706,-0.389) (76.471,-0.470) (88.235,-0.733) (100.000,-0.850) (12.500,-0.168) (12.500,-0.168) (25.000,-0.274) (37.500,-0.314) (50.000,-0.366) (50.000,-0.366) (62.500,-0.561) (75.000,-0.681) (87.500,-0.750) (100.000,-0.798) (11.111,-0.125) (11.111,-0.125) (22.222,-0.210) (33.333,-0.375) (44.444,-0.375) (55.556,-0.460) (66.667,-0.625) (77.778,-0.710) (88.889,-0.875) (100.000,-0.875) (5.263,-0.028) (15.789,-0.168) (26.316,-0.274) (36.842,-0.274) (47.368,-0.274) (57.895,-0.330) (68.421,-0.366) (78.947,-0.470) (89.474,-0.561) (100.000,-0.632) (9.091,0.092) (18.182,0.000) (27.273,-0.092) (36.364,-0.198) (45.455,-0.198) (54.545,-0.250) (63.636,-0.290) (72.727,-0.323) (81.818,-0.323)
            (8.333,-0.042) (16.667,-0.193) (25.000,-0.264) (33.333,-0.295) (50.000,-0.383) (58.333,-0.431) (66.667,-0.496) (75.000,-0.559) (83.333,-0.875) (100.000,-0.875) (12.500,0.000) (12.500,0.000) (25.000,-0.125) (37.500,-0.250) (50.000,-0.375) (50.000,-0.375) (62.500,-0.375) (75.000,-0.476) (87.500,-0.625) (100.000,-0.875) (10.000,-0.039) (20.000,-0.186) (30.000,-0.240) (40.000,-0.270) (50.000,-0.352) (60.000,-0.412) (70.000,-0.471) (80.000,-0.510) (90.000,-0.538) (100.000,-0.579) (8.696,-0.102) (17.391,-0.149) (26.087,-0.191) (39.130,-0.244) (47.826,-0.292) (56.522,-0.322) (69.565,-0.460) (78.261,-0.460) (86.957,-0.460) (100.000,-0.521) (12.500,-0.116) (12.500,-0.116) (25.000,-0.349) (37.500,-0.421) (50.000,-0.543) (50.000,-0.543) (62.500,-0.601) (75.000,-0.775) (87.500,-0.775) (100.000,-0.775) (14.286,-0.109) (14.286,-0.109) (28.571,-0.332) (28.571,-0.332) (42.857,-0.500) (57.143,-0.500) (57.143,-0.500) (71.429,-0.500) (85.714,-0.588) (100.000,-0.767) (10.000,-0.131) (20.000,-0.218) (30.000,-0.285) (40.000,-0.393) (50.000,-0.460) (60.000,-0.489) (70.000,-0.566) (80.000,-0.653) (90.000,-0.704) (100.000,-0.858) (9.091,0.119) (19.318,0.057) (29.545,-0.008) (39.773,-0.137) (50.000,-0.137) (59.091,-0.137) (69.318,-0.137) (79.545,-0.176) (89.773,-0.328) (100.000,-0.410) (7.143,-0.040) (14.286,-0.189) (28.571,-0.259) (35.714,-0.318) (50.000,-0.421) (57.143,-0.427) (64.286,-0.483) (78.571,-0.524) (85.714,-0.578) (100.000,-0.710) (11.111,0.055) (11.111,0.055) (22.222,-0.125) (33.333,-0.311) (44.444,-0.375) (55.556,-0.625) (66.667,-0.625) (77.778,-0.625) (88.889,-0.625) (100.000,-0.625) (5.556,-0.034) (16.667,-0.210) (27.778,-0.246) (38.889,-0.267) (50.000,-0.320) (55.556,-0.344) (66.667,-0.394) (77.778,-0.489) (88.889,-0.650) (100.000,-0.930) (11.111,-0.048) (11.111,-0.048) (22.222,-0.204) (33.333,-0.279) (44.444,-0.410) (55.556,-0.548) (66.667,-0.573) (77.778,-0.750) (88.889,-0.910) (100.000,-0.910) (7.692,-0.020) (15.385,-0.156) (23.077,-0.216) (38.462,-0.375) (46.154,-0.375) (53.846,-0.375) (69.231,-0.491) (76.923,-0.599) (84.615,-0.790) (100.000,-0.906) (9.091,0.113) (18.182,-0.080) (27.273,-0.149) (36.364,-0.263) (45.455,-0.342) (54.545,-0.369) (63.636,-0.460) (72.727,-0.521) (81.818,-0.614) (100.000,-0.915) (14.286,0.000) (14.286,0.000) (28.571,-0.125) (28.571,-0.125) (42.857,-0.250) (57.143,-0.375) (57.143,-0.375) (71.429,-0.375) (85.714,-0.625) (100.000,-0.875) (12.500,-0.198) (12.500,-0.198) (25.000,-0.323) (37.500,-0.323) (50.000,-0.448) (50.000,-0.448) (62.500,-0.573) (75.000,-0.698) (87.500,-0.698) (100.000,-0.823) (10.000,-0.037) (20.000,-0.185) (30.000,-0.283) (40.000,-0.364) (50.000,-0.464) (60.000,-0.601) (70.000,-0.710) (80.000,-0.710) (90.000,-0.710) (100.000,-0.710) (8.696,-0.040) (17.391,-0.125) (26.087,-0.189) (39.130,-0.295) (47.826,-0.375) (56.522,-0.375) (69.565,-0.375) (78.261,-0.375) (86.957,-0.435) (100.000,-0.790) (20.000,-0.092) (20.000,-0.092) (20.000,-0.092) (40.000,-0.290) (40.000,-0.290) (60.000,-0.351) (60.000,-0.351) (80.000,-0.415) (80.000,-0.415) 
            (6.667,0.101) (20.000,-0.177) (26.667,-0.177) (40.000,-0.224) (46.667,-0.243) (60.000,-0.347) (66.667,-0.387) (80.000,-0.625) (86.667,-0.625) (100.000,-0.625) (12.500,0.010) (12.500,0.010) (25.000,-0.111) (37.500,-0.242) (50.000,-0.335) (50.000,-0.335) (62.500,-0.536) (75.000,-0.646) (87.500,-0.802) (100.000,-0.802) (5.263,0.111) (15.789,-0.111) (26.316,-0.171) (36.842,-0.335) (47.368,-0.335) (57.895,-0.335) (68.421,-0.335) (78.947,-0.418) (89.474,-0.578) (100.000,-0.802) (11.111,-0.037) (11.111,-0.037) (22.222,-0.185) (33.333,-0.364) (44.444,-0.464) (55.556,-0.601) (66.667,-0.710) (77.778,-0.791) (88.889,-0.791) (100.000,-0.791) (14.286,-0.033) (14.286,-0.033) (28.571,-0.177) (28.571,-0.177) (42.857,-0.311) (57.143,-0.347) (57.143,-0.347) (71.429,-0.625) (85.714,-0.625) (100.000,-0.736) (7.143,-0.038) (14.286,-0.186) (28.571,-0.302) (35.714,-0.302) (50.000,-0.367) (57.143,-0.410) (64.286,-0.469) (78.571,-0.585) (85.714,-0.701) (100.000,-0.701) (9.091,-0.024) (18.182,-0.162) (27.273,-0.224) (36.364,-0.318) (45.455,-0.393) (54.545,-0.476) (63.636,-0.524) (72.727,-0.662) (81.818,-0.695) (100.000,-0.818) (6.667,0.049) (20.000,-0.146) (26.667,-0.227) (40.000,-0.335) (46.667,-0.335) (60.000,-0.382) (66.667,-0.447) (80.000,-0.646) (86.667,-0.802) (100.000,-0.802) (11.111,-0.086) (11.111,-0.086) (22.222,-0.158) (33.333,-0.278) (44.444,-0.393) (55.556,-0.500) (66.667,-0.500) (77.778,-0.500) (88.889,-0.500) (100.000,-0.799) (10.000,-0.008) (20.000,-0.138) (30.000,-0.257) (40.000,-0.272) (50.000,-0.416) (60.000,-0.482) (70.000,-0.588) (80.000,-0.612) (90.000,-0.875) (100.000,-0.875) (6.667,-0.023) (20.000,-0.222) (26.667,-0.314) (40.000,-0.347) (46.667,-0.388) (60.000,-0.412) (66.667,-0.441) (80.000,-0.568) (86.667,-0.602) (100.000,-0.699) (6.250,-0.022) (18.750,-0.269) (25.000,-0.269) (37.500,-0.344) (50.000,-0.435) (56.250,-0.475) (68.750,-0.507) (75.000,-0.612) (87.500,-0.629) (100.000,-0.747) (9.091,-0.052) (18.182,-0.210) (27.273,-0.287) (36.364,-0.344) (45.455,-0.427) (54.545,-0.489) (63.636,-0.540) (72.727,-0.585) (81.818,-0.733) (100.000,-0.960) (9.091,-0.139) (18.182,-0.230) (27.273,-0.302) (36.364,-0.302) (45.455,-0.422) (54.545,-0.437) (63.636,-0.471) (72.727,-0.539) (81.818,-0.647) (100.000,-0.743) (10.000,-0.039) (20.000,-0.186) (30.000,-0.255) (40.000,-0.368) (50.000,-0.412) (60.000,-0.471) (70.000,-0.559) (80.000,-0.627) (90.000,-0.737) (100.000,-0.835) (14.286,-0.085) (14.286,-0.085) (28.571,-0.274) (28.571,-0.274) (42.857,-0.387) (57.143,-0.489) (57.143,-0.489) (71.429,-0.750) (85.714,-0.750) (100.000,-0.844) (9.091,0.021) (18.182,-0.109) (27.273,-0.201) (36.364,-0.295) (45.455,-0.332) (54.545,-0.500) (63.636,-0.500) (72.727,-0.500) (81.818,-0.500) (100.000,-0.500) (8.333,0.016) (16.667,-0.102) (25.000,-0.202) (33.333,-0.213) (50.000,-0.405) (58.333,-0.460) (66.667,-0.539) (75.000,-0.557) (83.333,-0.638) (100.000,-0.849) (9.677,-0.068) (19.355,-0.134) (29.032,-0.162) (38.710,-0.162) (48.387,-0.197) (58.065,-0.239) (67.742,-0.318) (77.419,-0.435) (87.097,-0.524) (100.000,-0.524)  
            }; \addlegendentry{$\errLinfPosRel$}
            
        \end{axis}
    \end{tikzpicture} 
    \label{figure_real_data_relative_sessions}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$W=16$ (middle)] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel={\% of required rules},
        		ymin=-1.2, ymax = 0.2,
                ytick={-1.2,-1.0,-0.8,-0.6,-0.4,-0.2,0,0.2},
                %ylabel={$\lg{\text{error}}$},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.01,0.01)}, anchor=south west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [purple,mark=*,only marks,mark size=1pt] coordinates{
            (8.696,-0.095) (17.391,-0.189) (26.087,-0.277) (39.130,-0.353) (47.826,-0.410) (56.522,-0.448) (69.565,-0.571) (78.261,-0.632) (86.957,-0.705) (100.000,-0.811) (5.263,-0.169) (15.789,-0.278) (26.316,-0.358) (36.842,-0.440) (47.368,-0.522) (57.895,-0.592) (68.421,-0.680) (78.947,-0.777) (89.474,-0.821) (100.000,-0.912) (9.091,-0.144) (18.182,-0.225) (27.273,-0.305) (39.394,-0.433) (48.485,-0.477) (57.576,-0.548) (69.697,-0.601) (78.788,-0.643) (87.879,-0.758) (100.000,-0.844) (5.263,-0.179) (15.789,-0.273) (26.316,-0.345) (36.842,-0.430) (47.368,-0.526) (57.895,-0.569) (68.421,-0.675) (78.947,-0.716) (89.474,-0.796) (100.000,-0.822) (9.091,-0.075) (18.182,-0.232) (27.273,-0.312) (36.364,-0.370) (50.000,-0.482) (59.091,-0.578) (68.182,-0.657) (77.273,-0.694) (86.364,-0.802) (100.000,-0.917) (5.556,-0.067) (16.667,-0.145) (27.778,-0.252) (38.889,-0.363) (50.000,-0.389) (55.556,-0.505) (66.667,-0.550) (77.778,-0.643) (88.889,-0.699) (100.000,-0.879) (9.524,-0.133) (19.048,-0.263) (28.571,-0.297) (38.095,-0.409) (47.619,-0.442) (57.143,-0.561) (66.667,-0.582) (76.190,-0.695) (85.714,-0.744) (100.000,-0.840) (9.524,-0.105) (19.048,-0.173) (28.571,-0.231) (38.095,-0.340) (47.619,-0.420) (57.143,-0.461) (66.667,-0.532) (76.190,-0.640) (85.714,-0.765) (100.000,-0.829) (9.524,-0.136) (19.048,-0.278) (28.571,-0.318) (38.095,-0.340) (47.619,-0.391) (57.143,-0.479) (66.667,-0.585) (76.190,-0.638) (85.714,-0.784) (100.000,-0.881) (8.571,-0.125) (20.000,-0.238) (28.571,-0.330) (40.000,-0.404) (48.571,-0.442) (60.000,-0.510) (68.571,-0.540) (80.000,-0.600) (88.571,-0.619) (100.000,-0.767) (8.333,-0.129) (19.444,-0.225) (27.778,-0.279) (38.889,-0.343) (50.000,-0.420) (58.333,-0.467) (69.444,-0.498) (77.778,-0.636) (88.889,-0.676) (100.000,-0.795) (8.333,-0.260) (16.667,-0.317) (29.167,-0.398) (37.500,-0.426) (50.000,-0.468) (58.333,-0.550) (66.667,-0.575) (79.167,-0.670) (87.500,-0.726) (100.000,-0.787) (5.556,-0.119) (16.667,-0.239) (27.778,-0.314) (38.889,-0.349) (50.000,-0.431) (55.556,-0.462) (66.667,-0.550) (77.778,-0.709) (88.889,-0.858) (100.000,-0.885) (5.263,-0.014) (15.789,-0.135) (26.316,-0.207) (36.842,-0.291) (47.368,-0.389) (57.895,-0.459) (68.421,-0.649) (78.947,-0.777) (89.474,-0.914) (100.000,-0.914) (9.091,-0.169) (18.182,-0.250) (27.273,-0.323) (36.364,-0.371) (50.000,-0.481) (59.091,-0.514) (68.182,-0.607) (77.273,-0.735) (86.364,-0.823) (100.000,-0.871) (7.143,-0.072) (17.857,-0.212) (28.571,-0.290) (39.286,-0.391) (50.000,-0.470) (57.143,-0.508) (67.857,-0.606) (78.571,-0.685) (89.286,-0.796) (100.000,-0.842) (6.250,-0.079) (18.750,-0.251) (25.000,-0.291) (37.500,-0.365) (50.000,-0.506) (56.250,-0.588) (68.750,-0.681) (75.000,-0.778) (87.500,-0.838) (100.000,-0.947) (10.000,-0.222) (20.000,-0.366) (30.000,-0.426) (40.000,-0.470) (50.000,-0.558) (60.000,-0.599) (70.000,-0.667) (80.000,-0.710) (90.000,-0.817) (100.000,-0.883) (9.524,-0.106) (19.048,-0.207) (28.571,-0.266) (38.095,-0.366) (47.619,-0.468) (57.143,-0.518) (66.667,-0.606) (76.190,-0.691) (85.714,-0.729) (100.000,-0.888) (10.000,-0.122) (20.000,-0.271) (30.000,-0.339) (40.000,-0.431) (50.000,-0.494) (60.000,-0.565) (70.000,-0.624) (80.000,-0.743) (90.000,-0.813) (100.000,-0.932) (6.667,0.023) (20.000,-0.159) (26.667,-0.176) (40.000,-0.258) (46.667,-0.335) (60.000,-0.488) (66.667,-0.577) (80.000,-0.677) (86.667,-0.742) (100.000,-0.947) (6.667,-0.136) (20.000,-0.242) (26.667,-0.272) (40.000,-0.407) (46.667,-0.459) (60.000,-0.502) (66.667,-0.591) (80.000,-0.758) (86.667,-0.856) (100.000,-0.916) (8.333,-0.167) (16.667,-0.392) (25.000,-0.431) (33.333,-0.488) (50.000,-0.580) (58.333,-0.656) (66.667,-0.689) (75.000,-0.769) (83.333,-0.882) (100.000,-0.916) (6.667,0.013) (20.000,-0.228) (26.667,-0.294) (40.000,-0.398) (46.667,-0.507) (60.000,-0.599) (66.667,-0.653) (80.000,-0.766) (86.667,-0.802) (100.000,-0.942) (6.250,-0.162) (18.750,-0.214) (25.000,-0.258) (37.500,-0.403) (50.000,-0.461) (56.250,-0.547) (68.750,-0.666) (75.000,-0.722) (87.500,-0.897) (100.000,-0.897) (9.524,-0.152) (19.048,-0.257) (28.571,-0.359) (38.095,-0.414) (47.619,-0.506) (57.143,-0.553) (66.667,-0.638) (76.190,-0.709) (85.714,-0.776) (100.000,-0.916) (5.556,-0.193) (16.667,-0.314) (27.778,-0.389) (38.889,-0.425) (50.000,-0.542) (55.556,-0.565) (66.667,-0.616) (77.778,-0.743) (88.889,-0.879) (100.000,-0.959) (9.524,-0.121) (19.048,-0.170) (28.571,-0.281) (38.095,-0.393) (47.619,-0.445) (57.143,-0.581) (66.667,-0.651) (76.190,-0.741) (85.714,-0.796) (100.000,-0.877) (6.667,-0.057) (20.000,-0.176) (26.667,-0.264) (40.000,-0.386) (46.667,-0.469) (60.000,-0.539) (66.667,-0.620) (80.000,-0.774) (86.667,-0.836) (100.000,-0.897) (7.407,-0.215) (18.519,-0.335) (29.630,-0.375) (37.037,-0.392) (48.148,-0.482) (59.259,-0.597) (66.667,-0.662) (77.778,-0.729) (88.889,-0.828) (100.000,-0.861) (5.882,0.039) (17.647,-0.116) (29.412,-0.287) (35.294,-0.300) (47.059,-0.463) (58.824,-0.542) (64.706,-0.630) (76.471,-0.732) (88.235,-0.798) (100.000,-0.919) (6.250,-0.058) (18.750,-0.175) (25.000,-0.211) (37.500,-0.297) (50.000,-0.391) (56.250,-0.461) (68.750,-0.609) (75.000,-0.644) (87.500,-0.730) (100.000,-0.921) (8.333,-0.124) (16.667,-0.212) (29.167,-0.326) (37.500,-0.367) (50.000,-0.457) (58.333,-0.489) (66.667,-0.530) (79.167,-0.645) (87.500,-0.711) (100.000,-0.780) (7.692,-0.078) (19.231,-0.205) (26.923,-0.296) (38.462,-0.386) (50.000,-0.566) (57.692,-0.604) (69.231,-0.674) (76.923,-0.742) (88.462,-0.835) (100.000,-0.891) (8.696,-0.143) (17.391,-0.310) (26.087,-0.347) (39.130,-0.472) (47.826,-0.503) (56.522,-0.543) (69.565,-0.702) (78.261,-0.766) (86.957,-0.828) (100.000,-0.923) (5.882,-0.043) (17.647,-0.197) (29.412,-0.275) (35.294,-0.380) (47.059,-0.486) (58.824,-0.592) (64.706,-0.666) (76.471,-0.710) (88.235,-0.811) (100.000,-0.924) (6.897,-0.186) (17.241,-0.366) (27.586,-0.420) (37.931,-0.446) (48.276,-0.507) (58.621,-0.554) (68.966,-0.626) (79.310,-0.681) (89.655,-0.790) (100.000,-0.846) (7.407,-0.156) (18.519,-0.263) (29.630,-0.367) (37.037,-0.409) (48.148,-0.527) (59.259,-0.567) (66.667,-0.594) (77.778,-0.667) (88.889,-0.772) (100.000,-0.888) (6.667,-0.102) (20.000,-0.232) (26.667,-0.303) (40.000,-0.385) (46.667,-0.427) (60.000,-0.546) (66.667,-0.618) (80.000,-0.751) (86.667,-0.850) (100.000,-0.975) (6.667,-0.094) (20.000,-0.207) (26.667,-0.375) (40.000,-0.477) (46.667,-0.545) (60.000,-0.618) (66.667,-0.697) (80.000,-0.803) (86.667,-0.877) (100.000,-0.916) (5.882,0.007) (17.647,-0.229) (29.412,-0.336) (35.294,-0.349) (47.059,-0.436) (58.824,-0.562) (64.706,-0.575) (76.471,-0.686) (88.235,-0.865) (100.000,-0.904) (9.804,-0.291) (19.608,-0.324) (29.412,-0.355) (39.869,-0.410) (49.673,-0.474) (59.477,-0.525) (69.935,-0.564) (79.739,-0.629) (89.542,-0.672) (100.000,-0.730) (5.556,-0.158) (16.667,-0.325) (27.778,-0.454) (38.889,-0.522) (50.000,-0.596) (55.556,-0.601) (66.667,-0.689) (77.778,-0.721) (88.889,-0.771) (100.000,-0.843) (6.667,-0.114) (20.000,-0.224) (26.667,-0.284) (40.000,-0.393) (46.667,-0.468) (60.000,-0.586) (66.667,-0.634) (80.000,-0.745) (86.667,-0.778) (100.000,-0.875) (8.333,-0.148) (16.667,-0.246) (29.167,-0.396) (37.500,-0.447) (50.000,-0.490) (58.333,-0.600) (66.667,-0.710) (79.167,-0.806) (87.500,-0.840) (100.000,-0.840) (7.143,-0.141) (14.286,-0.182) (28.571,-0.292) (35.714,-0.352) (50.000,-0.461) (57.143,-0.600) (64.286,-0.655) (78.571,-0.745) (85.714,-0.822) (100.000,-0.934) (5.263,-0.022) (15.789,-0.178) (26.316,-0.252) (36.842,-0.355) (47.368,-0.438) (57.895,-0.557) (68.421,-0.606) (78.947,-0.713) (89.474,-0.806) (100.000,-0.818) (5.882,-0.192) (17.647,-0.273) (29.412,-0.313) (35.294,-0.387) (47.059,-0.480) (58.824,-0.534) (64.706,-0.619) (76.471,-0.714) (88.235,-0.790) (100.000,-0.971) (6.250,-0.057) (18.750,-0.206) (25.000,-0.263) (37.500,-0.371) (50.000,-0.511) (56.250,-0.552) (68.750,-0.691) (75.000,-0.699) (87.500,-0.830) (100.000,-0.895) (5.882,-0.026) (17.647,-0.154) (29.412,-0.296) (35.294,-0.414) (47.059,-0.509) (58.824,-0.583) (64.706,-0.654) (76.471,-0.821) (88.235,-0.903) (100.000,-0.985) (6.667,-0.067) (20.000,-0.202) (26.667,-0.281) (40.000,-0.418) (46.667,-0.434) (60.000,-0.622) (66.667,-0.630) (80.000,-0.742) (86.667,-0.766) (100.000,-0.883) (9.091,-0.127) (18.182,-0.270) (27.273,-0.361) (39.394,-0.394) (48.485,-0.422) (57.576,-0.451) (69.697,-0.581) (78.788,-0.606) (87.879,-0.654) (100.000,-0.853) (8.333,-0.062) (16.667,-0.186) (25.000,-0.204) (33.333,-0.302) (50.000,-0.423) (58.333,-0.515) (66.667,-0.568) (75.000,-0.674) (83.333,-0.711) (100.000,-0.928) (6.897,-0.167) (17.241,-0.281) (27.586,-0.396) (37.931,-0.449) (48.276,-0.516) (58.621,-0.612) (68.966,-0.692) (79.310,-0.776) (89.655,-0.836) (100.000,-0.836) (6.250,-0.061) (18.750,-0.184) (25.000,-0.224) (37.500,-0.336) (50.000,-0.421) (56.250,-0.428) (68.750,-0.660) (75.000,-0.733) (87.500,-0.870) (100.000,-0.982) (7.143,-0.164) (17.857,-0.318) (28.571,-0.387) (39.286,-0.432) (50.000,-0.473) (57.143,-0.519) (67.857,-0.565) (78.571,-0.603) (89.286,-0.750) (100.000,-0.872) (7.143,-0.101) (14.286,-0.165) (28.571,-0.272) (35.714,-0.299) (50.000,-0.474) (57.143,-0.535) (64.286,-0.560) (78.571,-0.710) (85.714,-0.876) (100.000,-0.923) (9.091,-0.062) (18.182,-0.185) (27.273,-0.295) (36.364,-0.304) (45.455,-0.408) (54.545,-0.479) (63.636,-0.584) (72.727,-0.681) (81.818,-0.766) (100.000,-0.871) (10.000,-0.106) (20.000,-0.198) (30.000,-0.306) (40.000,-0.390) (50.000,-0.449) (60.000,-0.522) (70.000,-0.597) (80.000,-0.720) (90.000,-0.785) (100.000,-0.891) (9.524,-0.068) (19.048,-0.167) (28.571,-0.228) (38.095,-0.330) (47.619,-0.398) (57.143,-0.460) (66.667,-0.593) (76.190,-0.715) (85.714,-0.764) (100.000,-0.925) (5.263,-0.033) (15.789,-0.254) (26.316,-0.306) (36.842,-0.446) (47.368,-0.472) (57.895,-0.537) (68.421,-0.599) (78.947,-0.673) (89.474,-0.740) (100.000,-0.868) (5.882,-0.055) (17.647,-0.178) (29.412,-0.301) (35.294,-0.338) (47.059,-0.429) (58.824,-0.497) (64.706,-0.539) (76.471,-0.663) (88.235,-0.775) (100.000,-0.845) (6.667,-0.107) (20.000,-0.176) (26.667,-0.253) (40.000,-0.354) (46.667,-0.381) (60.000,-0.489) (66.667,-0.566) (80.000,-0.669) (86.667,-0.737) (100.000,-0.906) (8.000,-0.184) (20.000,-0.319) (28.000,-0.357) (40.000,-0.455) (48.000,-0.517) (60.000,-0.595) (68.000,-0.619) (80.000,-0.685) (88.000,-0.781) (100.000,-0.835) (7.407,-0.183) (18.519,-0.288) (29.630,-0.330) (37.037,-0.375) (48.148,-0.468) (59.259,-0.571) (66.667,-0.641) (77.778,-0.747) (88.889,-0.801) (100.000,-0.838) (5.263,-0.149) (15.789,-0.335) (26.316,-0.354) (36.842,-0.467) (47.368,-0.487) (57.895,-0.623) (68.421,-0.653) (78.947,-0.718) (89.474,-0.807) (100.000,-0.856) (5.882,-0.070) (17.647,-0.240) (29.412,-0.354) (35.294,-0.375) (47.059,-0.494) (58.824,-0.596) (64.706,-0.624) (76.471,-0.741) (88.235,-0.837) (100.000,-0.865) (5.263,-0.116) (15.789,-0.193) (26.316,-0.342) (36.842,-0.361) (47.368,-0.466) (57.895,-0.562) (68.421,-0.652) (78.947,-0.746) (89.474,-0.832) (100.000,-0.889) (9.091,-0.112) (18.182,-0.185) (27.273,-0.232) (36.364,-0.274) (45.455,-0.426) (54.545,-0.441) (63.636,-0.540) (72.727,-0.698) (81.818,-0.722) (100.000,-0.917) (10.000,-0.189) (20.000,-0.273) (30.000,-0.405) (40.000,-0.426) (50.000,-0.461) (60.000,-0.567) (70.000,-0.641) (80.000,-0.678) (90.000,-0.800) (100.000,-0.845) (5.556,-0.088) (16.667,-0.192) (27.778,-0.268) (38.889,-0.313) (50.000,-0.406) (55.556,-0.524) (66.667,-0.578) (77.778,-0.761) (88.889,-0.840) (100.000,-0.911) (9.756,-0.232) (19.512,-0.347) (29.268,-0.372) (39.024,-0.415) (48.780,-0.434) (58.537,-0.471) (68.293,-0.511) (78.049,-0.552) (87.805,-0.626) (100.000,-0.798) 
            }; \addlegendentry{$\errLinfPosRel$}
        \end{axis}
    \end{tikzpicture}
    \label{figure_real_data_relative_packets}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    \hspace*{-2.1em}  % reduces horizontal space!
    ~
    \subfigure[$W=24$ (right)] {
        \begin{tikzpicture}
            \begin{axis}[
                width=0.2\textwidth,
        		height=0.2\textwidth,
        		xmin=0,
        		xmax=100,
        		xtick={0,20,40,60,80,100},
        		xlabel={\% of required rules},
        		ymin=-1.2, ymax = 0.2,
                ytick={-1.2,-1.0,-0.8,-0.6,-0.4,-0.2,0,0.2},
                %ylabel= {$\errLinfPosRel$ error},
                style={font=\scriptsize}, % two-levels smaller than 'small' which is the default size.
        		legend style={at={(0.01,0.01)}, anchor=south west,font=\footnotesize,legend columns=-1,},
        		label style={font=\footnotesize},
        		grid=both
            ]
            \addplot [purple,mark=*,only marks,mark size=1pt] coordinates{
            (8.333,-0.136) (19.444,-0.207) (27.778,-0.289) (38.889,-0.390) (50.000,-0.438) (58.333,-0.485) (69.444,-0.593) (77.778,-0.648) (88.889,-0.849) (100.000,-0.897) (7.692,-0.079) (19.231,-0.186) (26.923,-0.228) (38.462,-0.344) (50.000,-0.429) (57.692,-0.472) (69.231,-0.649) (76.923,-0.710) (88.462,-0.835) (100.000,-0.904) (8.163,-0.096) (18.367,-0.202) (28.571,-0.270) (38.776,-0.348) (48.980,-0.451) (59.184,-0.540) (69.388,-0.620) (79.592,-0.730) (89.796,-0.832) (100.000,-0.888) (9.677,-0.136) (19.355,-0.255) (29.032,-0.310) (38.710,-0.392) (48.387,-0.463) (58.065,-0.530) (67.742,-0.645) (77.419,-0.754) (87.097,-0.781) (100.000,-0.937) (10.000,-0.066) (20.000,-0.150) (30.000,-0.236) (40.000,-0.335) (50.000,-0.458) (60.000,-0.531) (70.000,-0.626) (80.000,-0.716) (90.000,-0.789) (100.000,-0.920) (7.692,-0.068) (19.231,-0.135) (26.923,-0.219) (38.462,-0.302) (50.000,-0.418) (57.692,-0.523) (69.231,-0.605) (76.923,-0.717) (88.462,-0.819) (100.000,-0.933) (9.091,-0.112) (18.182,-0.201) (27.273,-0.274) (39.394,-0.357) (48.485,-0.431) (57.576,-0.563) (69.697,-0.640) (78.788,-0.704) (87.879,-0.867) (100.000,-0.915) (8.824,-0.106) (17.647,-0.146) (29.412,-0.267) (38.235,-0.343) (50.000,-0.439) (58.824,-0.531) (67.647,-0.614) (79.412,-0.733) (88.235,-0.857) (100.000,-0.897) (8.108,-0.122) (18.919,-0.189) (29.730,-0.294) (37.838,-0.336) (48.649,-0.443) (59.459,-0.559) (67.568,-0.644) (78.378,-0.733) (89.189,-0.840) (100.000,-0.914) (9.091,-0.113) (19.697,-0.239) (28.788,-0.293) (39.394,-0.365) (50.000,-0.455) (59.091,-0.564) (69.697,-0.631) (78.788,-0.708) (89.394,-0.789) (100.000,-0.862) (8.475,-0.130) (18.644,-0.190) (28.814,-0.252) (38.983,-0.320) (49.153,-0.421) (59.322,-0.523) (69.492,-0.586) (79.661,-0.668) (89.831,-0.785) (100.000,-0.881) (8.163,-0.185) (18.367,-0.273) (28.571,-0.328) (38.776,-0.396) (48.980,-0.467) (59.184,-0.554) (69.388,-0.630) (79.592,-0.691) (89.796,-0.815) (100.000,-0.891) (10.000,-0.142) (20.000,-0.231) (30.000,-0.271) (40.000,-0.351) (50.000,-0.415) (60.000,-0.513) (70.000,-0.642) (80.000,-0.706) (90.000,-0.812) (100.000,-0.913) (8.696,-0.101) (17.391,-0.147) (26.087,-0.221) (39.130,-0.299) (47.826,-0.432) (56.522,-0.518) (69.565,-0.617) (78.261,-0.687) (86.957,-0.761) (100.000,-0.930) (8.108,-0.115) (18.919,-0.203) (29.730,-0.274) (37.838,-0.342) (48.649,-0.443) (59.459,-0.501) (67.568,-0.582) (78.378,-0.710) (89.189,-0.792) (100.000,-0.909) (9.302,-0.118) (18.605,-0.189) (27.907,-0.281) (39.535,-0.382) (48.837,-0.445) (58.140,-0.581) (69.767,-0.651) (79.070,-0.737) (88.372,-0.806) (100.000,-0.880) (8.696,-0.055) (17.391,-0.181) (26.087,-0.274) (39.130,-0.354) (47.826,-0.474) (56.522,-0.559) (69.565,-0.670) (78.261,-0.759) (86.957,-0.814) (100.000,-0.952) (7.895,-0.153) (18.421,-0.273) (28.947,-0.356) (39.474,-0.404) (50.000,-0.540) (57.895,-0.602) (68.421,-0.669) (78.947,-0.761) (89.474,-0.840) (100.000,-0.919) (9.091,-0.092) (18.182,-0.169) (27.273,-0.259) (39.394,-0.340) (48.485,-0.424) (57.576,-0.475) (69.697,-0.631) (78.788,-0.696) (87.879,-0.804) (100.000,-0.925) (9.091,-0.106) (18.182,-0.219) (27.273,-0.292) (39.394,-0.374) (48.485,-0.490) (57.576,-0.566) (69.697,-0.660) (78.788,-0.746) (87.879,-0.815) (100.000,-0.944) (8.000,-0.015) (20.000,-0.144) (28.000,-0.168) (40.000,-0.343) (48.000,-0.420) (60.000,-0.520) (68.000,-0.596) (80.000,-0.735) (88.000,-0.846) (100.000,-0.946) (8.696,-0.084) (17.391,-0.164) (26.087,-0.253) (39.130,-0.371) (47.826,-0.406) (56.522,-0.453) (69.565,-0.685) (78.261,-0.763) (86.957,-0.853) (100.000,-0.974) (10.000,-0.125) (20.000,-0.268) (30.000,-0.355) (40.000,-0.454) (50.000,-0.500) (60.000,-0.609) (70.000,-0.731) (80.000,-0.834) (90.000,-0.884) (100.000,-0.949) (8.333,-0.055) (16.667,-0.178) (29.167,-0.325) (37.500,-0.357) (50.000,-0.547) (58.333,-0.579) (66.667,-0.664) (79.167,-0.756) (87.500,-0.860) (100.000,-0.952) (7.143,-0.121) (17.857,-0.194) (28.571,-0.277) (39.286,-0.358) (50.000,-0.474) (57.143,-0.522) (67.857,-0.670) (78.571,-0.793) (89.286,-0.858) (100.000,-0.972) (8.824,-0.099) (17.647,-0.192) (29.412,-0.300) (38.235,-0.380) (50.000,-0.461) (58.824,-0.562) (67.647,-0.611) (79.412,-0.738) (88.235,-0.840) (100.000,-0.902) (7.692,-0.123) (19.231,-0.209) (26.923,-0.266) (38.462,-0.346) (50.000,-0.508) (57.692,-0.554) (69.231,-0.711) (76.923,-0.764) (88.462,-0.841) (100.000,-0.950) (9.677,-0.129) (19.355,-0.224) (29.032,-0.263) (38.710,-0.366) (48.387,-0.453) (58.065,-0.506) (67.742,-0.632) (77.419,-0.743) (87.097,-0.810) (100.000,-0.938) (9.524,-0.122) (19.048,-0.199) (28.571,-0.262) (38.095,-0.381) (47.619,-0.440) (57.143,-0.523) (66.667,-0.572) (76.190,-0.670) (85.714,-0.801) (100.000,-0.910) (7.692,-0.201) (17.949,-0.259) (28.205,-0.319) (38.462,-0.406) (48.718,-0.472) (58.974,-0.561) (69.231,-0.644) (79.487,-0.701) (89.744,-0.766) (100.000,-0.889) (10.000,-0.117) (20.000,-0.191) (30.000,-0.293) (40.000,-0.443) (50.000,-0.544) (60.000,-0.626) (70.000,-0.733) (80.000,-0.781) (90.000,-0.928) (100.000,-0.963) (7.407,-0.113) (18.519,-0.182) (29.630,-0.324) (37.037,-0.379) (48.148,-0.506) (59.259,-0.563) (66.667,-0.664) (77.778,-0.771) (88.889,-0.879) (100.000,-0.936) (9.302,-0.131) (18.605,-0.224) (27.907,-0.323) (39.535,-0.380) (48.837,-0.461) (58.140,-0.542) (69.767,-0.632) (79.070,-0.722) (88.372,-0.803) (100.000,-0.918) (9.375,-0.049) (18.750,-0.149) (28.125,-0.228) (37.500,-0.376) (50.000,-0.475) (59.375,-0.576) (68.750,-0.671) (78.125,-0.753) (87.500,-0.809) (100.000,-0.957) (8.571,-0.119) (20.000,-0.224) (28.571,-0.279) (40.000,-0.358) (48.571,-0.440) (60.000,-0.563) (68.571,-0.638) (80.000,-0.709) (88.571,-0.822) (100.000,-0.897) (7.407,-0.040) (18.519,-0.191) (29.630,-0.277) (37.037,-0.339) (48.148,-0.464) (59.259,-0.550) (66.667,-0.612) (77.778,-0.750) (88.889,-0.860) (100.000,-0.923) (8.333,-0.170) (18.750,-0.271) (29.167,-0.315) (39.583,-0.384) (50.000,-0.499) (58.333,-0.579) (68.750,-0.644) (79.167,-0.721) (89.583,-0.785) (100.000,-0.879) (9.091,-0.143) (18.182,-0.254) (29.545,-0.376) (38.636,-0.425) (50.000,-0.499) (59.091,-0.571) (68.182,-0.658) (79.545,-0.766) (88.636,-0.847) (100.000,-0.889) (9.091,-0.090) (18.182,-0.174) (27.273,-0.261) (36.364,-0.311) (50.000,-0.417) (59.091,-0.576) (68.182,-0.653) (77.273,-0.777) (86.364,-0.893) (100.000,-0.974) (9.091,-0.058) (18.182,-0.141) (27.273,-0.318) (36.364,-0.326) (50.000,-0.517) (59.091,-0.621) (68.182,-0.655) (77.273,-0.742) (86.364,-0.803) (100.000,-0.939) (6.897,-0.033) (17.241,-0.196) (27.586,-0.242) (37.931,-0.341) (48.276,-0.419) (58.621,-0.548) (68.966,-0.652) (79.310,-0.719) (89.655,-0.809) (100.000,-0.904) (9.633,-0.204) (19.725,-0.244) (29.817,-0.285) (39.908,-0.355) (50.000,-0.430) (59.633,-0.504) (69.725,-0.582) (79.817,-0.647) (89.908,-0.736) (100.000,-0.789) (9.677,-0.199) (19.355,-0.351) (29.032,-0.428) (38.710,-0.468) (48.387,-0.546) (58.065,-0.631) (67.742,-0.667) (77.419,-0.713) (87.097,-0.786) (100.000,-0.908) (8.000,-0.076) (20.000,-0.177) (28.000,-0.234) (40.000,-0.327) (48.000,-0.398) (60.000,-0.480) (68.000,-0.566) (80.000,-0.672) (88.000,-0.768) (100.000,-0.888) (7.692,-0.138) (17.949,-0.280) (28.205,-0.363) (38.462,-0.428) (48.718,-0.515) (58.974,-0.606) (69.231,-0.695) (79.487,-0.756) (89.744,-0.826) (100.000,-0.870) (10.000,-0.095) (20.000,-0.174) (30.000,-0.315) (40.000,-0.448) (50.000,-0.515) (60.000,-0.558) (70.000,-0.680) (80.000,-0.811) (90.000,-0.860) (100.000,-0.934) (9.677,-0.100) (19.355,-0.227) (29.032,-0.307) (38.710,-0.357) (48.387,-0.457) (58.065,-0.527) (67.742,-0.637) (77.419,-0.693) (87.097,-0.852) (100.000,-0.951) (7.692,-0.093) (19.231,-0.207) (26.923,-0.296) (38.462,-0.359) (50.000,-0.491) (57.692,-0.566) (69.231,-0.672) (76.923,-0.737) (88.462,-0.804) (100.000,-0.970) (10.000,-0.091) (20.000,-0.163) (30.000,-0.214) (40.000,-0.288) (50.000,-0.400) (60.000,-0.519) (70.000,-0.634) (80.000,-0.672) (90.000,-0.845) (100.000,-0.910) (9.091,-0.075) (18.182,-0.173) (27.273,-0.288) (36.364,-0.314) (50.000,-0.419) (59.091,-0.513) (68.182,-0.601) (77.273,-0.644) (86.364,-0.793) (100.000,-0.923) (7.407,-0.051) (18.519,-0.205) (29.630,-0.323) (37.037,-0.378) (48.148,-0.469) (59.259,-0.561) (66.667,-0.663) (77.778,-0.770) (88.889,-0.824) (100.000,-0.923) (8.511,-0.140) (19.149,-0.258) (29.787,-0.298) (38.298,-0.328) (48.936,-0.387) (59.574,-0.484) (68.085,-0.560) (78.723,-0.698) (89.362,-0.801) (100.000,-0.868) (8.696,-0.062) (17.391,-0.159) (26.087,-0.252) (39.130,-0.358) (47.826,-0.409) (56.522,-0.546) (69.565,-0.676) (78.261,-0.809) (86.957,-0.891) (100.000,-0.977) (7.692,-0.109) (17.949,-0.226) (28.205,-0.292) (38.462,-0.345) (48.718,-0.423) (58.974,-0.542) (69.231,-0.638) (79.487,-0.692) (89.744,-0.820) (100.000,-0.869) (8.696,-0.073) (17.391,-0.160) (26.087,-0.246) (39.130,-0.347) (47.826,-0.450) (56.522,-0.539) (69.565,-0.653) (78.261,-0.717) (86.957,-0.814) (100.000,-0.963) (9.302,-0.100) (18.605,-0.216) (27.907,-0.297) (39.535,-0.357) (48.837,-0.439) (58.140,-0.556) (69.767,-0.619) (79.070,-0.735) (88.372,-0.848) (100.000,-0.888) (7.692,-0.043) (19.231,-0.216) (26.923,-0.292) (38.462,-0.379) (50.000,-0.537) (57.692,-0.632) (69.231,-0.708) (76.923,-0.777) (88.462,-0.904) (100.000,-0.975) (5.263,-0.014) (15.789,-0.126) (26.316,-0.269) (36.842,-0.347) (47.368,-0.397) (57.895,-0.590) (68.421,-0.665) (78.947,-0.735) (89.474,-0.884) (100.000,-0.938) (9.375,-0.049) (18.750,-0.223) (28.125,-0.287) (37.500,-0.339) (50.000,-0.475) (59.375,-0.603) (68.750,-0.660) (78.125,-0.722) (87.500,-0.801) (100.000,-0.920) (9.677,-0.071) (19.355,-0.169) (29.032,-0.238) (38.710,-0.289) (48.387,-0.379) (58.065,-0.513) (67.742,-0.584) (77.419,-0.681) (87.097,-0.803) (100.000,-0.917) (8.824,-0.153) (17.647,-0.256) (29.412,-0.320) (38.235,-0.427) (50.000,-0.528) (58.824,-0.576) (67.647,-0.662) (79.412,-0.723) (88.235,-0.786) (100.000,-0.924) (7.407,-0.076) (18.519,-0.176) (29.630,-0.290) (37.037,-0.364) (48.148,-0.449) (59.259,-0.513) (66.667,-0.614) (77.778,-0.672) (88.889,-0.811) (100.000,-0.983) (8.333,-0.069) (16.667,-0.161) (29.167,-0.259) (37.500,-0.388) (50.000,-0.491) (58.333,-0.615) (66.667,-0.660) (79.167,-0.754) (87.500,-0.791) (100.000,-0.948) (8.108,-0.135) (18.919,-0.211) (29.730,-0.284) (37.838,-0.331) (48.649,-0.445) (59.459,-0.539) (67.568,-0.615) (78.378,-0.763) (89.189,-0.848) (100.000,-0.918) (8.108,-0.104) (18.919,-0.188) (29.730,-0.274) (37.838,-0.315) (48.649,-0.426) (59.459,-0.520) (67.568,-0.594) (78.378,-0.694) (89.189,-0.770) (100.000,-0.890) (6.897,-0.103) (17.241,-0.205) (27.586,-0.256) (37.931,-0.352) (48.276,-0.537) (58.621,-0.588) (68.966,-0.641) (79.310,-0.784) (89.655,-0.895) (100.000,-0.919) (7.143,-0.102) (17.857,-0.245) (28.571,-0.349) (39.286,-0.414) (50.000,-0.492) (57.143,-0.545) (67.857,-0.620) (78.571,-0.786) (89.286,-0.857) (100.000,-0.940) (9.375,-0.097) (18.750,-0.239) (28.125,-0.311) (37.500,-0.364) (50.000,-0.498) (59.375,-0.556) (68.750,-0.630) (78.125,-0.742) (87.500,-0.794) (100.000,-0.946) (5.556,-0.013) (16.667,-0.124) (27.778,-0.223) (38.889,-0.359) (50.000,-0.523) (55.556,-0.528) (66.667,-0.628) (77.778,-0.804) (88.889,-0.855) (100.000,-0.984) (9.091,-0.127) (18.182,-0.217) (27.273,-0.279) (39.394,-0.363) (48.485,-0.421) (57.576,-0.479) (69.697,-0.598) (78.788,-0.692) (87.879,-0.768) (100.000,-0.871) (10.000,-0.073) (20.000,-0.194) (30.000,-0.299) (40.000,-0.351) (50.000,-0.475) (60.000,-0.545) (70.000,-0.592) (80.000,-0.717) (90.000,-0.830) (100.000,-0.932) (9.375,-0.200) (18.750,-0.287) (29.688,-0.332) (39.062,-0.374) (50.000,-0.488) (59.375,-0.530) (68.750,-0.619) (79.688,-0.726) (89.062,-0.793) (100.000,-0.869) 
            }; \addlegendentry{$\errLinfPosRel$}
        \end{axis}
    \end{tikzpicture}
    \label{figure_real_data_relative_bytes}
    }% %not sure why this '%' is necessary, but otherwise the third figure breaks into a new row of sub-figures.
    
    \caption{Scatter plots of error versus number of rules for ``real data'' partitions. The number of rules is normalized by $n^*(P)$, the maximum number of rules needed for the lowest possible error (e.g.\ zero-error if the partition is integer).
    All three kinds of errors, $\errLinf$, $\errLinfPos$ and $\errLinfPosRel$, are presented in log-scale normalized by the width $W$. The columns plot, from left to right: session-partitions ($W=8$), packets-partitions ($W=16$), bytes-partitions ($W=24$) as explained in Section~\ref{subsection_experiments_real_data_partitions}. To reduce cluttering, only the first 72 partition out of 240 are used for the plot. Each partition corresponds to 10 points: the $i$th point gives the error when we approximate this partition with  $\floor{\frac{i \cdot n^*(P)}{10}}$ rules for $i=1,\ldots,10$.
    }
    \label{figure_real_data_all}
\end{figure}

